Representing Conversations for Scalable Overhearing

Open distributed multi-agent systems are gaining interest in the academic community and in industry. In such open settings, agents are often coordinated using standardized agent conversation protocols. The representation of such protocols (for analysis, validation, monitoring, etc) is an important aspect of multi-agent applications. Recently, Petri nets have been shown to be an interesting approach to such representation, and radically different approaches using Petri nets have been proposed. However, their relative strengths and weaknesses have not been examined. Moreover, their scalability and suitability for different tasks have not been addressed. This paper addresses both these challenges. First, we analyze existing Petri net representations in terms of their scalability and appropriateness for overhearing, an important task in monitoring open multi-agent systems. Then, building on the insights gained, we introduce a novel representation using Colored Petri nets that explicitly represent legal joint conversation states and messages. This representation approach offers significant improvements in scalability and is particularly suitable for overhearing. Furthermore, we show that this new representation offers a comprehensive coverage of all conversation features of FIPA conversation standards. We also present a procedure for transforming AUML conversation protocol diagrams (a standard human-readable representation), to our Colored Petri net representation.

==> helmert06a/architecture.tex <==
\section{Fast Downward}
\label{section:architecture}

We will now describe the overall architecture of the planner. Fast
Downward is a classical planning system based on the ideas of
heuristic forward search and hierarchical problem decomposition. It
can deal with the full range of propositional PDDL2.2
\cite{pddl2,pddl2.2}, {\ie}, in addition to STRIPS planning, it
supports arbitrary formulae in operator preconditions and goal
conditions, and it can deal with conditional and universally
quantified effects and derived predicates (axioms).

The name of the planner derives from two sources: Of course, one of
these sources is Hoffmann's very successful FF (``Fast Forward'')
planner \cite{ff}. Like FF, Fast Downward is a heuristic progression
planner, {\ie}, it computes plans by heuristic search in the space of
world states reachable from the initial situation. However, compared
to FF, Fast Downward uses a very different heuristic evaluation
function called the \emph{causal graph heuristic}. The heuristic
evaluator proceeds ``downward'' in so far as it tries to solve
planning tasks in the hierarchical fashion outlined in the introduction.
Starting from top-level goals, the algorithm recurses further and
further down the causal graph until all remaining subproblems are
basic graph search tasks.

Similar to FF, the planner has shown excellent performance: The original
implementation of the causal graph heuristic, plugged into a standard
best-first search algorithm, outperformed the previous champions in that
area, FF and LPG \cite{lpg}, on the set of STRIPS benchmarks from the
first three international planning competitions \cite{malte-icaps-cg}.
Fast Downward itself followed in the footsteps of FF and LPG by winning
the propositional, non-optimizing track of the 4th International
Planning Competition at ICAPS 2004 (referred to as IPC4 from now on).

As mentioned in the introduction, Fast Downward solves a planning task
in three phases (Fig.~\ref{figure:modules}):

\includepsfigure{modules}{The three phases of Fast Downward's
  execution.}

\begin{itemize}
\item The \emph{translation} component is responsible for transforming
  the PDDL2.2 input into a non-binary form which is more amenable to
  hierarchical planning approaches. It applies a number of
  normalizations to compile away syntactic constructs like
  disjunctions which are not directly supported by the causal graph
  heuristic and performs grounding of axioms and operators. Most
  importantly, it uses invariant synthesis methods to find groups of
  related propositions which can be encoded as a single multi-valued
  variable. The output of the translation component is a
  \emph{multi-valued planning task}, defined in the following section.
\item The \emph{knowledge compilation} component generates four kinds of
  data structures that play a central role during search: \emph{Domain
  transition graphs} encode how, and under what conditions, state
  variables can change their values. The \emph{causal graph} represents
  the hierarchical dependencies between the different state variables.
  The \emph{successor generator} is an efficient data structure for
  determining the set of applicable operators in a given state.
  Finally, the \emph{axiom evaluator} is an efficient data structure for
  computing the values of derived variables. The knowledge
  compilation component is described in Section
  \ref{section:knowledge-compilation}.
\item The \emph{search} component implements three different search
  algorithms to do the actual planning. Two of these algorithms make
  use of heuristic evaluation functions: One is the well-known greedy
  best-first search algorithm, using the causal graph heuristic. The
  other is called \emph{multi-heuristic best-first search}, a variant
  of greedy best-first search that tries to combine several heuristic
  evaluators in an orthogonal way; in the case of Fast Downward, it
  uses the causal graph and FF heuristics. The third search algorithm
  is called \emph{focused iterative-broadening search}; it is closely
  related to Ginsberg and Harvey's \citeyear{ginsberg-harvey:aij92}
  iterative broadening. It is not a heuristic search algorithm in the
  sense that it does not use an explicit heuristic evaluation
  function. Instead, it uses the information encoded in the causal
  graph to estimate the ``usefulness'' of operators towards satisfying
  the goals of the task. The search component is described in Section
  \ref{section:search}.
\end{itemize}


==> helmert06a/commands.tex <==
% Theorem-like environments.
\newtheorem{def1}{Definition}
\newtheorem{obs1}[def1]{Observation}

\newenvironment{definition}[2]
  {\begin{def1}{\label{def:#1}}\definedTerm{#2}\\ }
  {\end{def1}}
\newenvironment{observation}[2]
  {\begin{obs1}{\label{observation:#1}}\definedTerm{#2}\\ }
  {\end{obs1}}

% Algorithm environment.
\newenvironment{algorithm}
  {\begin{upshape}\setlength{\parindent}{0cm}}
  {\end{upshape}}

% Macros for including figures.

\newcommand{\includefigure}[3][tbp]{
  \begin{figure}[#1]
    \begin{center}
      \input{figures/#2}
    \end{center}
    \caption{#3}
    \label{figure:#2}
  \end{figure}
}

\newcommand{\includepsfigure}[3][tbp]{
  \begin{figure}[#1]
    \begin{center}
      \includegraphics{figures/#2}
    \end{center}
    \caption{#3}
    \label{figure:#2}
  \end{figure}
}

\newcommand{\includegraph}[3][tbp]{
  \begin{figure}[#1]
    \begin{center}
      \includegraphics{figures/#2}
    \end{center}
    \caption{#3}
    \label{figure:#2}
  \end{figure}
}

% Macros for typesetting abbreviations with the proper spacing (small
% space between the two words in e.g. and i.e., word spacing (not
% sentence spacing) after the abbreviations.

\newcommand{\cf}{cf.\@}
\newcommand{\eg}{e.\,g.\@}
\newcommand{\ie}{i.\,e.\@}

% Multi-character function names etc.
\newcommand{\pre}                   {\textit{pre}}
\newcommand{\eff}                   {\textit{eff}}
\newcommand{\cond}                  {\textit{cond}}

% Auxiliary macros for typesetting decision problems such as 3SAT and
% planning domains such as Blocksworld. These are only used inside
% this file.
\newcommand{\decisionProblem}[1] {\textsc{#1}}
\newcommand{\planningDomain}[1]  {\textsc{#1}}

% Macro for typesetting the defined term of a definition.
\newcommand{\definedTerm}[1]     {\textbf{#1}}

% Typesetting "SAS+" properly.
\newcommand{\sasplus}{SAS\ensuremath{{}^+}}

% Complexity classes.
\newcommand{\NP}                 {\textbf{\textup{NP}}}
\newcommand{\PSPACE}             {\textbf{\textup{PSPACE}}}

% The decision and search problems mentioned in the paper.
\newcommand{\mptplanex}          {\decisionProblem{MPT-PlanEx}}
\newcommand{\mptplan}            {\decisionProblem{MPT-Planning}}

% The planning domains mentioned in this paper.
\newcommand{\airport}            {\planningDomain{Airport}}
\newcommand{\assembly}           {\planningDomain{Assembly}}
\newcommand{\blocksworld}        {\planningDomain{Blocksworld}}
\newcommand{\depot}              {\planningDomain{Depot}}
\newcommand{\driverlog}          {\planningDomain{Driverlog}}
\newcommand{\freecell}           {\planningDomain{Freecell}}
\newcommand{\grid}               {\planningDomain{Grid}}
\newcommand{\gripper}            {\planningDomain{Gripper}}
\newcommand{\logistics}          {\planningDomain{Logistics}}
\newcommand{\miconic}            {\planningDomain{Miconic}}
\newcommand{\miconicstrips}      {\planningDomain{Miconic-STRIPS}}
\newcommand{\miconicsimple}      {\planningDomain{Miconic-SimpleADL}}
\newcommand{\miconicfull}        {\planningDomain{Miconic-FullADL}}
\newcommand{\movie}              {\planningDomain{Movie}}
\newcommand{\mystery}            {\planningDomain{Mystery}}
\newcommand{\mysteryprime}       {\planningDomain{MPrime}}
\newcommand{\opticaltelegraph}   {\planningDomain{Promela-OpticalTelegraph}}
\newcommand{\philosophers}       {\planningDomain{Promela-Philosophers}}
\newcommand{\pipesworld}         {\planningDomain{Pipesworld}}
\newcommand{\pipesworldnotankage}{\planningDomain{Pipesworld-NoTankage}}
\newcommand{\pipesworldtankage}  {\planningDomain{Pipesworld-Tankage}}
\newcommand{\promela}            {\planningDomain{Promela}}
\newcommand{\psr}                {\planningDomain{PSR}}
\newcommand{\psrsmall}           {\planningDomain{PSR-Small}}
\newcommand{\psrmiddle}          {\planningDomain{PSR-Middle}}
\newcommand{\psrlarge}           {\planningDomain{PSR-Large}}
\newcommand{\rovers}             {\planningDomain{Rovers}}
\newcommand{\satellite}          {\planningDomain{Satellite}}
\newcommand{\schedule}           {\planningDomain{Schedule}}
\newcommand{\zenotravel}         {\planningDomain{Zenotravel}}


==> helmert06a/definition.tex <==
\section{Multi-Valued Planning Tasks}
\label{section:definition}

Let us now formally introduce the problem of planning with
multi-valued state variables. Our formalism is based on the
{\sasplus} planning model \cite{complexity-sas,jonsson-sas},
but extends it with axioms and conditional effects.

\begin{definition}{mpt}{Multi-valued planning tasks (MPTs)}
A \definedTerm{multi-valued planning task (MPT)} is given by a
5-tuple $\Pi = \langle \mathcal V, s_0, s_\star, 
\mathcal A, \mathcal O \rangle$ with the following components:
\begin{itemize}
\item
  $\mathcal V$ is a finite set of \definedTerm{state variables}, each
  with an associated finite domain $\mathcal D_v$.
  State variables are partitioned into \definedTerm{fluents} (affected by
  operators) and \definedTerm{derived variables} (computed by evaluating
  axioms). The domains of derived variables must contain the
  \definedTerm{undefined value} $\bot$.

  A \definedTerm{partial variable assignment} or \definedTerm{partial
  state} over $\mathcal V$ is a function $s$ on some subset of
  $\mathcal V$ such that $s(v) \in \mathcal D_v$ wherever $s(v)$ is
  defined. A partial state is called an \definedTerm{extended state}
  if it is defined for all variables in $\mathcal V$ and a
  \definedTerm{reduced state} or \definedTerm{state} if it is defined
  for all fluents in $\mathcal V$. In the context of partial variable
  assignments, we write $v=d$ for the variable-value pairing $(v, d)$
  or $v \mapsto d$.
\item
  $s_0$ is a state over $\mathcal V$ called the \definedTerm{initial state}.
\item
  $s_\star$ is a partial variable assignment over $\mathcal V$ called
  the \definedTerm{goal}.
\item
  $\mathcal A$ is a finite set of (MPT) \definedTerm{axioms} over
  $\mathcal V$. Axioms are triples of the form $\langle \cond, v, d
  \rangle$, where $\cond$ is a partial variable assignment called the
  \definedTerm{condition} or \definedTerm{body} of the axiom,
  $v$ is a derived variable called the \definedTerm{affected variable},
  and $d \in \mathcal D_v$ is called the \definedTerm{derived value}
  for $v$. The pair $(v, d)$ is called the
  \definedTerm{head} of the axiom and can be written as $v:=d$.

  The axiom set $\mathcal A$ is partitioned into a totally ordered set
  of \definedTerm{axiom layers} $\mathcal A_1 \prec \dots \prec \mathcal A_k$
  such that within the same layer, each affected variable may only be
  associated with a single value in axiom heads and bodies. In other
  words, within the same layer, axioms with the same affected variable
  but different derived values are forbidden, and if a variable
  appears in an axiom head, then it may not appear with a different
  value in a body. This is called the \definedTerm{layering property}.
\item
  $\mathcal O$ is a finite set of (MPT) \definedTerm{operators} over $\mathcal
  V$. An operator $\langle \pre, \eff \rangle$ consists of a partial
  variable assignment $\pre$ over $\mathcal V$ called its
  \definedTerm{precondition}, and a finite set of \definedTerm{effects} $\eff$.
  Effects are triples $\langle \cond, v, d \rangle$, where $\cond$ is a (possibly
  empty) partial variable assignment called the \definedTerm{effect condition},
  $v$ is a fluent called the \definedTerm{affected variable}, and $d \in
  \mathcal D_v$ is called the \definedTerm{new value} for $v$.
\end{itemize}

For axioms and effects, we also use the notation $\cond
\rightarrow v:=d$ in place of $\langle \cond, v, d \rangle$.
\end{definition}

To provide a formal semantics for MPT planning, we first need to
formalize axioms:

\begin{definition}{extended-state}{Extended states defined by a state}
Let $s$ be a state of an MPT $\Pi$ with axioms $\mathcal A$, layered
as $\mathcal A_1 \prec \dots \prec \mathcal A_k$. The \definedTerm{extended
state defined by $s$}, written as $\mathcal A(s)$, is the result $s'$
of the following algorithm:

\smallskip

\begin{algorithm}
  \hspace*{0cm}\textbf{algorithm} evaluate-axioms($\mathcal A_1$, $\dots$,
    $\mathcal A_k$, $s$):\\
  \hspace*{1cm}\textbf{for each} variable $v$: \\
  \hspace*{2cm}$s'(v) := \begin{cases}
    s(v) & \text{if $v$ is a fluent variable} \\
    \bot & \text{if $v$ is a derived variable}\end{cases}$ \\
  \hspace*{1cm}\textbf{for} $i \in \{1, \dots, k\}$: \\
  \hspace*{2cm}\textbf{while} there exists an axiom
    $(\cond \rightarrow v := d) \in \mathcal A_i$ with
    $\cond \subseteq s'$ \textbf{and} $s'(v) \neq d$: \\
  \hspace*{3cm}Choose such an axiom $\cond \rightarrow v := d$. \\
  \hspace*{3cm}$s'(v) := d$
\end{algorithm}
\end{definition}

In other words, axioms are evaluated in a layer-by-layer fashion using
fixed point computations, which is very similar to the semantics of
stratified logic programs. It is easy to see that the layering
property from Definition \ref{def:mpt} guarantees that the algorithm
terminates and produces a deterministic result. Having defined the
semantics of axioms, we can now define the state space of an MPT:

\begin{definition}{mpt-state-space}{MPT state spaces}
The \definedTerm{state space} of an MPT
$\Pi = \langle \mathcal V, s_0, s_\star, \mathcal A, \mathcal O \rangle$,
denoted as $\mathcal S(\Pi)$, is a directed graph. Its vertex set is
the set of states of $\mathcal V$, and it contains an arc $(s,s')$ iff
there exists some operator $\langle \pre, \eff \rangle \in \mathcal O$
such that:
\begin{itemize}
\item $\pre \subseteq \mathcal A(s)$,
\item $s'(v) = d$ for all effects $\cond \rightarrow v := d \in
  \eff$ such that $\cond \subseteq \mathcal A(s)$, and
\item $s'(v) = s(v)$ for all other fluents.
\end{itemize}
\end{definition}

Finally, we can define the MPT planning problem:
\begin{definition}{mpt-planning-problem}{MPT planning}
{\mptplanex} is the following decision problem: Given an MPT $\Pi$
with initial state $s_0$ and goal $s_\star$, does
$\mathcal S(\Pi)$ contain a path from $s_0$ to some state $s'$ with
$s_\star \subseteq \mathcal A(s')$?

\smallskip

\noindent
{\mptplan} is the following search problem: Given an MPT $\Pi$
with initial state $s_0$ and goal $s_\star$, compute a path in
$\mathcal S(\Pi)$ from $s_0$ to some state $s'$ with $s_\star
\subseteq \mathcal A(s')$, or prove that none exists.
\end{definition}

The {\mptplanex} problem is easily shown to be \PSPACE-hard because it
generalizes the plan existence problem for propositional STRIPS, which
is known to be \PSPACE-complete \cite{complexity-bylander}. It is also
easy to see that the addition of multi-valued domains, axioms and
conditional effects does not increase the theoretical complexity of MPT
planning beyond propositional STRIPS. Thus, we conclude our formal
introduction of MPT planning by stating that {\mptplanex} is
\PSPACE-complete, and turn to the practical side of things in the
following section.


==> helmert06a/discussion.tex <==
\section{Summary and Discussion}
\label{section:discussion}

Before we turn to discussion, let us briefly summarize the
contributions of this article. As a motivating starting point, we
explained that planning tasks often exhibit a simpler structure if
expressed with \emph{multi-valued state variables}, rather than the
traditional propositional representations. We then introduced
\emph{Fast Downward}, a planning system based on the idea of
converting tasks into a multi-valued formalism and exploiting the
causal information underlying such encodings.

Fast Downward processes PDDL planning tasks in three stages. We
skipped the first of these stages, \emph{translation}, which
automatically transforms a PDDL task into an equivalent multi-valued
planning task with a nicer causal structure. We explained the inner
workings of the second stage, \emph{knowledge compilation},
demonstrating in depth what kind of knowledge the planner extracts
from the problem representation, discussing \emph{causal graphs},
\emph{domain transition graphs}, \emph{successor generators} and
\emph{axiom evaluators}. During our discussion of Fast Downward's
\emph{search} component, we introduced its heuristic search
algorithms, which use the technique of \emph{deferred heuristic
  evaluation} to reduce the number of states for which a heuristic
goal distance estimate must be computed. In addition to greedy
best-first search, Fast Downward employs the \emph{multi-heuristic
best-first search} algorithm to usefully integrate the information
of two heuristic estimators, namely the \emph{causal graph heuristic} and
\emph{FF heuristic}. Both heuristic search algorithms can utilize
preference information about operators. We also introduced Fast
Downward's experimental \emph{focused iterative-broadening search}
algorithm, which is based on the idea of pruning the set of operators
to only consider those successor states which are likely to lead
towards a specific goal.

We thus tried to give a complete account of the Fast Downward
planning system's approach to solving multi-valued planning tasks,
including its motivation, architecture, and algorithmic
foundations. In the previous section, we demonstrated its empirical
behaviour, showing good performance across the whole range of
propositional benchmarks from the previous planning competitions.

Among all the novel algorithms and search enhancements discussed in
this article, there are two aspects of Fast Downward which we consider
of central importance and which we would like to emphasize.
One of them is the use of multi-valued state variables for PDDL-style
planning. We believe that multi-valued representations are much more
structured and hence much more amenable to automated reasoning --- be
it for the purposes of heuristic evaluation, problem decomposition, or
other aspects of planning such as goal ordering or extraction of
landmarks.
The other central idea is the use of hierarchical decompositions
within a heuristic planning framework. Hierarchical approaches to
domain-independent planning have a considerable potential, but since
the work of Knoblock \citeyear{knoblock-abstractions} and Bacchus and
Yang \citeyear{bacchus-downward-refinement}, little work has been
published. With Fast Downward, we hope to renew interest in this area,
which we believe to be a very promising ground for further advances in
automated planning.

For the future, there are several aspects of Fast Downward that we
would like to investigate further. First, we intend to experiment with
other search techniques along the lines of focused
iterative-broadening search, which emphasize heuristically evaluating
operator usefulness rather than heuristically evaluating states.

Second, we would like to come up with an efficient heuristic for
multi-valued planning tasks which does not require pruning cycles of
the causal graph. Initial experiments in this direction have shown
that it is difficult to achieve this goal without losing the
performance of Fast Downward's heuristic estimator, but perhaps better
heuristic accuracy can outweigh worse per-state performance in many
cases.

Third, we want to investigate in how far the performance of the
planner could be improved by encoding some domains differently. In
some cases, merging a set of state variables which are closely
interrelated into a single state variable whose domain is the product
of the domains of the original state variables might be beneficial.
Also, we want to test if hand-tailored encodings lead to better
performance than automatically derived ones, and if so, how large the
performance gap is.

Fourth and finally, we would like to evaluate the
behaviour of the causal graph heuristic in specific planning domains
both empirically and theoretically, following Hoffmann's work on the
FF heuristic \cite{joerg-topology,hoffmann:aips-02,hoffmann:jair2005}.
Hopefully, this will give some indication when we can expect good
performance from the causal graph heuristic and when it is advisable
to look for other approaches.



==> helmert06a/experiments.tex <==
\section{Experiments}
\label{section:experiments}

To evaluate the performance of Fast Downward, and specifically the
differences between the various configurations of the search
component, we have performed a number of experiments on the set of
benchmarks from the previous international planning competitions.  The
purpose of these experiments is to compare Fast Downward to the state
of the art in PDDL planning, and to contrast the performance of the
different search algorithms of Fast Downward (greedy best-first search
with and without preferred operators, multi-heuristic best-first
search with and without preferred operators, and focused
iterative-broadening search).

To clearly state the purpose of our experiments, let us also point out
two areas worthy of study that we do \emph{not} choose to investigate
here:
\begin{itemize}
\item We do not compare the causal graph heuristic to other
  heuristics, such as the FF or HSP heuristics. Such a comparison
  would require evaluating the different heuristics within otherwise
  identical planning systems. We have performed such an experiment
  before \cite{malte-icaps-cg} and thus prefer to dedicate this
  section to an evaluation of the complete Fast Downward planning
  system, rather than just its heuristic function.
\item We do not give a final answer to the question \emph{why} Fast
  Downward performs well or badly in the domains we analyse. Where we
  do observe bad performance, we try to give a plausible explanation
  for this, but we do not conduct a full-blown study of heuristic
  quality in the spirit of Hoffmann's work on the FF and $h^+$
  heuristics \cite{hoffmann:jair2005}. While we do believe that much
  could be learned from such an investigation, it is a major
  undertaking that would go beyond the scope of this article.
\end{itemize}

Our aim in this section is to evaluate the Fast Downward planner as a
whole, so there are a number of algorithmic questions which we do not
address. For example, one might wonder what (if any) speed-up can be
obtained by using successor generators over simpler methods
which test each operator for applicability whenever a node is
expanded. Another question concerns the extent to which deferred
heuristic evaluation affects search performance. To keep this section
at a reasonable length, we do not discuss either of these questions
here. However, we have conducted experiments addressing them, and
include their results in an electronic appendix to this
paper.\footnote{See \texttt{http://www.jair.org/}. The short summary
  is that successor generators speed up search by up to two orders of
  magnitude in extreme cases like the largest {\satellite} tasks, but
  have little impact on performance most of the time. Deferred heuristic
  evaluation is very beneficial in some domains, with speed-ups of more
  than one order of magnitude being common, is somewhat beneficial in
  the majority of domains, with speed-ups between 2 and 4, and is very
  rarely detrimental to performance.}

\subsection{Benchmark Set}

The benchmark set we use consists of all propositional planning tasks
from the fully automated tracks of the first four international
planning competitions hosted at AIPS 1998, AIPS 2000, AIPS 2002 and
ICAPS 2004. The set of benchmark domains is shown in
Fig.~\ref{figure:domains}. Altogether, the benchmark suite comprises
1442 tasks. (The numbers in Fig.~\ref{figure:domains} add up to 1462,
but the 20 {\satellite} instances that were introduced for IPC3 were
also part of the benchmark set of IPC4, so we only count them once.)

\includefigure{domains}{Planning domains of the first four
  international planning competitions.}

We distinguish between three classes of domains:
\begin{itemize}
\item \emph{STRIPS domains:} These domains do not feature derived
  predicates or conditional effects, and all conditions appearing in
  goal and operators are conjunctions of positive literals.
\item \emph{ADL domains:} These domains make use of conditional
  effects in their operator and/or contain more general conditions
  than simple conjunctions in their goals and operators. However, they
  do not require axioms.
\item \emph{PDDL2.2 domains:} These domains use the full range of
  propositional PDDL2.2, including those features present in ADL
  domains and axioms.
\end{itemize}

At IPC4, some domains were presented in different
\emph{formulations}, meaning that the same real-world task was encoded
in several different ways. Participants were asked to only work on one
formulation per domain, being able to choose their preferred
formulation for a given domain freely. For example, the {\airport}
domain was available in a STRIPS formulation and an ADL formulation.

However, the organizers did not strictly follow the rule of
considering different encodings of the same real-world task different
\emph{formulations}, rather than different domains proper. Namely, for
the {\psrmiddle} and {\promela} domains, encodings with and without
axioms were available, and these were considered as different domains
on the grounds that the encodings without axioms were much larger and
hence likely more difficult to solve. We apply the formulation
vs.~encoding view more strictly and thus only consider one
{\psrmiddle} domain and one domain for each of the two {\promela}
variants, {\philosophers} and {\opticaltelegraph}.

Of the IPC1 benchmark set, all tasks are solvable except for 11
{\mystery} instances. Of the IPC2 benchmark set, all tasks are
solvable except for 11 {\miconicfull} instances. All IPC3 benchmarks are
solvable. For IPC4, we have not checked all instances of the
{\pipesworldtankage} domain, but we assume that all are tasks are
solvable.

If run in any of the heuristic search modes, Fast Downward proves the
unsolvability of the unsolvable {\mystery} and {\miconicfull} tasks by
using the dead-end detection routine described in our earlier article
on the causal graph heuristic \cite{malte-icaps-cg}, or in some cases
in the {\miconicfull} domain by exhaustively searching all states with
a finite FF heuristic. Of course, if an unsolvable task is proved
unsolvable by the planner, we report this as a ``successfully solved''
instance in the experimental results.

\subsection{Experimental Setup}

As discussed in Section \ref{section:search}, there are eleven
possible configurations of Fast Downward's search component. However,
not all of them are equally reasonable. For example, if we use FF's
helpful actions, it would seem wasteful not to use the FF heuristic
estimate, since these two are calculated together. Therefore, for the
greedy best-first search setup, we exclude configurations where
FF helpful actions are always computed. For the multi-heuristic
best-first search setup, we exclude configurations where only one type
of preferred operators is considered, but not the other, since this
would seem to be a very arbitrary choice. This leaves us with six
different configurations of the planner:
\begin{enumerate}
\item \textbf{G}: Use greedy best-first search without preferred
  operators.
\item \textbf{G + P}: Use greedy best-first search with helpful
  transitions as preferred operators.
\item \textbf{G + P${}^+$}: Use greedy best-first search with helpful
  transitions as preferred operators. Use helpful actions as preferred
  operators in states with no helpful transitions.
\item \textbf{M}: Use multi-heuristic best-first search without 
  preferred operators.
\item \textbf{M + P}: Use multi-heuristic best-first search with
  helpful transitions and helpful actions as preferred operators.
\item \textbf{F}: Use focused iterative-broadening search.
\end{enumerate}

We apply each of these planner configurations to each of the 1442
benchmark tasks, using a computer with a 3.066 GHz Intel Xeon CPU ---
the same machine that was used at IPC4 --- and set a memory limit of 1
GB and a timeout of 300 seconds.

To compare Fast Downward to the state of the art, we try to solve
each benchmark with the best-performing planners from the literature.
Unfortunately, this involves some intricacies: some planners are not
publicly available, and others only cover a restricted subset of PDDL2.2.
For the main experiment, we thus partition the benchmark domains into
three sets depending on which planners are available for comparison.

\subsection{Translation and Knowledge Compilation vs.~Search}

Of course, the results we report for Fast Downward include the time
spent in all three components of the planner: translation, knowledge
compilation, and search. Therefore, in the following presentation of
results, we only consider a task solved if the \emph{total} processing
time is below 300 seconds. However, we have also investigated which
tasks can be solved with a timeout of 300 seconds for the
\emph{search} component alone, allowing the other components to use an
arbitrary amount of resources. It turns out that this only makes a
difference in five cases, most of which could have been solved in a
total time below 310 seconds (Fig.~\ref{figure:total-time-above-300}).
Only in one of these five cases, a {\satellite} instance of exorbitant
size, did search take less time than the other two phases combined.
These results show that the search component is the only time-critical
part of Fast Downward in practice. Therefore, we do not report
separate performance results for the individual components.

\includefigure{total-time-above-300}{Tasks which could be solved by
  some configuration of Fast Downward with a search timeout of 300
  seconds, but not with a total processing timeout of 300 seconds. The
  column ``preprocessing'' shows the total time for translation and
  knowledge compilation.}

\subsection{STRIPS Domains from IPC1--3}

Let us now present the results of the main experiment. We abstain from
listing runtimes for individual planning tasks due to the
prohibitively large amount of data. These are available as an
electronic appendix to this
article.\footnote{\texttt{http://www.jair.org/}} Instead, we report
the following information:
\begin{itemize}
  \item Tables showing the number of tasks \emph{not solved} by each
    planner within the 300 second timeout. Here, we present individual
    results for each domain.
  \item Graphs showing the number of tasks solved in a given time by
    each planner. Here, we do not present separate results for each
    domain, as this would require too many graphs.
\end{itemize}

We do not discuss plan lengths; our observations in this regard are
similar to those made for the original implementation of the causal
graph heuristic \cite{malte-icaps-cg}.

\psfrag{diagonallydownward}[r][r]{\tiny \textsf{\textbf{FDD} (Fast Downward)}}
\psfrag{downward}[r][r]{\tiny \textsf{\textbf{FD} (Fast Downward)}}
\psfrag{yahsp}[r][r]{\tiny \textsf{YAHSP}}
\psfrag{macro-ff}[r][r]{\tiny \textsf{Macro-FF}}
\psfrag{sgplan}[r][r]{\tiny \textsf{SGPlan}}
\psfrag{lpg-td}[r][r]{\tiny \textsf{LPG-TD}}

\psfrag{CG}[r][r]{\tiny \textsf{CG}}
\psfrag{FF}[r][r]{\tiny \textsf{FF}}
\psfrag{LPG}[r][r]{\tiny \textsf{LPG}}
\psfrag{Any}[r][r]{\tiny \textsf{\textbf{Any} (Fast Downward)}}
\psfrag{G+P+}[r][r]{\tiny \textsf{\textbf{G + P${}^+$} (Fast Downward)}}
\psfrag{G+P}[r][r]{\tiny \textsf{\textbf{G + P} (Fast Downward)}}
\psfrag{G}[r][r]{\tiny \textsf{\textbf{G} (Fast Downward)}}
\psfrag{M+P}[r][r]{\tiny \textsf{\textbf{M + P} (Fast Downward)}}
\psfrag{M}[r][r]{\tiny \textsf{\textbf{M} (Fast Downward)}}
\psfrag{F}[r][r]{\tiny \textsf{\textbf{F} (Fast Downward)}}

\includefigure[htbp]{experiments1-unsolved}{Number of unsolved tasks for the
  STRIPS domains from IPC1, IPC2, and IPC3.}

\includegraph[p]{experiment1a-graph}{Number of tasks solved
  vs.~runtime for the STRIPS domains from IPC1, IPC2 and IPC3. This
  graph shows the results for the various configurations of Fast
  Downward.}

\includegraph[p]{experiment1b-graph}{Number of tasks solved
  vs.~runtime for the STRIPS domains from IPC1, IPC2 and IPC3. This
  graph shows the results for CG, FF and LPG and the hypothetical
  ``Any'' planner which always chooses the best configuration of Fast
  Downward. The result for greedy best-first search with helpful
  transitions is repeated for ease of comparison with
  Fig.~\ref{figure:experiment1a-graph}.}

Fig.~\ref{figure:experiments1-unsolved} shows the number of unsolved
tasks for each of the STRIPS domains from IPC1--3.
Figs.~\ref{figure:experiment1a-graph} and
\ref{figure:experiment1b-graph} show the number of tasks solved by
each planner within a given time bound between 0 and 300 seconds.
In addition to the six configurations of Fast Downward under
consideration, the table includes four other columns.

Under the heading ``Any'', we include results for a hypothetical
meta-planner that guesses the best of the six configuration of Fast
Downward for each input task and then executes Fast Downward with this
setting. Under the heading ``CG'', we report the results for our first
implementation of the causal graph heuristic
\cite{malte-icaps-cg}.\footnote{Apart from missing support for ADL and
  axioms, CG is very similar to Fast Downward using greedy best-first
  search and no preferred operators (configuration \textbf{G}). The
  translation and knowledge compilation components are essentially
  identical. The older search component mainly differs from Fast
  Downward in that it does not use deferred heuristic evaluation.}
Finally, ``FF'' and ``LPG'' refer to the well-known planners
\cite{ff,lpg} which won the fully-automated tracks of IPC2 and IPC3.
They were chosen for comparison on this benchmark set because they
showed the best performance by far of all publicly available planners
we experimented with. For LPG, which uses a randomized search
strategy, we attempted to solve each task five times and report the
median result.

The results show excellent performance of Fast Downward on this set of
benchmarks. Compared to CG, which was already shown to solve more
tasks than FF and LPG on this benchmark set \cite{malte-icaps-cg}, we
get another slight improvement for half of the planner configurations.
One of the configurations, multi-heuristic best-first search
using preferred operators, solves all benchmarks in all domains except
{\depot} and {\freecell}. Even more importantly, the number of tasks
not solved by any of the Fast Downward configurations is as small as 10.
Note that the planning competitions typically allowed a planner to
spend 30 minutes on each task; under these time constraints, we could
allocate five minutes to each of the six configurations of Fast
Downward, getting results which are at least as good as those reported
for the ``Any'' planner. Results might even be better under a cleverer
allocation scheme.

Even the configuration using focused iterative-broadening search
performs comparatively well on these benchmarks, although it cannot
compete with the other planners. Not surprisingly, this version of the
planner has difficulties in domains with many dead ends
(\freecell, \mystery, \mysteryprime) or where goal ordering is very
important (\blocksworld, \depot). It also fares comparatively badly in
domains with very large instances, namely {\logistics} (IPC1) and
\satellite. The reader should keep in mind that FF and LPG are
excellent planning systems; of all the other planners we experimented
with, including all those that were awarded prizes at the first three
planning competitions, none solved more benchmarks from this group
than focused iterative-broadening search.

The one domain that proves quite resistant to Fast Downward's solution
attempts in any configuration is {\depot}. As we already observed in
the initial experiments with the causal graph heuristic
\cite{malte-icaps-cg}, we believe that one key problem here is that
Fast Downward, unlike FF, does not use any goal ordering techniques,
which are very important in this domain. The fact that the domain
includes a \blocksworld-like subproblem is also problematic, as it
gives rise to very dense causal graphs as we demonstrated in Section
\ref{section:causal-graph-examples}.

\subsection{ADL Domains from IPC1--3}

Second, we present results for the ADL domains of the first three
planning competitions. This is a much smaller group than the previous,
including only four domains. This time, we cannot consider CG or LPG,
since neither CG nor the publicly available version of LPG supports
ADL domains. Therefore, we compare to FF exclusively. Again, we report
the number of unsolved tasks in each domain
(Fig.~\ref{figure:experiments2-unsolved}) and present graphs showing
how quickly the tasks are solved
(Figs.~\ref{figure:experiment2a-graph} and
\ref{figure:experiment2b-graph}).

\includefigure[htbp]{experiments2-unsolved}{Number of unsolved tasks for the
  ADL domains from IPC1, IPC2 and IPC3.}

\includegraph[p]{experiment2a-graph}{Number of tasks solved
  vs.~runtime for the ADL domains from IPC1, IPC2 and IPC3. This
  graph shows the results for the various configurations of Fast
  Downward.}

\includegraph[p]{experiment2b-graph}{Number of tasks solved
  vs.~runtime for the ADL domains from IPC1, IPC2 and IPC3. This
  graph shows the results for FF and the hypothetical
  ``Any'' planner which always chooses the best configuration of Fast
  Downward. The result for multi-heuristic best-first search with
  preferred operators is repeated for ease of comparison with
  Fig.~\ref{figure:experiment2a-graph}.}

These results do not look as good as for the first group of domains.
Results in both {\miconic} domains are good, even improving on those
of FF. However, greedy best-first search performs very badly in the
{\assembly} domain, and all configurations perform badly in the
{\schedule} domain. Currently, we have no good explanation for the
{\assembly} behaviour. For the {\schedule} domain, the weak performance
again seems to be related to missing goal ordering techniques: In many
{\schedule} tasks, several goals are defined for the same object which
can only be satisfied in a certain order. For instance, for objects
that should be cylindrical, polished and painted, these three goals
must be satisfied in precisely this order: making an object
cylindrical reverts the effects of polishing and painting, and
polishing reverts the effect of painting. Not recognising these
constraints, the heuristic search algorithm assumes to be close to the
goal when an object is already polished and painted but not
cylindrical, and is loathe to transform the object into cylindrical
shape because this would undo the already achieved goals. With some
rudimentary manual goal ordering, ignoring painting goals until all
other goals have been satisfied, the number of tasks not solved by
multi-heuristic best-first search with preferred operators drops from
28 to 3. These three failures appear to be due to the remaining ordering
problems with regard to cylindrical and polished objects.

\subsection{Domains from IPC4}

Third and finally, we present results for the IPC4 domains. Here, we
do not compare to FF: for these benchmarks, FF does not perform as
well as the best planners from the competition. Besides, several of
the IPC4 competitors are extensions of FF or hybrids using FF as part
of a bigger system, so FF-based planning is well-represented even if
we limit our attention to the IPC4 planners. For this comparison, we
chose the four most successful competition participants besides Fast
Downward, namely LPG-TD, SGPlan, Macro-FF and YAHSP \cite<cf.~the
results in>{ipc4}.
Similar to the previous two experiments, we report the number of
unsolved tasks in each domain
(Fig.~\ref{figure:experiments3-unsolved}) and present graphs showing
how quickly the tasks are solved
(Figs.~\ref{figure:experiment3a-graph} and
\ref{figure:experiment3b-graph}).

\includefigure[htbp]{experiments3-unsolved}{Number of unsolved tasks for the
  IPC4 domains. Results for the various configurations of Fast Downward
  are listed in the upper part, results for the competition
  participants in the lower part. ``FD'' and ``FDD'' denote the
  versions of Fast Downward that participated in IPC4 under the names
  ``Fast Downward'' and ``Fast Diagonally Downward''
  (cf.~Section~\ref{section:search}).}

\includegraph[p]{experiment3a-graph}{Number of tasks solved
  vs.~runtime for the IPC4 domains. This graph shows the results for
  the various configurations of Fast Downward.}

\includegraph[p]{experiment3b-graph}{Number of tasks solved
  vs.~runtime for the IPC4 domains. This graph shows the results for
  the hypothetical ``Any'' planner which always chooses the best
  configuration of Fast Downward, the competition configurations of
  Fast Downward and the best four other participants.}

Fast Downward is competitive with the other planners across domains,
and better than all others in some. The {\pipesworld} domains are the
only ones in which any of the other planners is noticeably better than the two
competition versions of Fast Downward. This is the case for YAHSP in
both {\pipesworld} domain variants and for SGPlan in {\pipesworldnotankage}.
The {\pipesworld} domain is not very hierarchical in nature; this
might be a domain where the decomposition approach of the causal graph
heuristic is not very appropriate. The results of the heuristic search
configurations in the {\opticaltelegraph} domain are extremely bad and
require further investigation.

Interestingly, focused iterative-broadening search performs very well
on some of the benchmarks from this suite. One of the reasons for this
is that in many of the tasks of the IPC4 suite, there are many
individual goals which are easy to serialize and can be
solved mostly independently.\footnote{We have devised an experiment
  which shows that if this property is artificially violated by a
  simple goal reformulation, the performance of the algorithm degrades
  quickly; see the electronic appendix for details.}  Comparing the
configuration \textbf{G} to \textbf{G + P${}^+$} and especially
\textbf{M} to \textbf{M + P}, we also observe that using preferred
operators is very useful for these benchmarks, even more so than in
the two previous experiments.

As a final remark, we observe that if we implemented the ``Any''
meta-planner by calling the six Fast Downward configurations in a
round-robin fashion, we would obtain a planning system that could
solve all but 54 of the IPC4 benchmarks within a $6 \cdot 5 = 30$
minute timeout. This is almost on par with the top performer of IPC4,
Fast Diagonally Downward, which solved all but 52 of the IPC4
benchmarks under the same timeout. Thus, this is a benchmark set for
which exploring different planner configurations definitely pays off.

\subsection{Conclusions from the Experiment}

How can we interpret these experimental results? Our first conclusion is
that Fast Downward is clearly competitive with the state of the art.
This is especially true for the configuration using multi-heuristic
best-first search with preferred operators (\textbf{M+P}), which
outperforms all competing planning systems both on the set of STRIPS
domains from IPC1--3 and on the domains from IPC4. If it were not for
the problems in the {\schedule} domain, the same would be true for the
remaining group of benchmarks, the ADL domains from IPC1--3.

With regard to the second objective of the investigation, evaluating
the relative strengths of the different planner configurations, the
\textbf{M+P} configuration emerges as a clear-cut winner. In 23 out of
29 domains, no other configuration solves more tasks, and unlike the
other configurations, there is only one domain (\opticaltelegraph) in
which it performs very badly. We conclude that both multi-heuristic
best-first search and the use of preferred operators are promising
extensions to heuristic planners.

This is particularly true for preferred operators. Indeed, after the
\textbf{M+P} configuration, the two variants of greedy best-first
search with preferred operators show the next best overall
performance, both in terms of the number of domains where they are among
the top performers and in terms of the total number of tasks solved.
Comparing \textbf{G} to \textbf{G+P}, there are ten domains in which
the variant using preferred operators solves more tasks than the one
not using them; the opposite is true in five domains. Comparing
\textbf{M} to \textbf{M+P}, the difference is even more striking, with
the preferred operator variant outperforming the other in fifteen
domains, while being worse in two (in both of which it only solves one
task less).  These are convincing arguments for the use of preferred
operators.


==> helmert06a/figures/compute-all-costs.tex <==
\framebox{
  \parbox{14.8cm}{
    \begin{algorithm}
      \hspace*{0cm}\textbf{algorithm} compute-costs-bottom-up($\Pi$, $s$): \\
      \hspace*{1cm}\textbf{for each} variable $v$ of $\Pi$,
        traversing the pruned causal graph in bottom-up order: \\
      \hspace*{2cm}Let $\mathcal V'$ be the set of immediate
        predecessors of $v$ in the pruned causal graph. \\
      \hspace*{2cm}\textbf{for each} pair of values $(d, d') \in
        \mathcal D_v \times \mathcal D_v$: \\
      \hspace*{3cm}Generate a planning task $\Pi_{v,d,d'}$ with the
        following components: \\
      \hspace*{3cm}\quad--- \emph{Variables:} $\mathcal V' \cup \{v\}$. \\
      \hspace*{3cm}\quad--- \emph{Initial state:}
        $v=d$ and $v'=s(v')$ for all $v' \in \mathcal V'$. \\
      \hspace*{3cm}\quad--- \emph{Goal:}
        $v=d'$. \\
      \hspace*{3cm}\quad--- \emph{Axioms and operators:} \\
      \hspace*{3cm}\quad\phantom{---} %
	1. Those corresponding to transitions in the pruned DTG
	of $v$. \\
      \hspace*{3cm}\quad\phantom{---} %
	2. For all variables $v' \in \mathcal V'$ and values
	$e, e' \in \mathcal D_{v'}$, an operator \\
      \hspace*{3cm}\quad\phantom{--- 2.} %
	 with precondition $v'=e$, effect $v'=e'$ and cost
	 $\textit{cost}_v'(e,e')$. \\
      \hspace*{3cm}\quad\phantom{--- 2.} %
      \{ Note that all variables $v' \in \mathcal V'$
        have been considered previously, \\
      \hspace*{3cm}\quad\phantom{--- 2. \{} %
	so that their cost values are known. \} \\
      \hspace*{3cm}Set $\textit{cost}_{v}(d,d')$ to the cost of a plan
        $\pi$ that solves $\Pi_{v,d,d'}$.
    \end{algorithm}
  }
}


==> helmert06a/figures/compute-costs.tex <==
\framebox{
  \parbox{14.8cm}{
    \begin{algorithm}
      \hspace*{0cm}\textbf{algorithm} compute-costs($\Pi$, $s$, $v$, $d$): \\
      \hspace*{1cm}Let $\mathcal V'$ be the set of immediate
        predecessors of $v$ in the pruned causal graph of $\Pi$. \\
      \hspace*{1cm}Let $\mathit{DTG}$ be the
        pruned domain transition graph of $v$. \\
      \hspace*{1cm}$\textit{cost}_v(d,d) := 0$ \\
      \hspace*{1cm}$\textit{cost}_v(d,d') := \infty$ for all $d' \in
        \mathcal D_v \setminus \{d\}$ \\
      \hspace*{1cm}$\textit{local-state}_d := s$ restricted to
        $\mathcal V'$ \\
      \hspace*{1cm}$\textit{unreached} := \mathcal D_v$ \\
      \hspace*{1cm}\textbf{while} \textit{unreached} contains a value
        $d' \in \mathcal D_v$ with $\textit{cost}_v(d,d') < \infty$: \\
      \hspace*{2cm}Choose such a value $d' \in \textit{unreached}$
        minimizing $\textit{cost}_v(d,d')$. \\
      \hspace*{2cm}$\textit{unreached} := \textit{unreached}
        \setminus \{d'\}$ \\
      \hspace*{2cm}\textbf{for each} transition $t$ in $\textit{DTG}$
        leading from $d'$ to some $d'' \in \textit{unreached}$: \\
      \hspace*{3cm}$\textit{transition-cost} := 0$ if $v$ is a
        derived variable; $1$ if $v$ is a fluent \\
      \hspace*{3cm}\textbf{for each} pair $v'=e'$ in the condition of
        $t$: \\
      \hspace*{4cm}$e := \textit{local-state}_{d'}(v')$ \\
      \hspace*{4cm}\textbf{call} $\textrm{compute-costs}(\Pi, s, v',
        e)$. \\
      \hspace*{4cm}$\textit{transition-cost} :=
        \textit{transition-cost} + \textit{cost}_{v'}(e, e')$ \\
      \hspace*{3cm}\textbf{if} $\textit{cost}_v(d, d') +
        \textit{transition-cost} < \textit{cost}_v(d,d'')$: \\
      \hspace*{4cm}$\textit{cost}_v(d,d'') := \textit{cost}_v(d,d') +
        \textit{transition-cost}$ \\
      \hspace*{4cm}$\textit{local-state}_{d''} :=
        \textit{local-state}_{d'}$ \\
      \hspace*{4cm}\textbf{for each} pair $v'=e'$ in the condition of
        $t$: \\
      \hspace*{5cm}$\textit{local-state}_{d''}(v') := e'$
    \end{algorithm}
  }
}


==> helmert06a/figures/domains.tex <==
%\framebox{
    \newcommand{\heading}[1]{%
      \multicolumn{1}{c}{\textbf{#1}}}
    \begin{tabular}{llcr}
    \heading{Competition}
    & \heading{Domain}
    & \heading{Class}
    & \heading{Number of tasks} \\[6pt]
    IPC1 (AIPS 1998) & \assembly & ADL & 30 \\
    & \grid & STRIPS & 5 \\
    & \gripper & STRIPS & 20 \\
    & \logistics & STRIPS & 35 \\
    & \movie & STRIPS & 30 \\
    & \mystery & STRIPS & 30 \\
    & \mysteryprime & STRIPS & 35 \\[6pt]
    IPC2 (AIPS 2000) & \blocksworld & STRIPS & 35 \\
    & \freecell & STRIPS & 60 \\
    & \logistics & STRIPS & 28 \\
    & \miconicstrips & STRIPS & 150 \\
    & \miconicsimple & ADL & 150 \\
    & \miconicfull & ADL & 150 \\
    & \schedule & ADL & 150 \\[6pt]
    IPC3 (AIPS 2002) & \depot & STRIPS & 22 \\
    & \driverlog & STRIPS & 20 \\
    & \freecell & STRIPS & 20 \\
    & \rovers & STRIPS & 20 \\
    & \satellite & STRIPS & 20 \\
    & \zenotravel & STRIPS & 20 \\[6pt]
    IPC4 (ICAPS 2004) & \airport & STRIPS & 50 \\
    & \opticaltelegraph & PDDL2.2 & 48 \\
    & \philosophers & PDDL2.2 & 48 \\
    & \pipesworldnotankage & STRIPS & 50 \\
    & \pipesworldtankage & STRIPS & 50 \\
    & \psrsmall & STRIPS & 50 \\
    & \psrmiddle & PDDL2.2 & 50 \\
    & \psrlarge & PDDL2.2 & 50 \\
    & \satellite & STRIPS & 36
    \end{tabular}
%}


==> helmert06a/figures/evaluate-axioms-efficiently.tex <==
\framebox{
  \parbox{14.8cm}{
    \begin{algorithm}
      \hspace*{0cm}\textbf{algorithm} evaluate-axiom-layer($s$, $\mathcal A_i$): \\
      \hspace*{1cm}\textbf{for each} axiom $a \in \mathcal A_i$: \\
      \hspace*{2cm}$a\textrm{.counter} := |a\textrm{.cond}|$ \\
      \hspace*{1cm}\textbf{for each} variable $v$: \\
      \hspace*{2cm}\textbf{for each} axiom $a \in \mathcal A_i$ with a
        condition $v = s(v)$ in the body: \\
      \hspace*{3cm}$a\textrm{.counter} := a\textrm{.counter} - 1$ \\
      \hspace*{1cm}\textbf{while} there exists an axiom $a \in
        \mathcal A_i$ with $a\textrm{.counter} = 0$ that was not yet considered: \\
      \hspace*{2cm}Let $\langle v, d\rangle$ be the head of such an axiom. \\
      \hspace*{2cm}\textbf{if} $s(v) \neq d$: \\
      \hspace*{3cm}$s(v) := d$ \\
      \hspace*{3cm}\textbf{for each} axiom $a \in \mathcal A_i$ with a
        condition $v = d$ in the body: \\
      \hspace*{4cm}$a\textrm{.counter} := a\textrm{.counter} - 1$
  \end{algorithm}
  }
}



==> helmert06a/figures/experiments1-unsolved.tex <==
%\framebox{
    \newcommand{\heading}[1]{%
      \multicolumn{1}{c}{\makebox[0.6cm]{\textbf{#1}}}}
    \newcommand{\headingrule}[1]{%
      \multicolumn{1}{c|}{\makebox[0.6cm]{\textbf{#1}}}}
    \begin{tabular}{lr|cccccc|c|ccc}
      \heading{Domain}
    & \multicolumn{1}{c|}{\textbf{\#Tasks}}
    & \heading{G}
    & \heading{G+P}
    & \heading{G+P${}^+$}
    & \heading{M}
    & \heading{M+P}
    & \headingrule{F}
    & \headingrule{Any}
    & \heading{CG}
    & \heading{FF}
    & \heading{LPG} \\[6pt]
    \blocksworld & 35
      & 0 & 0 & 0 & 0 & 0 & 17 & 0 & 0 & 4 & 0 \\
    \depot & 22
      & 12 & 13 & 13 & 12 & 8 & 11 & 7 & 14 & 3 & 0 \\
    \driverlog & 20
      & 2 & 0 & 0 & 1 & 0 & 1 & 0 & 3 & 5 & 0 \\
    {\freecell} (IPC2) & 60
      & 4 & 4 & 12 & 11 & 12 & 40 & 3 & 2 & 3 & 55 \\
    {\freecell} (IPC3) & 20
      & 0 & 0 & 5 & 1 & 2 & 14 & 0 & 0 & 2 & 19 \\
    \grid & 5
      & 1 & 2 & 1 & 1 & 0 & 4 & 0 & 1 & 0 & 1 \\
    \gripper & 20
      & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    {\logistics} (IPC1) & 35
      & 1 & 0 & 0 & 4 & 0 & 26 & 0 & 0 & 0 & 4 \\
    {\logistics} (IPC2) & 28
      & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    \miconicstrips & 150
      & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    \movie & 30
      & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    \mystery & 30
      & 1 & 2 & 1 & 0 & 0 & 13 & 0 & 1 & 12 & 15 \\
    \mysteryprime & 35
      & 0 & 0 & 0 & 2 & 0 & 14 & 0 & 1 & 3 & 7 \\
    \rovers & 20
      & 2 & 0 & 0 & 0 & 0 & 2 & 0 & 3 & 0 & 0 \\
    {\satellite} (IPC3) & 20
      & 1 & 0 & 0 & 0 & 0 & 6 & 0 & 0 & 0 & 0 \\
    \zenotravel & 20
      & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\[6pt]
    \textbf{Total} & 550
      & 24 & 21 & 32 & 32 & 22 & 148 & 10 & 25 & 32 & 101
    \end{tabular}
%}


==> helmert06a/figures/experiments2-unsolved.tex <==
%\framebox{
    \newcommand{\heading}[1]{%
      \multicolumn{1}{c}{\makebox[0.6cm]{\textbf{#1}}}}
    \newcommand{\headingrule}[1]{%
      \multicolumn{1}{c|}{\makebox[0.6cm]{\textbf{#1}}}}
    \begin{tabular}{lr|cccccc|c|c}
      \heading{Domain}
    & \multicolumn{1}{c|}{\textbf{\#Tasks}}
    & \heading{G}
    & \heading{G+P}
    & \heading{G+P${}^+$}
    & \heading{M}
    & \heading{M+P}
    & \headingrule{F}
    & \headingrule{Any}
    & \heading{FF} \\[6pt]
    \assembly & 30 &
      28 & 27 & 25 & 3 & 0 & 30 & 0 & 0 \\
    \miconicsimple & 150 & 
      0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    \miconicfull & 150 &
      9 & 8 & 9 & 9 & 8 & 90 & 6 & 12 \\
    \schedule & 150 &
      134 & 93 & 93 & 132 & 28 & 113 & 25 & 0 \\
    \textbf{Total} & 480
      & 171 & 128 & 127 & 144 & 36 & 233 & 31 & 12
    \end{tabular}
%}


==> helmert06a/figures/experiments3-unsolved.tex <==
%\framebox{
    \newcommand{\heading}[1]{%
      \multicolumn{1}{c}{\makebox[0.6cm]{\textbf{#1}}}}
    \newcommand{\headingrule}[1]{%
      \multicolumn{1}{c|}{\makebox[0.6cm]{\textbf{#1}}}}
    \begin{tabular}{lr|cccccc|c}
      \heading{Domain}
    & \multicolumn{1}{c|}{\textbf{\#Tasks}}
    & \heading{G}
    & \heading{G+P}
    & \heading{G+P${}^+$}
    & \heading{M}
    & \heading{M+P}
    & \headingrule{F}
    & \heading{Any} \\[6pt]
    \airport & 50
      & 28 & 30 & 17 & 18 & 14 &  0 &  0 \\
    \pipesworldnotankage & 50
      & 24 & 25 & 23 & 14 &  7 & 10 &  7 \\
    \pipesworldtankage & 50
      & 36 & 36 & 36 & 34 & 17 & 34 & 14 \\
    \opticaltelegraph & 48
      & 48 & 47 & 48 & 47 & 46 & 13 & 13 \\
    \philosophers & 48
      &  0 &  0 &  0 & 16 &  0 & 21 &  0 \\
    \psrsmall & 50
      &  0 &  0 &  0 &  0 &  0 &  1 &  0 \\
    \psrmiddle & 50
      &  0 &  0 &  0 &  0 &  0 & 22 &  0 \\
    \psrlarge & 50
      & 22 & 20 & 22 & 23 & 22 & 39 & 20 \\
    {\satellite} (IPC4) & 36
      &  8 &  0 &  0 &  8 &  3 & 22 &  0 \\
    \textbf{Total} & 432
      &166 &158 &146 &160 & 109&162 & 54
    \end{tabular}

    \bigskip

    \renewcommand{\heading}[1]{%
      \multicolumn{1}{c}{\textbf{#1}}}
    \renewcommand{\headingrule}[1]{%
      \multicolumn{1}{c|}{\textbf{#1}}}
    \begin{tabular}{l|cc|cccc}
      \headingrule{Domain}
    & \heading{FD}
    & \headingrule{FDD}
    & \heading{LPG-TD}
    & \heading{Macro-FF}
    & \heading{SGPlan}
    & \heading{YAHSP} \\[6pt]
    \airport
      &  0 &  0 &  7 & 30 &  6 & 17 \\
    \pipesworldnotankage
      & 11 &  7 & 10 & 12 &  0 &  0 \\
    \pipesworldtankage
      & 34 & 19 & 29 & 29 & 20 & 13 \\
    \opticaltelegraph
      & 22 & 22 & 37 & 31 & 29 & 36 \\
    \philosophers
      &  0 &  0 &  1 & 36 &  0 & 19 \\
    \psrsmall
      &  0 &  0 &  2 & 50 &  6 &  3 \\
    \psrmiddle
      &  0 &  0 &  0 & 19 &  4 & 50 \\
    \psrlarge
      & 22 & 22 & 50 & 50 & 39 & 50 \\
    {\satellite} (IPC4)
      &  0 &  3 &  1 &  0 &  6 &  0 \\
    \textbf{Total}
      & 89 & 73 &137 & 257&110 &188
    \end{tabular}
%}


==> helmert06a/figures/initial-example-sas.tex <==
\newcommand{\operator}[3]{%
  \textrm{Operator} #1\textrm{:} \\
  \phantom{XX}\textrm{PRE:} #2%
  \phantom{XX}\textrm{EFF:} #3 \par
}

\framebox{
  \parbox{14cm}{
    \begin{ttfamily}
      \textrm{Variables:} \\
      \phantom{XX}p1\textrm{,} p2 $\in$ \{at-a\textrm{,} at-b\textrm{,} at-c\textrm{,} at-d\textrm{,} at-e\textrm{,} at-f\textrm{,}
          at-g\textrm{,} \\
      \phantom{XXXXXXXXXX\textrm{,}\{}in-c1\textrm{,} in-c2\textrm{,} in-c3\textrm{,} in-t\} \\
      \phantom{XX}c1\textrm{,} c2 $\in$ \{at-a\textrm{,} at-b\textrm{,} at-c\textrm{,} at-d\} \\
      \phantom{XX}c3\phantom{XXX\textrm{,}} $\in$ \{at-e\textrm{,} at-f\textrm{,} at-g\} \\
      \phantom{XX}t\phantom{XXXX\textrm{,}} $\in$ \{at-d\textrm{,} at-e\}

      \textrm{Init:} \\
      \phantom{XX}p1 = at-c\textrm{,} p2 = at-f \\
      \phantom{XX}c1 = at-a\textrm{,} c2 = at-b\textrm{,} c3 = at-g\textrm{,} t = at-e

      \textrm{Goal:} \\
      \phantom{XX}p1 = at-g\textrm{,} p2 = at-e

      \operator{drive-c1-a-d}{c1 = at-a}{c1 = at-d}
      \operator{drive-c1-b-d}{c1 = at-b}{c1 = at-d}
      \operator{drive-c1-c-d}{c1 = at-c}{c1 = at-d}
      \dots \\
      \operator{load-c1-p1-a}{c1 = at-a\textrm{,} p1 = at-a}{p1 = in-c1}
      \operator{load-c1-p1-b}{c1 = at-b\textrm{,} p1 = at-b}{p1 = in-c1}
      \operator{load-c1-p1-c}{c1 = at-c\textrm{,} p1 = at-c}{p1 = in-c1}
      \dots \\
      \operator{unload-c1-p1-a}{c1 = at-a\textrm{,} p1 = in-c1}{p1 = at-a}
      \operator{unload-c1-p1-b}{c1 = at-b\textrm{,} p1 = in-c1}{p1 = at-b}
      \operator{unload-c1-p1-c}{c1 = at-c\textrm{,} p1 = in-c1}{p1 = at-c}
      \dots
    \end{ttfamily}
  }
}

==> helmert06a/figures/initial-example-strips.tex <==
\newcommand{\operator}[4]{%
  \textrm{Operator} #1\textrm{:} \\
   \phantom{XX}\textrm{PRE:} #2%
   \phantom{XX}\textrm{ADD:} #3%
   \phantom{XX}\textrm{DEL:} #4 \par
}

\framebox{
  \parbox{14cm}{
    \begin{ttfamily}
      \textrm{Variables:} \\
      \phantom{XX}at-p1-a\textrm{,} at-p1-b\textrm{,} at-p1-c\textrm{,} at-p1-d\textrm{,}
        at-p1-e\textrm{,} at-p1-f\textrm{,} at-p1-g\textrm{,} \\
      \phantom{XX}at-p2-a\textrm{,} at-p2-b\textrm{,} at-p2-c\textrm{,} at-p2-d\textrm{,}
        at-p2-e\textrm{,} at-p2-f\textrm{,} at-p2-g\textrm{,} \\
      \phantom{XX}at-c1-a\textrm{,} at-c1-b\textrm{,} at-c1-c\textrm{,} at-c1-d\textrm{,} \\
      \phantom{XX}at-c2-a\textrm{,} at-c2-b\textrm{,} at-c2-c\textrm{,} at-c2-d\textrm{,} \\
      \phantom{XX}at-c3-e\textrm{,} at-c3-f\textrm{,} at-c3-g\textrm{,} \\
      \phantom{XX}at-t-d\textrm{,} at-t-e\textrm{,} \\
      \phantom{XX}in-p1-c1\textrm{,} in-p1-c2\textrm{,} in-p1-c3\textrm{,} in-p1-t\textrm{,} \\
      \phantom{XX}in-p2-c1\textrm{,} in-p2-c2\textrm{,} in-p2-c3\textrm{,} in-p2-t

      \textrm{Init:} \\
      \phantom{XX}at-p1-c\textrm{,} at-p2-f\textrm{,} at-c1-a\textrm{,} at-c2-b\textrm{,} at-c3-g\textrm{,} at-t-e

      \textrm{Goal:} \\
      \phantom{XX}at-p1-g\textrm{,} at-p2-e

      \operator{drive-c1-a-d}{at-c1-a}{at-c1-d}{at-c1-a}
      \operator{drive-c1-b-d}{at-c1-b}{at-c1-d}{at-c1-b}
      \operator{drive-c1-c-d}{at-c1-c}{at-c1-d}{at-c1-c}
      \dots \\
      \operator{load-c1-p1-a}{at-c1-a\textrm{,} at-p1-a}{in-p1-c1}{at-p1-a}
      \operator{load-c1-p1-b}{at-c1-b\textrm{,} at-p1-b}{in-p1-c1}{at-p1-b}
      \operator{load-c1-p1-c}{at-c1-c\textrm{,} at-p1-c}{in-p1-c1}{at-p1-c}
      \dots \\
      \operator{unload-c1-p1-a}{at-c1-a\textrm{,} in-p1-c1}{at-p1-a}{in-p1-c1}
      \operator{unload-c1-p1-b}{at-c1-b\textrm{,} in-p1-c1}{at-p1-b}{in-p1-c1}
      \operator{unload-c1-p1-c}{at-c1-c\textrm{,} in-p1-c1}{at-p1-c}{in-p1-c1}
      \dots
    \end{ttfamily}
  }
}


==> helmert06a/figures/planning-algorithm-easy-task.tex <==
\framebox{
  \parbox{14.8cm}{
    \begin{algorithm}
      \hspace*{0cm}\textbf{algorithm} solve-easy-MPT($\mathcal V$,
      $s_0$, $s_\star$, $\mathcal O$): \\
      \hspace*{1cm}\textbf{if} $s_\star = \emptyset$: \\
      \hspace*{2cm}\{ The goal is empty: the empty plan is a solution.
         \} \\
      \hspace*{2cm}\textbf{return} $\langle\rangle$. \\
      \hspace*{1cm}\textbf{else}: \\
      \hspace*{2cm}Let $v \in \mathcal V$ be a variable not
	occurring in preconditions or effect conditions in $\mathcal O$. \\
      \hspace*{2cm}\{ Such a variable always exists if
        the causal graph of the task is acyclic. \} \\
      \hspace*{2cm}$\mathcal V' := \mathcal V \setminus \{v\}$. \\
      \hspace*{2cm}$\mathcal O' := \{~o \in \mathcal O~|~o \text{~does
        not affect~} v~\}$. \\
      \hspace*{2cm}$\textit{plan} := \langle \rangle$ \\
      \hspace*{2cm}\textbf{if} $s_\star(v)$ is defined: \\
      \hspace*{3cm}Let $t_1$, $\dots$, $t_k$ be a path of
        transitions in $\textit{DTG}(v)$ from $s_0(v)$ to
	$s_\star(v)$. \\
      \hspace*{3cm}\{ $t_1$, $\dots$, $t_k$ is a ``high-level plan''
        that reaches the goal for $v$, \\
      \hspace*{3cm}\phantom{\{ }but ignores preconditions
        on other variables. \} \\
      \hspace*{3cm}\textbf{for each} $t \in \{t_1, \dots, t_k\}$: \\
      \hspace*{4cm}\{ Recursively find a plan that achieves the
        conditions of $t$. \} \\
      \hspace*{4cm}Let $\cond$ and $o$ be the condition and operator
        associated with $t$. \\
      \hspace*{4cm}Let $s_0'$ be the state reached after executing
        $\textit{plan}$, restricted to $\mathcal V'$. \\
      \hspace*{4cm}Extend $\textit{plan}$ by $\textrm{solve-easy-MPT}(\mathcal V',
  	s'_0, \cond, \mathcal O')$. \\
      \hspace*{4cm}Extend $\textit{plan}$ by $o$. \\
      \hspace*{2cm}\{ After dealing with $v$, recursively
        plan for goals on the remaining variables. \} \\
      \hspace*{2cm}Let $s_0'$ be the state reached after executing
        $\textit{plan}$, restricted to $\mathcal V'$. \\
      \hspace*{2cm}$s'_\star := s_\star$ restricted to
        $\mathcal V'$. \\
      \hspace*{2cm}Extend $\textit{plan}$ by
        $\textrm{solve-easy-MPT}(\mathcal V', s'_0, s'_\star, \mathcal
        O')$. \\
      \hspace*{2cm}\textbf{return} $\textit{plan}$
    \end{algorithm}
  }
}


==> helmert06a/figures/reach-one-goal-complete.tex <==
\framebox{
  \parbox{14.8cm}{
    \begin{algorithm}
      \hspace*{0cm}\textbf{algorithm}
        reach-one-goal($\Pi$, $v$, $d$, $\cond$): \\
      \hspace*{1cm}\textbf{for each} $\vartheta \in
        \{0, 1, \dots, \textit{max-threshold}\}$: \\
      \hspace*{2cm}Let $\mathcal O_\vartheta$ be the set of operators of
        $\Pi$ whose modification distance with respect to $v$ \\
      \hspace*{2cm}\quad is at most $\vartheta$
        and which do not affect any state
        variable occurring in $\cond$. \\
      \hspace*{2cm}Assign the cost $c$ to each operator $o \in
        \mathcal O_\vartheta$ with modification distance $c$ with \\
      \hspace*{2cm}\quad respect to $v$. \\
      \hspace*{2cm}Call the \emph{uniform-cost-search} algorithm with
        a closed list, using the operator set $O_\vartheta$, \\
      \hspace*{2cm}\quad to find a state satisfying $\{v = d\} \cup \cond$. \\
      \hspace*{2cm}\textbf{return} the plan if uniform-cost-search succeeded. \\
      \hspace*{1cm}\textbf{for each} $\vartheta \in
        \{0, 1, \dots, \textit{max-threshold}\}$: \\
      \hspace*{2cm}Let $\mathcal O_\vartheta$ be the set of operators of
        $\Pi$ whose modification distance with respect to $v$ \\
      \hspace*{2cm}\quad is at most $\vartheta$. \\
      \hspace*{2cm}Assign the cost $c$ to each operator $o \in
        \mathcal O_\vartheta$ with modification distance $c$ with \\
      \hspace*{2cm}\quad respect to $v$. \\
      \hspace*{2cm}Call the \emph{uniform-cost-search} algorithm with
        a closed list, using the operator set $O_\vartheta$, \\
      \hspace*{2cm}\quad to find a state satisfying $\{v = d\} \cup \cond$. \\
      \hspace*{2cm}\textbf{return} the plan if uniform-cost-search succeeded.
    \end{algorithm}
  }
}


==> helmert06a/figures/reach-one-goal.tex <==
\framebox{
  \parbox{14.8cm}{
    \begin{algorithm}
      \hspace*{0cm}\textbf{algorithm}
        reach-one-goal($\Pi$, $v$, $d$, $\cond$): \\
      \hspace*{1cm}\textbf{for each} $\vartheta \in
        \{0, 1, \dots, \textit{max-threshold}\}$: \\
      \hspace*{2cm}Let $\mathcal O_\vartheta$ be the set of operators of
        $\Pi$ whose modification distance with respect to $v$ \\
      \hspace*{2cm}\quad is at most $\vartheta$. \\
      \hspace*{2cm}Assign the cost $c$ to each operator $o \in
        \mathcal O_\vartheta$ with modification distance $c$ with \\
      \hspace*{2cm}\quad respect to $v$. \\
      \hspace*{2cm}Call the \emph{uniform-cost-search} algorithm with
        a closed list, using the operator set $O_\vartheta$, \\
      \hspace*{2cm}\quad to find a state satisfying $\{v = d\} \cup \cond$. \\
      \hspace*{2cm}\textbf{return} the plan if uniform-cost-search succeeded.
    \end{algorithm}
  }
}


==> helmert06a/figures/total-time-above-300.tex <==
%\framebox{
    \newcommand{\heading}[1]{%
      \multicolumn{1}{c}{\textbf{#1}}}
    \begin{tabular}{@{}lllrr@{}}
    \heading{Domain}
    & \heading{Task}
    & \heading{Configuration}
    & \heading{Preprocessing}
    & \heading{Search} \\[3pt]
    {\freecell} (IPC2)  & \texttt{probfreecell-10-1} &
      \textbf{M + P}    &   9.30\,s & 298.64\,s \\
    {\grid}             & \texttt{prob05} &
      \textbf{M}        &  10.04\,s & 291.01\,s \\
    {\mysteryprime}     & \texttt{prob14} & 
      \textbf{M}        &  22.38\,s & 291.67\,s \\
    {\psrlarge}         & \texttt{p30-s179-n30-l3-f30} &
      \textbf{G + P}    &  43.43\,s & 265.29\,s \\
    {\satellite} (IPC4) & \texttt{p33-HC-pfile13} &
      \textbf{M + P}    & 180.74\,s & 169.09\,s
    \end{tabular}
%}


==> helmert06a/introduction.tex <==
\section{Introduction}
\label{section:introduction}

Consider a typical transportation planning task: The postal service must
deliver a number of parcels to their respective destinations using its
vehicle fleet of cars and trucks. Let us assume that a car serves all
the locations of one city, and that different cities are connected via
highways that are served by trucks. For the sake of simplicity, let us
further assume that travelling on each segment of road or highway incurs
the same cost. This is not a highly realistic assumption, but for the
purposes of exposition it will do. There can be any number of parcels,
posted at arbitrary locations and with arbitrary destinations. Moreover,
cities can be of varying size, there can be one or several cars within
each city, and there can be one or several trucks connecting the
cities. Cars will never leave a city.  Fig.~\ref{figure:initial-example}
shows an example task of this kind with two cities, three cars and a
single truck. There are two parcels to be delivered, one of which
($p_1$) must be moved between the two cities, while the other ($p_2$)
can stay within its initial city.

\includepsfigure{initial-example}{A transportation planning task. Deliver
parcel $p_1$ from $C$ to $G$ and parcel $p_2$ from $F$ to $E$, using the
cars $c_1$, $c_2$, $c_3$ and truck $t$. The cars may only use inner-city
roads (thin edges), the truck may only use the highway (thick edge).}

The astute reader familiar with the planning literature will have
noticed by now that we are essentially describing the {\logistics}
domain, a standard benchmark for classical planning systems, extended to
roadmaps that are not complete graphs. (Part of) a propositional
STRIPS-like encoding of the task is shown in
Fig.~\ref{figure:initial-example-strips}.

\includefigure[p]{initial-example-strips}{Part of a typical
propositional encoding of the transportation planning task (no actual
PDDL syntax).}

How would human planners go about solving tasks of this kind? Very
likely, they would use a hierarchical approach: For $p_1$, it is clear
that the parcel needs to be moved between cities, which is only possible
by using the truck. Since in our example each city can access the
highway at only one location, we see that we must first load the parcel
into some car at its initial location, then drop it off at the first
city's highway access location, load it into the truck, drop it off at
the other city's highway access location, load it into the only car in
that city, and finally drop it off at its destination. We can commit to
this ``high-level'' plan for delivering $p_1$ without worrying about
``lower-level'' aspects such as path planning for the cars. It is
obvious to us that \emph{any} good solution will have this structure,
since the parcel can only change its location in a few clearly defined
ways (Fig.~\ref{figure:initial-example-parcel-dtg}). The same figure
shows that the only reasonable plans for getting $p_2$ to its
destination require loading it into the car in its initial city and
dropping it off at its target location. There is no point in ever
loading it into the truck or into any of the cars in the left city.

\includepsfigure{initial-example-parcel-dtg}{Domain transition graph for
the parcels $p_1$ and $p_2$. Indicates how a parcel can change its
state. For example, the arcs between ``at $D$'' and ``in $t$''
correspond to the actions of loading/unloading the parcel at location
$D$ with the truck $t$.}

\includepsfigure{initial-example-other-dtgs}{Domain transition graphs
for the cars $c_1$ and $c_2$ (left), truck $t$ (centre), and car $c_3$
(right). Note how each graph corresponds to the part of the roadmap that can
be traversed by the respective vehicle.}

\includepsfigure{initial-example-high-level-plan}{High-level plan for
the transportation planning task.}

So say we have committed to the (partially ordered, as movements of the
two parcels can be interleaved) ``high-level plan'' shown in
Fig.~\ref{figure:initial-example-high-level-plan}. All we need to do to
complete the plan is choose a linearization of the high-level steps and
fill in movements of the vehicle fleet between them. We have thus
decomposed the planning task into a number of subproblems. The parcel
scheduling problem (where, and by which vehicles, a parcel should be
loaded and unloaded) is separated from the path planning problem for
each vehicle in the fleet (how to move it from point X to Y). Both of
these are graph search problems, and the corresponding graphs are shown
in Fig.~\ref{figure:initial-example-parcel-dtg} and
Fig.~\ref{figure:initial-example-other-dtgs}. Graphs of this kind will
be formally introduced as \emph{domain transition graphs} in Section
\ref{section:knowledge-compilation}.

Of course these graph search problems interact, but they only do so in
limited ways: State transitions for the parcels have associated
conditions regarding the vehicle fleet, which need to be considered in
addition to the actual path planning in
Fig.~\ref{figure:initial-example-parcel-dtg}. For example, a parcel can
only change state from ``at location $A$'' to ``inside car $c_1$'' if
the car $c_1$ is at location $A$. However, state transitions for the
vehicles have no associated conditions from other parts of the planning
task, and hence moving a vehicle from one location to another is indeed
as easy as finding a path in the associated domain transition graph. We
say that the parcels have \emph{causal dependencies} on the vehicles
because there are operators that change the state of the parcels and
have preconditions on the state of the vehicles. Indeed, these are the
only causal dependencies in this task, since parcels do not depend on
other parcels and vehicles do not depend on anything except themselves
(Fig.~\ref{figure:initial-example-causal-graph}). The set of causal
dependencies of a planning task is visualized in its
\emph{causal graph}.

\includepsfigure{initial-example-causal-graph}{Causal dependencies in
the transportation planning task.}

We argue that humans often solve planning tasks in the hierarchical
fashion outlined in the preceding paragraphs, and that algorithmic
approaches to action planning can usefully apply similar ideas.
Indeed, as we will show in the following section, we are not the first
to introduce domain transition graphs and causal graphs. However,
earlier work has almost exclusively focused on \emph{acyclic} causal
graphs, and for a good reason: If the causal graph of a planning task
exhibits a cycle, hierarchical decomposition is not possible, because
the subproblems that must be solved to achieve an operator
precondition are not necessarily smaller than the original task. As
far as we are aware, we were the first \cite{malte-icaps-cg} to
present a \emph{general} planning algorithm that focuses on exploiting
hierarchical information from causal graphs. However, our \emph{causal
graph heuristic} also requires acyclicity; in the general case, it
considers a relaxed planning problem in which some operator
preconditions are ignored to break causal cycles.

Knowing that cycles in causal graphs are undesirable, we take a closer
look at the transportation planning task. Let us recall our informal
definition of causal graphs: The causal graph of a planning task
contains a vertex for each state variable and arcs from variables that
occur in preconditions to variables that occur in effects of the same
operator. So far, we may have given the impression that the causal graph
of the example task has the well-behaved shape shown in
Fig.~\ref{figure:initial-example-causal-graph}. Unfortunately, having a
closer look at the STRIPS encoding in
Fig.~\ref{figure:initial-example-strips}, we see that this is not the
case: The correct causal graph, shown in
Fig.~\ref{figure:initial-example-strips-causal-graph}, looks very messy.
This discrepancy between the intuitive and actual graph is due to the
fact that in our informal account of ``human-style'' problem solving, we
made use of (non-binary) state variables like ``the location of car
$c_1$'' or ``the state of parcel $p_1$'', while STRIPS-level state
variables correspond to (binary) object-location propositions like
``parcel $p_1$ is at location $A$''. It would be much nicer if we were
given a multi-valued encoding of the planning task that explicitly
contains a variable for ``the location of car $c_1$'' and similar
properties. Indeed, the nice looking acyclic graph in
Fig.~\ref{figure:initial-example-causal-graph} is the causal graph of
the multi-valued encoding shown in
Fig.~\ref{figure:initial-example-sas}.

\includepsfigure{initial-example-strips-causal-graph}{Causal graph for
the STRIPS encoding of the transportation planning task.}

\includefigure[p]{initial-example-sas}{Part of an encoding of the
transportation planning task with multi-valued state variables.}

Having provided some intuition for its underlying concepts, let us now
state our design goal for the Fast Downward planning system: \emph{To
develop an algorithm that efficiently solves general propositional
planning tasks by exploiting the hierarchical structure inherent in
causal graphs.} We need to overcome three major obstacles in
this undertaking:
\begin{itemize}
\item First, propositionally encoded planning tasks usually have very
  unstructured causal graphs. However, the intuitive dependencies
  often become visible in encodings with multi-valued state variables.
  To exploit this fact in an automated PDDL planning system, we have
  devised an automatic algorithm for ``translating'' (or
  reformulating) propositional tasks to multi-valued ones. The
  translation algorithm can be considered independently from the rest
  of the planner; in fact, it is now also used as part of other
  planning systems \cite{menkes-ilp}. To keep the article focused, we
  do \emph{not} discuss the translation algorithm here, referring to
  our earlier work for some of its central ideas \cite{minimize}.
  Instead, we consider its output, a \emph{multi-valued planning
    task}, as a base formalism.
\item Second, no matter how clever the encoding is, most planning
  tasks are not completely hierarchical in nature. To deal with causal
  cycles, we consider relaxations where some causal dependencies are
  ignored and use solutions to the relaxed problem within a heuristic
  search algorithm.
\item Third, even for planning tasks that can be solved
  hierarchically, finding such a solution is difficult (indeed, still
  \PSPACE-complete). For this reason, our heuristic function only
  considers a fragment of a task at a time, namely subproblems induced
  by a single state variable and its predecessors in the causal graph.
  Even \emph{this} planning problem is still NP-complete, so that we
  are content with an incomplete solution algorithm within the
  heuristic solver. This solution algorithm has theoretical
  shortcomings but never failed us in practice.
\end{itemize}

Having introduced the rationale of our approach, we discuss related
work in the next section. This is followed by an overview of the
general architecture of the Fast Downward planning system in
Section~\ref{section:architecture}. The planning system consists of
three components: \emph{translation}, \emph{knowledge compilation},
and \emph{search}. The translation component converts PDDL2.2 tasks to
multi-valued planning tasks, which we formally introduce in Section
\ref{section:definition}. The knowledge compilation component is
discussed in Section \ref{section:knowledge-compilation}, the search
component in Section \ref{section:search}. We conclude with a
presentation of experimental results in
Section~\ref{section:experiments} and some discussion in
Section~\ref{section:discussion}.


==> helmert06a/knowledge-compilation.tex <==
\section{Knowledge Compilation}
\label{section:knowledge-compilation}

The purpose of the knowledge compilation component is to set the stage
for the search algorithms by compiling the critical information about
the planning task into a number of data structures for efficient
access. In other contexts, computations of this kind are often called
\emph{preprocessing}. However, ``preprocessing'' is such a nondescript
word that it can mean basically anything. For this reason, we prefer a term that
puts a stronger emphasis on the role of this module: To rephrase the
critical information about the planning task in such a way that it is
directly useful to the search algorithms. Of the three building blocks
of Fast Downward (translation, knowledge compilation, search), it is
the least time-critical part, always requiring less time than
translation and being dominated by search for all but the most trivial
tasks.

Knowledge compilation comprises three items. First and foremost, we
compute the \emph{domain transition graph} of each state variable. The
domain transition graph for a state variable encodes under what
circumstances that variable can change its value, {\ie}, from which
values in the domain there are transitions to which other values,
which operators or axioms are responsible for the transition, and
which conditions on other state variables are associated with the
transition. Domain transition graphs are described in Section
\ref{section:domain-transition-graphs}. They are a central concept for
the computation of the causal graph heuristic, described in Section
\ref{section:cg-heuristic}.

Second, we compute the \emph{causal graph} of the planning task. Where
domain transition graphs encode dependencies between values for a
given state variable, the causal graph encodes dependencies between
different state variables. For example, if a given location in a
planning task can be unlocked by means of a key that can be carried by
the agent, then the variable representing the lock state of the
location is dependent on the variable that represents whether or not
the key is being carried. This dependency is encoded as an arc in the
causal graph. Like domain transition graphs, causal graphs are a
central concept for the computation of the causal graph heuristic, giving it its
name. The causal graph heuristic requires causal graphs to be acyclic. For this
reason, the knowledge compilation component also generates an acyclic
subgraph of the real causal graph when cycles occur. This amounts to a
relaxation of the planning task where some operator preconditions are
ignored. In addition to their usefulness for the causal graph heuristic, causal
graphs are also a key concept of the \emph{focused iterative-broadening
search} algorithm introduced in Section
\ref{section:focused-iterative-broadening-search}. We discuss causal
graphs in Section \ref{section:causal-graphs}.

Third, we compute two data structures that are useful for any
forward-searching algorithm for MPTs, called \emph{successor
generators} and \emph{axiom evaluators}. Successor generators
compute the set of applicable operators in a given world state, and
axiom evaluators compute the values of derived variables for a given
reduced state. Both are designed to do their job as
quickly as possible, which is especially important for the focused
iterative-broadening search algorithm, which does not compute
heuristic estimates and thus requires the basic operations for
expanding a search node to be implemented efficiently. These data
structures are discussed in Section
\ref{section:successor-generators}.

\subsection{Domain Transition Graphs}
\label{section:domain-transition-graphs}

The domain transition graph of a state variable is a representation of
the ways in which the variable can change its value, and of the
conditions that must be satisfied for such value changes to be
allowed. Domain transition graphs were introduced by Jonsson and
B\"ackstr\"om \citeyear{jonsson-sas} in the context of {\sasplus}
planning. Our formalization of domain transition graphs
generalizes the original definition to planning tasks involving axioms
and conditional effects.

\begin{definition}{domain-transition-graph}{Domain transition graphs}
Let $\Pi = \langle \mathcal V, s_0, s_\star, \mathcal A, \mathcal O
\rangle$ be a multi-valued planning task, and let $v \in \mathcal V$
be a state variable of $\Pi$.

The \definedTerm{domain transition graph} of $v$, in symbols
$\textit{DTG}(v)$, is a labelled directed graph with vertex set
$\mathcal D_v$.
If $v$ is a fluent, $\textit{DTG}(v)$ contains the following arcs:
\begin{itemize}
\item For each effect $\cond \rightarrow v := d'$ of an
  operator $o$ with precondition $\pre$ such that $\pre \cup \cond$
  contains some condition $v = d$, an arc from $d$ to $d'$ labelled
  with $\pre \cup \cond \setminus \{v=d\}$.
\item For each effect $\cond \rightarrow v := d'$ of an
  operator $o$ with precondition $\pre$ such that $\pre \cup \cond$
  does not contain the condition $v = d$ for any $d \in \mathcal D_v$,
  an arc from each $d \in \mathcal D_v \setminus \{d'\}$ to $d'$
  labelled with $\pre \cup \cond$.
\end{itemize}

If $v$ is a derived variable, $\textit{DTG}(v)$ contains the following
arcs:
\begin{itemize}
\item For each axiom $\cond \rightarrow v := d' \in \mathcal A$ such
  that $\cond$ contains some condition $v = d$, an arc from $d$ to
  $d'$ labelled with $\cond \setminus \{v=d\}$.
\item For each axiom $\cond \rightarrow v := d' \in \mathcal A$ such
  that $\cond$ does not contain the condition $v = d$ for any $d \in
  \mathcal D_v$, an arc from each $d \in \mathcal D_v \setminus
  \{d'\}$ to $d'$ labelled with $\cond$.
\end{itemize}

Arcs of domain transition graphs are called \definedTerm{transitions}.
Their labels are referred to as the \definedTerm{conditions} of the
transition.

Domain transition graphs can be weighted, in which case each
transition has an associated non-negative integer weight. Unless
stated otherwise, we assume that all transitions derived from
operators have weight 1 and all transitions derived from axioms have
weight 0.
\end{definition}

The definition is somewhat lengthy, but its informal content is easy
to grasp: The domain transition graph for $v$ contains a transition
from $d$ to $d'$ if there exists some operator or axiom that can
change the value of $v$ from $d$ to $d'$. Such a transition is
labelled with the conditions on \emph{other} state variables that must
be true if the transition shall be applied. Multiple transitions
between the same values using different conditions are allowed and
occur frequently.

\includepsfigure{domain-transition-graphs-grid}{Domain transition
  graphs of a {\grid} task.
  Top left: $\textit{DTG}(r)$
  (robot); right: $\textit{DTG}(k)$ (key); bottom left:
  $\textit{DTG}(d)$ (door).}

We have already seen domain transition graphs in the introductory
section (Figs.~\ref{figure:initial-example-parcel-dtg} and
\ref{figure:initial-example-other-dtgs}), although they were only
introduced informally and did not show the arc labels usually
associated with transitions.
Fig.~\ref{figure:domain-transition-graphs-grid} shows some examples
from a simple task in the {\grid} domain, featuring a $3\times2$ grid
with a single initially locked location in the centre of the upper
row, unlockable by a single key. In the MPT encoding of the task,
there are three state variables: variable $r$ with $\mathcal D_r =
\{~(x,y)~|~x \in \{1, 2, 3\}, \ y \in \{1, 2\}~\}$ encodes the
location of the robot, variable $k$ with $\mathcal D_k = \mathcal D_r
\cup \{\textit{carried}\}$ encodes the state of the key, and
variable $d$ with $\mathcal D_d = \{\textit{closed},
\textit{open}\}$ encodes the state of the initially locked grid
location.

If all operators of an MPT are unary ({\ie}, only have a single
effect) and we leave aside axioms for a moment, then there is a strong
correspondence between the state space of an MPT and its domain
transition graphs. Since vertices in domain transition graphs
correspond to values of state variables, a given state is represented
by selecting one vertex in each domain transition graph, called the
\emph{active vertex} of this state variable. Applying an operator
means changing the active vertex of some state variable by performing
a transition in the corresponding domain transition graph. Whether or
not such a transition is allowed depends on its condition, which is
checked against the active vertices of the other domain transition
graphs.

Let us use the {\grid} example to illustrate this correspondence.
Consider an initial state where the robot is at location $(1,1)$, the
key is at location $(3,2)$, and the door is locked. We represent this
by placing pebbles on the appropriate vertices of the three domain
transition graphs. We want to move the pebble in the domain transition
graph of the key to location $(2,1)$. This can be done by moving the
robot pebble to vertex $(1,2)$, then $(2,2)$, then $(3,2)$, moving the
key pebble to the vertex \emph{carried}, moving the robot pebble back
to vertex $(2,2)$, moving the door pebble to \emph{open}, moving the
robot pebble to vertex $(2,1)$ and finally moving the key pebble to
vertex $(2,1)$.

The example shows how plan execution can be viewed as simultaneous
traversal of domain transition graphs \cite<cf.>{carmel-ecp99}. This
is an important notion for Fast Downward because the causal graph heuristic
computes its heuristic estimates by solving subproblems of the
planning task by looking for paths in domain transition graphs in
basically the way we have described.

As mentioned before, this view of MPT planning is only completely
accurate for unary tasks without axioms, for which the domain
transition graphs are indeed a complete representation of the state
space. For non-unary operators, we would need to ``link'' certain
transitions in different domain transition graphs which belong to the
same operator. These could then only be executed together. For axioms,
we would need to mark certain transitions as ``mandatory'', requiring
that they be taken whenever possible. (This is only intended as a
rough analogy and leaves out details like layered axioms.)

In our previous work \cite{malte-icaps-cg}, we have successfully
applied this view of planning to STRIPS tasks. Extending the notion to
plans with conditional effects provides no challenges because domain
transition graphs always consider planning operators one effect at a
time, in which case effect condition can simply be seen as part of the
operator precondition. However, axioms provide a challenge that is
easily overlooked. If we want to change the value of a fluent
from $d$ to $d'$, the domain transition graph contains
all the important information; just find a path from $d$ to $d'$ and
try to find out how the associated conditions can be achieved.
Consider the same problem for a derived state variable. Let us assume
that unlocking the location in the {\grid} example leads to a drought,
causing the robot to freeze if it enters a horizontally adjacent
location. We could encode this with a new derived variable $f$ (for
\emph{freezing}) with domain $\mathcal D_f = \{\top, \bot\}$, defined
by the axioms $d = \textit{open}, r = (1,1) \rightarrow f := \top$ and
$d = \textit{open}, r = (3,1) \rightarrow f := \top$. The domain
transition graph $\textit{DTG}(f)$ is depicted in
Fig.~\ref{figure:domain-transition-graph-grid-axiom} (left).

\includepsfigure{domain-transition-graph-grid-axiom}{Domain transition
  graphs for the \emph{freezing} variable in the {\grid} task, normal
  (left) and extended (right). Note that only the extended graph shows
  how to change state from ``freezing'' ($\top$) to ``not freezing''
  ($\bot$).}

The problem with that domain transition graph is that it does not tell
us how we can change the state of variable $f$ from $\top$ to $\bot$.
In general, in MPTs derived from STRIPS tasks where derived predicates
occur negatively in any condition, the domain transition graph does
not contain sufficient information for changing the value of a derived
variable from ``true'' to ``false''. Derived variables never assume
the value $\bot$ due to a \emph{derivation} of this value; because of
negation as failure semantics, they only assume the value \emph{by
default} if \emph{no other value} can be derived. If we want to
reason about ways of setting the value of a derived variable to
$\bot$, we will need to make this information explicit.

In logical notation, whether or not a derived variable assumes a given
value by triggering an axiom at a given layer is determined by a
formula in disjunctive normal form, with one disjunct for each axiom
setting the value. For example, our axioms  $d = \textit{open}, r =
(1,1) \rightarrow f := \top$ and $d = \textit{open}, r = (3,1)
\rightarrow f := \top$ correspond to the DNF formula
$(d = \textit{open} \land r = (1,1)) \lor (d = \textit{open} \land
r = (3,1))$. If we want to know when these rules do \emph{not}
trigger, we must negate this formula, leading to the CNF formula
$(d \neq \textit{open} \lor r \neq (1,1)) \land (d \neq \textit{open}
\lor r \neq (3,1))$. To be able to encode this information in the
domain transition graph, we need to replace the inequalities with
equalities and translate the formula back to DNF. Since such
transformations can increase the formula size dramatically, we apply
simplifications along the way, removing duplicated and dominated
disjuncts. The result in this case is the DNF formula
$d = \textit{closed} \lor r = (2, 1) \lor
r = (1, 2) \lor r = (2, 2) \lor r = (3, 2)$.

A domain transition graph for a derived variable which has been
enriched to contain the possible ways of causing the variable to
assume the value $\bot$ is called an \emph{extended domain transition
graph}, as shown for the {\grid} example in
Fig.~\ref{figure:domain-transition-graph-grid-axiom} (right). Since
computing the extended domain transition graph can be costly and is
not always necessary, the knowledge compilation component scans the
conditions of the planning task (axioms, operator preconditions and
effect conditions, goal) for occurrences of pairings of the type $v =
\bot$ for derived variables $v$. Extended domain transition graphs are
only computed for those derived variables for which they are required.

Note that negative occurrences of derived variables can cascade: If
$u$, $v$ and $w$ are derived variables with domain $\{\top, \bot\}$
and the condition $v = \bot$ is present in some operator precondition,
and moreover $v$ is defined by the axiom $u = \top, w = \top
\rightarrow v := \top$, then $v$ assumes the value $\bot$ whenever $u$
or $w$ do, so we would require extended domain transition graphs for
$u$ and $w$ as well.

On the other hand, multiple layers of negation as failure can cancel
each other out: If derived variable $v$ only occurs in conditions of
the form $v = \bot$ but never in positive form and is defined by the
axiom $u = \bot, w = \bot \rightarrow v := \top$, then we do not
necessarily require extended domain transition graphs for $u$ and $w$.

In general, whether or not we need extended domain transition graphs
for a derived variable is determined by the following rules:
\begin{itemize}
\item If $v$ is a derived variable for which the condition $v = d$
  for $d \neq \bot$ appears in an operator precondition, effect
  condition or in the goal, then $v$ \emph{is used positively}.
\item If $v$ is a derived variable for which the condition $v = \bot$
  appears in an operator precondition, effect condition or in the
  goal, then $v$ \emph{is used negatively}.
\item If $v$ is a derived variable for which the condition $v = d$
  for $d \neq \bot$ appears in the body of an axiom whose head is used
  positively (negatively), then $v$ is used positively (negatively).
\item If $v$ is a derived variable for which the condition $v = \bot$
  appears in the body of an axiom whose head is used
  positively (negatively), then $v$ is used negatively (positively).
\end{itemize}

The knowledge compilation component computes extended domain
transition graphs for all derived variables which are used negatively
and (standard) domain transition graphs for all other state variables.
Normal domain transition graphs are computed by going through the set
of axioms and the set of operator effects following Definition
\ref{def:domain-transition-graph}, which is reasonably
straight-forward; the computation of extended domain transition
graphs has been outlined above. Therefore, the algorithmic aspects of
this topic should not require further discussion.

\subsection{Causal Graphs}
\label{section:causal-graphs}

Causal graphs have been introduced informally in the introduction.
Here is a formal definition.

\begin{definition}{causal-graph}{Causal graphs}
Let $\Pi$ be a multi-valued planning task with variable set $\mathcal
V$. The \definedTerm{causal graph} of $\Pi$, in symbols
$\textit{CG}(\Pi)$, is the directed graph with vertex set $\mathcal V$
containing an arc $(v,v')$ iff $v \neq v'$ and one of the following
conditions is true:
\begin{itemize}
\item The domain transition graph of $v'$ has a transition with some
  condition on $v$.
\item The set of affected variables in the effect list of some
  operator includes both $v$ and $v'$.
\end{itemize}
In the first case, we say that an arc is induced by a \definedTerm{transition
condition}. In the second case we say that it is induced by
\definedTerm{co-occurring effects}.
\end{definition}

Of course, arcs induced by transition conditions and arcs induced by
co-occurring effects are not mutually exclusive. The same causal graph
arc can be generated for both reasons.

Informally, the causal graph contains an arc from a source variable to
a target variable if changes in the value of the target variable can
depend on the value of the source variable. Such arcs are included
also if this dependency is of the form of an \emph{effect} on the
source variable. This agrees with the definition of \emph{dependency
graphs} by Jonsson and B\"ackstr\"om \citeyear{jonsson-3s}, although
these authors distinguish between the two different ways in which an
arc in the graph can be introduced by using labelled arcs.

Whether or not co-occurring effects should induce arcs in the causal
graph depends on the intended semantics: If such arcs are not included, the
set of causal graph ancestors $\textit{anc}(v)$ of a variable $v$ are
precisely those variables which are relevant if our goal is to change
the value of $v$. Plans for this goal can be computed without
considering any variables outside $\textit{anc}(v)$, by eliminating
all variables outside $\textit{anc}(v)$ from the planning task and
simplifying axioms and operators accordingly. We call this the
\emph{achievability definition} of causal graphs, because causal
graphs encode what variables are important for achieving a given
assignment to a state variable.

However, with the achievability definition, a planner that only
considers $\textit{anc}(v)$ while generating an action sequence that
achieves a given valuation for $v$ may modify variables outside of
$\textit{anc}(v)$, {\ie}, the generated plans have side effects which
could destroy previously achieved goals or otherwise have a negative
impact on overall planning. Therefore, we prefer our definition, which
we call the \emph{separability definition} of causal graphs.

\subsubsection{Acyclic Causal Graphs}

Following the separability definition of causal graphs, solving a
subproblem over variables $\textit{anc}(v)$ is always possible without
changing any values outside of $\textit{anc}(v)$. This leads us to the
following observation.

\begin{observation}{easy-problems}{Acyclic causal graphs and
    strongly connected domain transition graphs}
Let $\Pi$ be an MPT such that $\textit{CG}(\Pi)$ is acyclic, all
domain transition graphs are strongly connected, there are no derived
variables, and no trivially false conditions occur in operators or
goals. Then $\Pi$ has a solution.
\end{observation}

By \emph{trivially false} conditions, we mean conditions of the kind
$\{v = d, v = d'\}$ for $d \neq d'$. Note the similarity of
Observation \ref{observation:easy-problems} to the results of
Williams and Nayak \citeyear{williams-nayak} on planning in domains
with unary operators, acyclic causal graphs and reversible
transitions. Under the separability definition of causal graphs,
acyclic causal graphs imply unariness of operators because operators
with several effects introduce causal cycles. Moreover, strong
connectedness of domain transition graphs is closely related to
Williams' and Nayak's reversibility property, although it is a weaker
requirement.

The truth of the observation can easily be seen inductively: If the
planning task has only one state variable and the domain transition
graph is strongly connected, then any state (of the one variable) can
be transformed into any other state by applying graph search
techniques. If the planning task has several state variables and the
causal graph is acyclic, we pick a sink of the causal graph, {\ie}, a
variable $v$ without outgoing arcs, and check if a goal is defined for
this variable. If not, we remove the variable from the task, thus
reducing the problem to one with fewer state variables, solved
recursively. If yes, we search for a path from $s_0(v)$ to
$s_\star(v)$ in the domain transition graph of $v$, which is
guaranteed to exist because the graph is strongly connected. This
yields a ``high-level plan'' for setting $v$ to $s_\star(v)$ which can
be fleshed out by recursively inserting the plans for setting the
variables of the predecessors of $v$ in the causal graph to the values
required for the transitions that form the high-level plan. Once the
desired value of $v$ has been set, $v$ can be eliminated from the
planning task and the remaining problem can be solved recursively.

\includefigure{planning-algorithm-easy-task}{Planning algorithm for
  MPTs with acyclic causal graph and strongly connected domain
  transition graphs.}

The algorithm is shown in
Fig.~\ref{figure:planning-algorithm-easy-task}. Although it is
backtrack-free, it can require exponential time to execute because the
generated plans can be exponentially long. This is unavoidable; even
for MPTs that satisfy the conditions of Observation
\ref{observation:easy-problems}, shortest plans can be exponentially
long. A family of planning tasks with this property is given in the proof of
Theorem 4.4 in the article by B\"ackstr\"om and Nebel
\citeyear{complexity-sas}.

This method for solving multi-valued planning tasks is
essentially \emph{planning by refinement}: We begin by constructing a
very abstract skeleton plan, which is merely a path in some domain
transition graph, then lower the level of abstraction by adding
operators to satisfy the preconditions required for the transitions
taken by the path. Strong connectedness of domain transition graphs
guarantees that every abstract plan can actually be refined to a
concrete plan. This is precisely Bacchus and Yang's
\citeyear{bacchus-downward-refinement} \emph{downward 
refinement property} (cf.~Section
\ref{section:related-work-abstractions}).

\subsubsection{Generating and Pruning Causal Graphs}

The usefulness of causal graphs for planning by refinement is not
limited to the acyclic case. Consider a subset $\mathcal V'$ of the
task variables which contains all its causal graph descendants. In
general, if we restrict the task to $\mathcal V'$ by removing all
occurrences of other variables from the initial state, goal, operators
and axioms, we obtain an abstraction of the original problem which
satisfies Knoblock's \citeyear{knoblock-abstractions} ordered
monotonicity property (Section
\ref{section:related-work-abstractions}).

Unfortunately, one major problem with this approach is that the
requirement to include all causal graph descendants is quite limiting.
It is not uncommon for the causal graph of a planning task to be
strongly connected, in which case this technique will not allow us to
abstract away any variables at all. However, in a heuristic approach,
we are free to simplify the planning task. In particular, by ignoring
some operator preconditions for the purposes of heuristic evaluation,
we can make an arbitrary causal graph acyclic. Clearly, the more
aspects of the real task we ignore, the worse we can expect our
heuristic to approximate the actual goal distance. Considering this, our aim is to
ignore as little information as possible. We will now explain how this
is done.

The knowledge compilation component begins its causal graph processing
by generating the ``full'' causal graph (Definition
\ref{def:causal-graph}). One consequence of the separability
definition of causal graphs is that all state variables which are not
ancestors of variables mentioned in the goal are completely
irrelevant. Therefore, having computed the graph, we then compute the
causal graph ancestors of all variables in the goal. Any state
variables which are not found to be goal ancestors are eliminated from
the planning task and causal graph, and associated operators and axioms
are removed.\footnote{This simplification is closely related to Knoblock's
  criterion for the \emph{problem-specific} ordered monotonicity
  property \cite{knoblock-abstractions}.}  Afterwards, we compute a
\emph{pruned causal graph}, an acyclic subgraph of the causal graph
with the same vertex set. We try do this in such a fashion that
``important'' causal dependencies are retained whenever possible. More
specifically, we apply the following algorithm.

First, we compute the strongly connected components of the causal
graph. Cycles only occur within strongly connected components, so each
component can be dealt with separately. Second, for each connected
component, we compute a total order $\prec$ on the vertices, retaining
only those arcs $(v,v')$ for which $v \prec v'$. If $v \prec v'$, we
say that $v'$ has a \emph{higher level} than $v$. The total order is
computed in the following way:

\begin{enumerate}
\item
  We assign a weight to each arc in the causal graph. The weight of an
  arc is $n$ if it is induced by $n$ axioms or operators. The
  lower the cumulated weight of the incoming arcs of a vertex, the
  fewer conditions are ignored by assigning a low level to this
  vertex.
\item 
  We then pick a vertex $v$ with minimal cumulated weight of
  incoming arcs and select it for the lowest level, {\ie}, we set
  $v \prec v'$ for all other vertices $v'$ in the strongly connected
  component.
\item Since $v$ has been dealt with, we remove the vertex and its
  incident arcs from consideration for the rest of the ordering
  algorithm.
\item The remaining problem is solved by iteratively applying the same
  technique to order the other vertices until only a single vertex
  remains.
\end{enumerate}

The reader will notice that the pruning choices within a strongly
connected component are performed by a greedy algorithm. We could also
try to find sets of arcs of minimal total weight such that
eliminating these arcs results in an acyclic graph. However, this is
an \NP-equivalent problem, even in the case of unweighted graphs
\cite[problem GT8]{garey-johnson}.

After generating the pruned causal graph, we also prune the domain
transition graphs by removing from the transition labels of
$\textit{DTG}(v)$ all conditions on variables $v'$ with $v \prec v'$.
These are the conditions that are ignored by the heuristic computation.
Finally, we simplify the domain transition graphs by removing
\emph{dominated transitions}: If $t$ and $t'$ are transitions between
the same two values of a variable, and the condition of $t$ is a
proper subset of the condition of $t'$, then transition $t$ is easier
to apply than $t'$, so that we remove $t'$.  Similarly, if there are
several transitions with identical conditions, we only keep one of
them.

\subsubsection{Causal Graph Examples}
\label{section:causal-graph-examples}

\includepsfigure{causal-graph-logistics}{Causal graph of a
  {\logistics} task. State variables $t_i$ and $a_i$ encode the
  locations of trucks and airplanes, state variables $p_i$ the
  locations of packages.}

To give some impression of the types of causal graphs typically found
in the standard benchmarks and the effects of pruning, we show some
examples of increasing graph complexity.

As our first and simplest example,
Fig.~\ref{figure:causal-graph-logistics} shows the causal graph of a
task from the {\logistics} domain, featuring two trucks, two airplanes
and two packages. As can be seen, the graph is acyclic, so it requires
no pruning for the causal graph heuristic. Since {\logistics} tasks
also feature strongly connected domain transition graphs, they can
even be solved by the polynomial \emph{solve-easy-MPT} algorithm.

\includepsfigure{causal-graph-mystery}{Causal graph of a
  {\mystery} task (left) and of a relaxed version of the task (right).
  State variables $f_i$ encode the fuel at a location, state variables $l_i$
  and $c_i$ encode the locations and remaining capacities of trucks, and
  state variables $p_i$ encode the locations of packages.}

As a slightly more complicated example, the next figure,
Fig.~\ref{figure:causal-graph-mystery}, shows a task from the
{\mystery} domain with three locations, two trucks and two packages.
The causal graph contains a number of cycles, but these are mostly
local. By pruning arcs from vertices $l_i$ to $f_j$, we ignore the
fact that we must move trucks to certain locations if we want to use
up fuel at that location. As using up fuel is not a very useful thing
to do, this is not a big loss in information. By pruning arcs from
vertices $p_i$ to $c_j$, we ignore the fact that vehicles can only
increase or decrease their current capacity by unloading or loading
packages. Compared to heuristics based on ignoring delete effects,
this is not a great loss in information, since ignoring delete effects
in the {\mystery} domain almost amounts to ignoring capacity and fuel
constraints altogether. By pruning just these arcs, we can eliminate
all cycles in the causal graph, so the {\mystery} domain can be
considered fairly well-behaved.

\includepsfigure{causal-graph-grid}{Causal graph of a {\grid} task
  (left) and of a relaxed version of the task (right). State variable
  $r$ encodes the location of the robot, $a$ encodes the status of the
  robot arm (empty or carrying a key), $l$ encodes the status of the
  locked location (locked or open), and $k_1$ and $k_2$ encode the
  locations of the two keys.}

A worse case is shown in Fig.~\ref{figure:causal-graph-grid}, which
shows an example from the {\grid} domain with an arbitrary number of
locations, of which a single one is locked. There are two keys, one of
which can unlock the locked location. Eliminating cycles here requires
a few minor relaxations regarding the status of the robot arm (empty
or non-empty), but also one major simplification, namely the
elimination of the arc from $l$ to $r$ representing the fact that the
robot can only enter the locked location if it has been unlocked.

As a (nearly) worst-case example, consider a task in the
{\blocksworld} domain (no figure). A typical MPT encoding uses one
state variable $h$ for encoding whether or not the hand is empty and
two state variables per block in the task: For the $i$-th block, $t_i$
encodes whether or not the block is lying on the table, and $b_i$
encodes which block is lying on top of it, or if it is clear or being
held by the arm. In the causal graph of such a task, variable $h$ has
ingoing arcs from and outgoing arcs to all other state variables, and
all state variables $b_i$ are connected to each other in both
directions. Only the state variables $t_i$ have a slightly simpler
connection structure, being only connected to $h$ and to $b_i$ for the
same value of $i$. Any relaxation of the problem that eliminates
cycles from the causal graph loses a large amount of information, and
it is not surprising that the {\depot} domain, which includes a
{\blocksworld} subproblem, is the one for which the precursor of Fast
Downward fared worst \cite{malte-icaps-cg}. Still, it should be
pointed out that planners that ignore delete effects have similar
problems with \blocksworld-like domains, as the comparison between the FF
and causal graph heuristics in the same article shows.

\subsection{Successor Generators and Axiom Evaluators}
\label{section:successor-generators}

In addition to good heuristic guidance, a forward searching planning
system needs efficient methods for generating successor states if it
is to be applied to the benchmark suite from the international
planning competitions. For some domains, our causal graph heuristic or
other popular methods like the FF heuristic provide excellent goal
estimates, yet still planning can be too time-consuming because of
very long plans and vast branching factors.

The variant of best-first search implemented in Fast Downward does not
compute the heuristic estimate for each state that is generated.
Essentially, heuristic evaluations are only computed for closed nodes,
while computation is deferred for nodes on the search
frontier. For domains with strong heuristic guidance and large
branching factors, the number of nodes on the frontier can by far
dominate the number of nodes in the closed set. As a case in point,
consider the problem instance {\satellite} \#29. For solving this
task, the default configuration of Fast Downward only computes
heuristic estimates for 67\,597 world states while adding
107\,233\,381 states to the frontier. Clearly, determining the set of
applicable operators quickly is of critical importance in such a
scenario.

In some {\satellite} tasks, there are almost 1\,000\,000 ground
operators, so we should try to avoid individually checking each
operator for applicability.  Similarly, in the biggest {\psr} tasks,
more than 100\,000 axioms must be evaluated in each state to compute
the values of the derived variables, so this computation must be made
efficient. For these purposes, Fast Downward uses two data structures
called \emph{successor generators} and \emph{axiom evaluators}.

\subsubsection{Successor Generators}

Successor generators are recursive data structures very similar to
decision trees. The internal nodes have associated conditions, which
can be likened to the decisions in a decision tree, and the leaves
have associated operator lists which can be likened to a set of
classified samples in a decision tree leaf. They are formally defined
as follows.

\begin{definition}{successor-generator}{Successor generators}
  A \definedTerm{successor generator} for an MPT $\Pi = \langle
  \mathcal V, s_0, s_\star, \mathcal A, \mathcal O\rangle$ is a tree
  consisting of \definedTerm{selector nodes} and
  \definedTerm{generator nodes}.

  A selector node is an internal node of the tree. It has an
  associated variable $v \in \mathcal V$ called the
  \definedTerm{selection variable}. Moreover, it has $|\mathcal D_v|
  + 1$ children accessed via labelled edges, one edge labelled $v = d$
  for each value $d \in \mathcal D_v$, and one edge labelled $\top$.
  The latter edge is called the \definedTerm{don't care edge} of the
  selector.

  A generator node is a leaf node of the tree. It has an associated
  set of operators from $\mathcal O$ called the set of
  \definedTerm{generated operators}.

  Each operator $o \in \mathcal O$ must occur in exactly one generator
  node, and the set of edge labels leading from the root to this
  node (excluding don't care edges) must equal the precondition of $o$.
\end{definition}

Given a successor generator for an MPT $\Pi$ and a state $s$ of $\Pi$,
we can compute the set of applicable operators in $s$ by traversing
the successor generator as follows, starting from the root:
\begin{itemize}
\item At a selector node with selection variable $v$, follow the edge
  $v = s(v)$ and the don't care edge.
\item At a generator node, report the generated operators as
  applicable.
\end{itemize}

To build a successor generator for $\Pi$, we apply a
top-down algorithm which considers the task variables in an arbitrary
order $v_1 \prec v_2 \prec \dots \prec v_n$. At the root node, we
choose $v_1$ as selection variable and classify the set of operators
according to their preconditions with respect to $v_1$. Operators with
a precondition $v_1=d$ will be represented in the child of the root
accessed by the edge with the corresponding label, while operators without
preconditions on $v_1$ will be represented in the child of the root
accessed by the don't care edge. In the children of the root, we
choose $v_2$ as selection variable, in the grandchildren $v_3$, and so
on.

There is one exception to this rule to avoid creating unnecessary
selection nodes: If no operator in a certain branch of the tree has a
condition on $v_i$, then $v_i$ is not considered as a selection
variable in this branch. The construction of a branch ends when all
variables have been considered, at which stage a generator node is
created for the operators associated with that branch.

\subsubsection{Axiom Evaluators}

Axiom evaluators are a simple data structure used for efficiently
implementing the well-known \emph{marking algorithm} for propositional
Horn logic \cite{horn-marking}, extended and modified for the
layered logic programs that correspond to the axioms of an MPT.
They consist of two parts. Firstly, an indexing data structure maps a
given variable/value pairing and a given axiom layer to the set of
axioms in the given layer in whose body the pairing appears. Secondly, a
set of counters, one for each axiom, counts the number of conditions
of the axiom that have not yet been derived.

\includefigure{evaluate-axioms-efficiently}{Computing the values of
  the derived variables in a given planning state.}

Within Fast Downward, axioms are evaluated in two steps. First, all
derived variables are set to their default value $\bot$. Second,
algorithm \emph{evaluate-axiom-layer}
(Fig.~\ref{figure:evaluate-axioms-efficiently}) is executed for each
axiom layer in sequence to determine the final values of the derived
variables.

We assume that the reader is familiar enough with the marking
algorithm not to require much explanation, so we only point out that
the test whether or not an axiom is ready to trigger is implemented by
means of a queue in which axioms are put as soon as their counter
reaches 0. The actual implementation of \emph{evaluate-axiom-layer}
within Fast Downward initializes axiom counters slightly more
efficiently than indicated by the pseudo-code. However, this is a
minor technical detail, so we turn to the remaining piece of Fast
Downward's architecture, the search component.



==> helmert06a/related-work.tex <==
\section{Related Work}
\label{section:related-work}

As a planning system based on heuristic forward search, Fast Downward
is clearly related to other heuristic planners such as HSP \cite{hsp}
or FF \cite{ff} on the architectural level. However, in this section
we focus on work that is related on the \emph{conceptual} level, \ie,
work that uses similar forms of hierarchical decomposition of causal
graphs and work that uses similar forms of search in domain transition
graphs.

\subsection{Causal Graphs and Abstraction}
\label{section:related-work-abstractions}

The term \emph{causal graph} first appears in the literature in the
work by Williams and Nayak \citeyear{williams-nayak}, but the general
idea is considerably older. The approach of hierarchically
decomposing planning tasks is arguably as old as the field of AI
Planning itself, having first surfaced in Newell and Simon's
\citeyear{newell-simon:1963} work on the General Problem Solver.

Still, it took a long time for these notions to evolve to their
modern form. Sacerdoti's \citeyear{sacerdoti:aij74} ABSTRIPS algorithm
introduced the concept of \emph{abstraction spaces} for STRIPS-like
planning tasks. An abstraction space of a STRIPS task is the state
space of an \emph{abstracted task}, which is obtained by removing all
preconditions from the operators of the original task that belong to a
given set of propositions (which are \emph{abstracted
away}).\footnote{In later work by other authors, propositions which
are abstracted away are also removed from the operator effects. This
only makes a difference in subtle cases that require the presence of
axioms; we do not distinguish between these two kinds of abstraction
here.} To solve a planning task, ABSTRIPS first generates a plan for
an abstracted task, then refines this plan by inserting concrete plans
between the abstract plan steps that ``bridge the gap'' between
abstract states by satisfying the operator preconditions which were
ignored at the abstract level. The idea is easily generalized to
several levels of abstraction forming an \emph{abstraction hierarchy},
with a very abstract level at the top where almost all preconditions
are ignored, successively introducing more preconditions at every
layer until the final layer of the hierarchy equals the original
planning task.

One problem with this approach to planning is that in general there
is no guarantee that the abstract plans bear any resemblance to
reasonable concrete plans. For example, if abstraction spaces are
chosen badly, it is quite possible that finding a concrete plan that
satisfies the precondition of the first operator in the abstract plan
is more difficult than solving the original goal at the concrete
level. Such shortcomings spawned a large amount of research on the
properties of abstraction hierarchies and how they can be generated
automatically.

Tenenberg \citeyear{tenenberg:1991} gives one of the
first formal accounts of the properties of different kinds of
abstraction. Among other contributions, he defines the so-called
\emph{upward solution property}, which can be informally stated as:
``If there exists a concrete solution, then there also exists an
abstract solution''. Rather surprisingly, not all abstractions
considered at the time satisfied this very basic property, without
which one would be loathe to call a given state space an
``abstraction'' of another state space.

A limitation of the upward solution property is that it states no
relationship between the concrete and abstract plan at all. For
ABSTRIPS-style hierarchical planning to be successful, the abstract
plan must bear some resemblance to a concrete one; otherwise there is
little point in trying to refine it. Indeed, Tenenberg introduces
stronger versions of the upward solution property, but more relevant
to Fast Downward is Knoblock's \citeyear{knoblock-abstractions} work
on the \emph{ordered monotonicity property}. An abstraction space
satisfies the ordered monotonicity property if, roughly speaking, any
concrete solution can be derived from some abstract solution while
leaving the actions in the abstract plan intact and relevant to the
concrete plan. Clearly, this is a very important property for
ABSTRIPS-like hierarchical planning.

It is in Knoblock's article that causal graphs first surface (although
he does not introduce a name for them). Translated to our terminology,
Knoblock proves the following relationship between useful abstractions
and causal graphs: \emph{If the causal graph contains no path from a
variable that is not abstracted away to a variable that is abstracted
away, then the abstraction has the ordered monotonicity property.} In
particular, this means that for acyclic causal graphs, it is possible
to devise an abstraction hierarchy where only one new variable is
introduced at each level.

Besides these theoretical contributions, Knoblock presents a
planning system called ALPINE which computes an abstraction hierarchy
for a planning task from its causal graph and exploits this within a
hierarchical refinement planner. Although the planning method is very
different, the derivation of the abstraction hierarchy is very similar
to Fast Downward's method for generating hierarchical decompositions
of planning tasks (Section \ref{section:causal-graphs}).

By itself, the ordered monotonicity property is not sufficient to
guarantee good performance of a hierarchical planning approach. It
guarantees that every concrete solution can be obtained in a natural
way from an abstract solution, but it does not guarantee that all
abstract solutions can be refined to concrete ones. Such a guarantee
is provided by the \emph{downward refinement property}, introduced by
Bacchus and Yang \citeyear{bacchus-downward-refinement}.

The downward refinement property can rarely be guaranteed in actual
planning domains, so Bacchus and Yang develop an analytical model for
the performance of hierarchical planning in situations where a given
abstract plan can only be refined with a certain probability $p < 1$.
Based on this analysis, they present an extension to ALPINE called
HIGHPOINT, which selects an abstraction hierarchy with high refinement
probability among those that satisfy the ordered monotonicity
property. In practice, it is not feasible to compute the refinement
probability, so HIGHPOINT approximates this value based on the notion
of \emph{$k$-ary necessary connectivity}.

\subsection{Causal Graphs and Unary STRIPS Operators}

Causal graphs are first given a name by Jonsson and B\"ackstr\"om
\citeyear{jonsson-backstrom:ewsp95,jonsson-3s}, who call them
\emph{dependency graphs}. They study a fragment of propositional
STRIPS with negative conditions which has the interesting property
that plan existence can be decided in polynomial time, but minimal
solutions to a task can be exponentially long, so that no polynomial
planning algorithm exists. They present an \emph{incremental} planning
algorithm with polynomial delay, \ie, a planning algorithm that
decides within polynomial time whether or not a given task has a
solution, and, if so, generates such a solution step by step, requiring
only polynomial time between any two subsequent
steps.\footnote{However, there is no guarantee that the length of the
generated solution is polynomially related to the length of an
optimal solution; it might be exponentially longer. Therefore, the
algorithm might spend exponential time on tasks that can be solved
in polynomial time.}

The fragment of STRIPS covered by Jonsson and
B\"ackstr\"om's algorithm is called \emph{3S} and is defined by the
requirement that the causal graph of the task is acyclic and each
state variables is \emph{static}, \emph{symmetrically reversible}, or
\emph{splitting}. \emph{Static} variables are those for which it is
easy to guarantee that they never change their value in any solution
plan. These variables can be detected and compiled away easily.
\emph{Symmetrically reversible} variables are those where for each
operator which makes them true there is a corresponding operator with
identical preconditions which makes them false, and vice versa. In
other words, a variable is symmetrically reversible iff its domain
transition graph is undirected. Finally, a variable $v$ is
\emph{splitting} iff its removal from the causal graph weakly
disconnects its positive successors (those variables which appear in
effects of operators of which $v$ is a precondition) from its negative
successors (those variables which appear in effects of operators of
which $\neg v$ is a precondition).

Williams and Nayak \citeyear{williams-nayak} independently prove that
incremental (or, in their setting, \emph{reactive}) planning is a
polynomial problem in a STRIPS-like setting where causal graphs are
acyclic and all operators are reversible. If all operators are
reversible (according to the definition by Williams and Nayak), all
variables are symmetrically reversible (according to the definition by
Jonsson and B\"ackstr\"om), so this is actually a special case of the
previous result. However, Williams and Nayak's work applies to a more
general formalism than propositional STRIPS, so that the approaches are not
directly comparable.

More recently, Domshlak and Brafman provide a detailed account of the
complexity of finding plans in the propositional STRIPS (with
negation) formalism with unary operators and acyclic graphs
\cite{carmel-unary,brafman-domshlak:jair2003}.\footnote{According to
our formal definition of causal graphs in Section
\ref{section:causal-graphs}, operators with several effects always
induce cycles in the causal graph, so \emph{acyclic causal graph}
implies \emph{unary operators}. Some researchers define causal
graphs differently, so we name both properties explicitly here.}
Among other results, they prove that the restriction to unary
operators and acyclic graphs does not reduce the complexity of plan
existence: the problem is \PSPACE-complete, just like unrestricted
propositional STRIPS planning \cite{complexity-bylander}. They also
show that for singly connected causal graphs, shortest plans cannot be
exponentially long, but the problem is still \NP-complete. For an even
more restricted class of causal graphs, namely polytrees of bounded
indegree, they present a polynomial planning algorithm. More
generally, their analysis relates the complexity of STRIPS planning in
unary domains to the \emph{number of paths} in their causal graph.

\subsection{Multi-Valued Planning Tasks}

With the exception of Williams and Nayak's paper, all the work
discussed so far exclusively deals with \emph{propositional} planning
problems, where all state variables assume values from a binary
domain. As we observed in the introduction, the question of
propositional vs.~multi-valued encodings usually has a strong impact
on the connectivity of the causal graph of a task. In fact, apart
from the trivial {\movie} domain, none of the common planning
benchmarks exhibits an acyclic causal graph when considering its
propositional representation. By contrast, the multi-valued encoding
of our introductory example does have an acyclic causal graph.

Due to the dominance of the PDDL (and previously, STRIPS) formalism,
non-binary state variables are not studied very often in the classical
planning literature. One of the most important exceptions to this rule
is the work on the {\sasplus} planning formalism, of which the papers
by B\"ackstr\"om and Nebel \citeyear{complexity-sas} and Jonsson and
B\"ackstr\"om \citeyear{jonsson-sas} are most relevant to Fast Downward.
The {\sasplus} planning formalism is basically equivalent to the
\emph{multi-valued planning tasks} we introduce in Section
\ref{section:definition} apart from the fact that it does not include
derived variables (axioms) or conditional effects. B\"ackstr\"om and
Nebel analyse the complexity of various subclasses of the
{\sasplus} formalism and discover three properties (\emph{unariness},
\emph{post-uniqueness} and \emph{single-valuedness}) that together
allow optimal planning in polynomial time. One of these three
properties (unariness) is related to acyclicity of causal graphs, and
one (post-uniqueness) implies a particularly simple shape of domain
transition graphs (namely, in post-unique tasks, all domain transition
graphs must be simple cycles or trees).

B\"ackstr\"om and Nebel do not analyse domain transition graphs
formally. Indeed, the term is only introduced in the later article by
Jonsson and B\"ackstr\"om \citeyear{jonsson-sas}, which refines the
earlier results by introducing five additional restrictions for
{\sasplus} tasks, all of which are related to properties of
domain transition graphs.

Neither of these two articles discusses the notion of causal graphs.
Indeed, the only earlier work we are aware of which includes
\emph{both} causal graphs and domain transition graphs as central
concepts is the article by Domshlak and Dinitz \citeyear{carmel-ecp99}
on the \emph{state-transition support} (STS) problem, which is
essentially equivalent to {\sasplus} planning with unary operators. In
the context of STS, domain transition graphs are called \emph{strategy
  graphs} and causal graphs are called \emph{dependence graphs}, but
apart from minor details, the semantics of the two formalisms are
identical. Domshlak and Dinitz provide a map of the complexity of the
STS problem in terms of the shape of its causal graph, showing that
the problem is \NP-complete or worse for almost all non-trivial cases.
One interesting result is that if the causal graph is a simple chain
of $n$ nodes and all variables are three-valued, the length of minimal
plans can already grow as $\Omega(2^n)$. By contrast,
\emph{propositional} tasks with the same causal graph shape admit
polynomial planning algorithms according to the result by Brafman and
Domshlak \citeyear{brafman-domshlak:jair2003}, because such causal
graphs are polytrees with a constant indegree bound (namely, a bound
of $1$).

To summarize and conclude our discussion of related work, we observe
that the central concepts of Fast Downward and the causal graph
heuristic, such as causal graphs and domain transition graphs, are
firmly rooted in previous work. However, Fast Downward is the first
attempt to marry hierarchical problem decomposition to the use of
multi-valued state variables within a general planning framework. It
is also the first attempt to apply techniques similar to those of
Knoblock \citeyear{knoblock-abstractions} and Bacchus and Yang
\citeyear{bacchus-downward-refinement} within a heuristic search
planner.

The significance of this latter point should not be
underestimated: For classical approaches to hierarchical problem
decomposition, it is imperative that an abstraction satisfies the
ordered monotonicity property, and it is important that the
probability of being able to refine an abstract plan to a concrete
plan is high, as the analysis by Bacchus and Yang shows.
Unfortunately, non-trivial abstraction hierarchies are rarely
ordered monotonic, and even more rarely guarantee high
refinement probabilities. Within a heuristic approach, these
``must-haves'' turn into ``nice-to-haves'': If an abstraction
hierarchy is not ordered monotonic or if an abstract plan considered by
the heuristic evaluator is not refinable, this merely reduces the
quality of the heuristic estimate, rather than causing the search to
fail (in the worst case) or spend a long time trying to salvage
non-refinable abstract plans (in the not much better case).



==> helmert06a/search.tex <==
\section{Search}
\label{section:search}

Unlike the translation and knowledge compilation components, for which
there is only a single mode of execution, the search component of Fast
Downward can perform its work in various alternative ways. There are
three basic search algorithms to choose from:

\begin{enumerate}
\item \emph{Greedy best-first search:} This is the standard textbook
  algorithm \cite{russell-norvig}, modified with a technique called
  \emph{deferred heuristic evaluation} to mitigate the negative
  influence of wide branching. We have also extended the algorithm to
  deal with \emph{preferred operators}, similar to FF's helpful
  actions \cite{ff}. We discuss greedy best-first search in Section
  \ref{section:greedy-best-first-search}.  Fast Downward uses this
  algorithm together with the causal graph heuristic, discussed
  in Section \ref{section:cg-heuristic}.
\item \emph{Multi-heuristic best-first search:} This is a variation of
  greedy best-first search which evaluates search states using multiple
  heuristic estimators, maintaining separate open lists for each. Like
  our variant of greedy best-first search, it supports the use of
  \emph{preferred operators}. Multi-heuristic best-first search is
  discussed in Section
  \ref{section:multi-heuristic-best-first-search}. Fast Downward uses
  this algorithm together with the causal graph and FF heuristics,
  discussed in Sections \ref{section:cg-heuristic} and
  \ref{section:ff-heuristic}.
\item \emph{Focused iterative-broadening search:} This is a simple
  search algorithm that does not use heuristic estimators, and instead
  reduces the vast set of search possibilities by focusing on a
  limited operator set derived from the causal graph. It is an
  experimental algorithm; in the future, we hope to further develop
  the basic idea of this algorithm into a more robust method. Focused
  iterative-broadening search is discussed in Section
  \ref{section:focused-iterative-broadening-search}.
\end{enumerate}

For the two heuristic search algorithms, a second choice must be made
regarding the use of \emph{preferred operators}. There are five
options supported by the planner:
\begin{enumerate}
\item Do not use preferred operators.
\item Use the \emph{helpful transitions} of the causal graph heuristic
  as preferred operators.
\item Use the \emph{helpful actions} of the FF heuristic as preferred
  operators.
\item Use helpful transitions as preferred operators, falling back to
  helpful actions if there are no helpful transitions in the current
  search state.
\item Use both helpful transitions and helpful actions as preferred
  operators.
\end{enumerate}

Each of these five options can be combined with any of the two
heuristic search algorithms, so that there is a total of eleven
possible settings for the search component, ten using one of the
heuristic algorithms and one using focused iterative-broadening search.

In addition to these basic settings, the search component can be
configured to execute several alternative configurations in parallel
by making use of an internal scheduler. Both configurations of Fast
Downward that participated in IPC4 made use of this feature by running
one configuration of the heuristic search algorithms in parallel with
focused iterative-broadening search. As its heuristic search
algorithm, the configuration \emph{Fast Downward} employed greedy
best-first search with helpful transitions, falling back to helpful
actions when necessary (option 4.). The configuration \emph{Fast
Diagonally Downward} employed multi-heuristic best-first search using
helpful transitions and helpful actions as preferred operators (option
5.).

To avoid confusion between the complete Fast Downward planning system
and the particular configuration called ``Fast Downward'', we will
refer to the IPC4 planner configurations as \emph{FD} and \emph{FDD}
for the rest of this paper. The name of the planning system as a whole
is never abbreviated.

\subsection{The Causal Graph Heuristic}
\label{section:cg-heuristic}

The \emph{causal graph heuristic} is the centrepiece of Fast
Downward's heuristic search engine. It estimates the cost of reaching
the goal from a given search state by solving a number of subproblems
of the planning task which are derived by looking at small ``windows''
of the (pruned) causal graph.
For some additional intuitions about the design
of the heuristic and a discussion of theoretical aspects, we
refer to the article in which the heuristic was first introduced
\cite{malte-icaps-cg}.

\subsubsection{Conceptual View of the Causal Graph Heuristic}

For each state variable $v$ and each pair of values $d, d' \in
\mathcal D_v$, the causal graph heuristic computes a heuristic estimate
$\textit{cost}_v(d,d')$ for the cost of changing the value of $v$ from
$d$ to $d'$, assuming that all other state variables carry the same
values as in the current state. (This is a simplification. Cost
estimates are not computed for state variables $v$ or values $d$ for
which they are never required. We ignore this fact when discussing the
heuristic on the conceptual level.) The heuristic estimate of a given
state $s$ is the sum over the costs $\textit{cost}_v(s(v),
s_\star(v))$ for all variables $v$ for which a goal condition
$s_\star(v)$ is defined.

Conceptually, cost estimates are computed one variable after the
other, traversing the (pruned) causal graph in a bottom-up fashion.
By bottom-up, we mean that we start with the variables that have no
predecessors in the causal graphs; we call this order of computation
``bottom-up'' because we consider variables that can change their
state of their own accord \emph{low-level}, while variables whose
state transitions require the help of other variables have more
complex transition semantics and are thus considered
\emph{high-level}. Note that in our figures depicting causal graphs,
\emph{high-level} variables are typically displayed near the
\emph{bottom}.

For variables without predecessors in the causal graph,
$\textit{cost}_v(d,d')$ simply equals the cost of a shortest path from
$d$ to $d'$ in the (pruned) domain transition graph $\textit{DTG}(v)$.
For other variables, cost estimates are also computed by graph search
in the domain transition graph. However, the conditions of transitions
must be taken into account during path planning, so that in addition
to counting the number of transitions required to reach the
destination value, we also consider the costs for achieving the value
changes of the other variables necessary to set up the transition
conditions.

The important point here is that in computing the values
$\textit{cost}_v(d,d')$, we completely consider all interactions of
the state variable $v$ with its predecessors in the causal graph. If
changing the value from $d$ to $d'$ requires several steps and each of
these steps has an associated condition on a variable $v'$, then we
realize that $v'$ must assume the values required by those conditions
\emph{in sequence}. For example, if $v$ represents a package in a
transportation task that must be moved from $A$ to $B$ by means of a
vehicle located at $C$, then we recognize that the vehicle must first
move from $C$ to $A$ and then from $A$ to $B$ in order to drop the
package at $B$. This is very different to the way HSP- or FF-based
heuristics work on such examples. However, we only consider
interactions with the \emph{immediate} predecessors of $v$ in the
causal graph. Interactions that occur via several graph layers
are not captured by the heuristic estimator.

In essence, we compute $\textit{cost}_v(d,d')$ by solving a particular
subproblem of the MPT, induced by the variable $v$ and its
predecessors in the pruned causal graph. For this subproblem, we
assume that $v$ is initially set to $d$, we want $v$ to assume the
value $d'$, and all other state variables carry the same value as in
the current state. We call this planning problem the \emph{local
subproblem for $v$, $d$ and $d'$}, or the \emph{local subproblem for
$v$ and $d$} if we leave the target value $d'$ open.

\includefigure{compute-all-costs}{The \emph{compute-costs-bottom-up}
  algorithm, a high-level description of the causal graph heuristic.}

For a formalization of these intuitive notions of how the \emph{cost}
estimates are generated, consider the pseudo-code in
Fig.~\ref{figure:compute-all-costs}. It does not reflect the way the
heuristic values are actually computed within Fast Downward; the
algorithm in the figure would be far too expensive to evaluate for
each search state. However, it computes the same cost values as Fast
Downward does, provided that the algorithm generating the plans
$\pi$ in the last line of the algorithm is the same one as the one
used for the ``real'' cost estimator.

\subsubsection{Computation of the Causal Graph Heuristic}

The actual computation of the causal graph heuristic traverses the causal graph
in a top-down direction starting from the goal variables, rather than
bottom-up starting from variables without causal predecessors. In
fact, this top-down traversal of the causal graph is the reason for
Fast Downward's name.

Computing cost estimates in a top-down traversal implies that while
the algorithm is computing plans for local subproblems of a given
variable, it typically does not yet know the costs for changing the
state of its causal predecessors. The algorithm \emph{compute-costs}
addresses this by evaluating the cost values of dependent variables
through recursive invocations of itself.

For a given variable-value pairing $v=d$, we always compute the costs
$\textit{cost}_v(d,d')$ for all values of $d' \in \mathcal D_v$ at the
same time, similar to the way Dijkstra's algorithm computes the
shortest path not from a single source to a single destination vertex,
but from a single source to all possible destination vertices.
Computing the costs for all values of $d'$ is not (much) more
expensive than computing only one of these values, and once all cost
values have been determined, we can cache them and re-use them if they
are needed again later during other parts of the computation of the
heuristic value for the current state.

In fact, the similarity to shortest path problems is not superficial
but runs quite deeply. If we ignore the recursive calls for computing
cost values of dependent variables, \emph{compute-costs} is basically
an implementation of Dijkstra's algorithm for the single-source
shortest path problem on domain transition graphs. The only difference
to the ``regular'' algorithm lies in the fact that we do not know the
cost for using an arc in advance. Transitions of derived variables
have a base cost of 0 and transitions of fluents have a base cost of
1, but in addition to the base cost, we must pay the cost for
achieving the conditions associated with a transition. However, the
cost for achieving a given condition $v'=e'$ depends on the current
value $e$ of that state variable at the time the transition is taken.
Thus, we can only compute the real cost for a transition once we know
the values of the dependent state variables in the relevant situation.

Of course, there are many different ways of taking transitions through
domain transition graphs, all potentially leading to different values for the
dependent state variables. When we first introduced the causal graph heuristic, we
showed that deciding plan existence for the local subproblems is
\NP-complete \cite{malte-icaps-cg}, so we are content with an approach
that does not lead to a complete planning algorithm, as long as it
works well for the subproblems we face in practice.

The approach we have chosen is to achieve each value of state variable
$v$ in the local subproblem for $v$ and $d$ as quickly as possible,
following a greedy policy. In the context of the Dijkstra algorithm,
this means that we start by finding the cheapest possible plan to
make a transition from $d$ to some other value $d'$. Once we have
found the cheapest possible plan $\pi_{d'}$, we commit to it,
annotating the vertex $d'$ of the domain transition graph with the
local state obtained by applying plan $\pi_{d'}$ to the current state.
In the next step, we look for the cheapest possible plan to achieve
another value $d''$, by either considering transitions that start from
the initial value $d$, or by considering transitions that continue the
plan $\pi_{d'}$ by moving to a neighbour of $d'$. This process is
iterated until all vertices of the domain transition graph have been
reached or no further progress is possible.

\includefigure{compute-costs}{Fast Downward's implementation of the causal graph
  heuristic: the \emph{compute-costs} algorithm for computing the
  estimates $cost_v(d, d')$ for all values $d' \in \mathcal D_v$ in a
  state $s$ of an MPT $\Pi$.}

Our implementation follows Dijkstra's algorithm
(Fig.~\ref{figure:compute-costs}). We have implemented the priority
queue as a vector of buckets for maximal speed and use a cache to
avoid generating the same $\textit{cost}_v(d,d')$ value twice for the
same state. In addition to this, we use a global cache that is shared
throughout the whole planning process so that we need to compute the
values $\textit{cost}_v(d,d')$ for variables $v$ with few ancestors in
the pruned causal graph only once. (Note that $\textit{cost}_v(d,d')$
only depends on the current values of the ancestors of $v$.)

Apart from these and some other technical considerations,
Fig.~\ref{figure:compute-costs} gives an accurate account of Fast
Downward's implementation of the causal graph heuristic. For more details,
including complexity considerations and a worked-out example, we refer
to the original description of the algorithm \cite{malte-icaps-cg}.

\subsubsection{States with Infinite Heuristic Value}

We noted that Fast Downward uses an incomplete planning algorithm
for determining solutions to local planning problems. Therefore, there
can be states $s$ with $\textit{cost}_v(s(v), s_\star(v)) =
\infty$ even though the goal condition $v=s_\star(v)$ can still be
reached. This means that we cannot trust infinite values returned by
the causal graph heuristic. In our experience, states with infinite heuristic
evaluation from which it is still possible to reach the goal are rare,
so we indeed treat such states as \emph{dead ends}.

If it turns out that \emph{all} states at the search frontier are dead
ends, we cannot make further progress with the causal graph heuristic.
In this case, we use a sound dead-end detection routine to verify the
heuristic assessment. If it turns out that all frontier states are
indeed dead ends, then we report the problem as unsolvable. Otherwise,
search is restarted with the FF heuristic (cf.~Section
\ref{section:ff-heuristic}), which is sound for purposes of dead-end
detection.\footnote{In practice, we have never observed the causal
graph heuristic to fail on a solvable task. Therefore, the fallback
mechanism is only used for some unsolvable tasks in the {\miconicfull}
domain which are not recognized by our dead-end detection technique.}

The dead-end detection routine has been originally developed for
STRIPS-like tasks. However, extending it to full MPTs is easy; in
fact, no changes to the core algorithm are required, as it works at
the level of domain transition graphs and is still sound when applied
to tasks with conditional effects and axioms. Since it is not a
central aspect of Fast Downward, we do not discuss it here, referring
to our earlier work instead \cite{malte-icaps-cg}.

\subsubsection{Helpful Transitions}

Inspired by Hoffmann's very successful use of \emph{helpful actions}
within the FF planner \cite{ff}, we have extended our algorithm for
computing the causal graph heuristic so that in addition to the heuristic
estimate, it also generates a set of applicable operators considered
useful for steering search towards the goal.

To compute helpful actions in FF, Hoffmann's algorithm generates a
plan for the relaxed planning task defined by the current search state
and considers those operators \emph{helpful} which belong to the
relaxed plan and are applicable in the current state.

Our approach follows a similar idea. After computing the heuristic
estimate $\textit{cost}_v(s(v), s_\star(v))$ for a variable $v$ for
which a goal condition is defined, we look into the domain transition
graph of $v$ to trace the path of transitions leading from $s(v)$ to
$s_\star(v)$ that gave rise to the cost estimate. In particular, we
consider the first transition on this path, starting at $s(v)$. If
this transition corresponds to an applicable operator, we consider
that operator a \emph{helpful transition} and continue to check the
next goal. If the transition does not correspond to an applicable
operator because it has associated conditions of the form $v'=e'$
which are not currently satisfied, then we recursively look for
helpful transitions in the domain transition graph of each such
variable $v'$, checking the path that was generated during the
computation of $\textit{cost}_{v'}(s(v'), e')$.

The recursive process continues until we have found all helpful
transitions. Unlike the case for FF, where helpful actions can be
found for all non-goal states, we might not find any helpful
transition at all. It may be the case that a transition does not
correspond to an applicable operator even though it has no associated
conditions; this can happen when some operator preconditions are not
represented in the pruned domain transition graph due to cycles in the
causal graph. Even so, we have found helpful transitions to be a
useful tool in guiding our best-first search algorithms.

\subsection{The FF Heuristic}
\label{section:ff-heuristic}

The \emph{FF heuristic} is named after Hoffmann's planning algorithm
of the same name, in the context of which it was originally introduced
\cite{ff}. It is based on the notion of \emph{relaxed planning tasks}
that ignore \emph{negative interactions}. In the context of MPTs,
ignoring negative interactions means that we assume that each state
variable can hold several values simultaneously. An operator effect or
axiom that sets a variable $v$ to a value $d$ in the original task
corresponds to an effect or axiom that \emph{adds} the value $d$ to
the range of values assumed by $v$ in the relaxed task. A condition
$v=d$ in the original task corresponds to a condition requiring $d$ to
be an element of the set of values currently assumed by $v$ in the
relaxed task.

It is easy to see that applying some operator in a solvable relaxed
planning task can never render it unsolvable. It can only lead to more
operators being applicable and more goals being true, if it has any
significant effect at all. For this reason, relaxed planning tasks can
be solved efficiently, even though optimal solutions are still
\NP-hard to compute \cite{complexity-bylander}. A plan for the
relaxation of a planning task is called a \emph{relaxed plan} for
that task.

The FF heuristic estimates the goal distance of a world state by
generating a relaxed plan for the task of reaching the goal from this
world state. The number of operators in the generated plan is then used as the
heuristic estimate. Our implementation of the FF heuristic does not
necessarily generate the same, or even an equally long, relaxed plan
as FF. In our experiments, this did not turn out to be problematic, as
both implementations appear to be equally informative.

While the FF heuristic was originally introduced for ADL domains,
extending it to tasks involving derived predicates is
straight-forward. One possible extension is to simply assume that each
derived predicate is initially set to its default value $\bot$ and
treat axioms as relaxed operators of cost 0. In a slightly more
complicated, but also more accurate approach, derived variables are
initialized to their actual value in a given world state, allowing the
relaxed planner to achieve the value $\bot$ (or other values) by
applying the transitions of the extended domain transition graph of
the derived variable. We have followed the second approach.

In addition to heuristic estimates, the FF heuristic can also be
exploited for restricting or biasing the choice of operators to apply
in a given world state $s$. The set of \emph{helpful actions} of $s$
consists of all those operators of the relaxed plan computed for $s$
that are applicable in that state. As mentioned in the introduction to
this section, Fast Downward can be configured to treat helpful actions
as preferred operators.

There is a wealth of work on the FF heuristic in the literature, so we
do not discuss it further. For a more thorough treatment, we 
point to the references
\cite{ff,joerg-topology,hoffmann:aips-02,hoffmann:jair2005}.

\subsection{Greedy Best-First Search in Fast Downward}
\label{section:greedy-best-first-search}

Fast Downward uses \emph{greedy best-first search with a closed list}
as its default search algorithm. We assume that the reader is familiar
with the algorithm and refer to the literature for details
\cite{russell-norvig}.

Our implementation of greedy best-first search differs from the
textbook algorithm in two ways. First, it can treat helpful
transitions computed by the causal graph heuristic or helpful actions
computed by the FF heuristic as \emph{preferred operators}. Second, it
performs \emph{deferred heuristic evaluation} to reduce the influence
of large branching factors. We now turn to describing these two search
enhancements.

\subsubsection{Preferred Operators}

To make use of helpful transitions computed by the causal graph heuristic
or helpful actions computed by the FF heuristic, our variant of
greedy best-first search supports the use of so-called \emph{preferred
operators}.
The set of preferred operators of a given state is a subset of the set
of applicable operators for this state. Which operators are considered
preferred depends on the settings for the search component, as
discussed earlier. The intuition behind preferred operators is that a
randomly picked successor state is more likely to be closer to the
goal if it is generated by a preferred operator, in which case we call
it a \emph{preferred successor}. Preferred successors should be
considered before non-preferred ones on average.

Our search algorithm implements this preference by maintaining two
separate open lists, one containing \emph{all} successors of expanded
states and one containing \emph{preferred} successors exclusively. The search
algorithm alternates between expanding a regular successor and a
preferred successor. On even iterations it will consider the one open
list, on odd iterations the other. No matter which open list a state
is taken from, all its successors are placed in the first open list,
and the preferred successors are additionally placed in the second
open list.  (Of course we could limit the first open list to only
contain non-preferred successors; however, typically the total number
of successors is vast and the number of preferred successors is tiny.
Therefore, it is cheaper to add all successors to the first open list
and detect duplicates upon expansion than scan through the list of
successors determining for each element whether or not it is
preferred.)

Since the number of preferred successors is smaller than the total
number of successors, this means that preferred successors are
typically expanded much earlier than others. This is especially
important in domains where heuristic guidance is weak and a lot of
time is spent exploring plateaus. When faced with plateaus, Fast
Downward's open lists operate in a first-in-first-out fashion. (In
other words: For a constant heuristic function, our search algorithm
behaves like breadth-first search.) Preferred operators typically
offer much better chances of escaping from plateaus since they lead
to significantly lower effective branching factors.

\subsubsection{Deferred Heuristic Evaluation}

Upon expanding a state $s$, the textbook version of greedy best-first
search computes the heuristic evaluation of all successor states of
$s$ and sorts them into the open list accordingly. This can be
wasteful if $s$ has many successors and heuristic evaluations are
costly, two conditions that are often true for heuristic search
approaches to planning.

This is where our second modification comes into play. If a successor
with a better heuristic estimate than $s$ is generated early and leads
to a promising path towards the goal, we would like to avoid
generating the other successors. Let us assume that $s$ has 1000
successors, and that $s'$, the 10th successor of $s$ being generated,
has a better heuristic estimate than $s$. Furthermore, let us assume
that the goal can be reached from $s'$ on a path with non-increasing
heuristic estimates. Then we would like to avoid computing heuristic
values for the 990 later successors of $s$ altogether.

Deferred heuristic evaluation achieves this by \emph{not} computing
heuristic estimates for the successors of an expanded state $s$
immediately. Instead, the successors of $s$ are placed in the open
list together with the heuristic estimate \emph{of state $s$}, and
their own heuristic estimates are only computed when and if they are
expanded, at which time it is used for sorting \emph{their} successors
into the open list, and so on. In general, each state is sorted into
the open list according to the heuristic evaluation of its parent,
with the initial state being an exception. In fact, we do not need to
put the successor state itself into the open list, since we do not
require its representation before we want to evaluate its heuristic
estimate. Instead, we save memory by storing only a reference to the
parent state and the operator transforming the parent state into the
successor state in the open list.

It might not be clear how this approach can lead to significant
savings in time, since deferred evaluation also means that information
is only available later. The potential savings become most apparent
when considering deferred heuristic evaluation together with the use
of preferred operators: If an improving successor $s'$ of a state $s$
is reached by a preferred operator, it is likely that it will be
expanded (via the second open list) long before most other successors
--- or even most siblings --- of $s$. In the situation described
above, where there exists a non-increasing path from $s'$ to the goal,
heuristic evaluations will never be computed for most successors of
$s$. In fact, deferred heuristic evaluation can significantly improve
search performance even when preferred operators are not used,
especially in tasks where branching factors are large and the
heuristic estimate is informative.

At first glance, deferred heuristic evaluation might appear related to
another technique for reducing the effort of expanding a node within a
best-first search algorithm, namely A${}^*$ with Partial Expansion
\cite{astar-partial-expansion}. However, this algorithm is designed
for reducing the \emph{space} requirements of best-first search at the
expense of additional heuristic evaluations: When expanding a node,
A${}^*$ with Partial Expansion computes the heuristic value of
\emph{all} successors, but only stores those in the open queue whose
heuristic values fall below a certain \emph{relevance threshold}. In
later iterations, it might turn out that the threshold was chosen too
low, in which case the node needs to be re-expanded and the heuristic
values of its successors re-evaluated. In general, A${}^*$ with
Partial Expansion will never compute fewer heuristic estimates than
standard A${}^*$, but it will usually require less memory.

However, for heuristic search approaches to planning (and certainly
for Fast Downward), heuristic evaluations are usually so costly in
time that memory for storing open and closed lists is not a limiting
factor. We are thus willing to trade off memory with time in the
opposite way: Deferred heuristic evaluation normally leads to more
node expansions and higher space requirements than standard best-first
search because the heuristic values used for guiding the search are
less informative (they evaluate the predecessor of a search node
rather than the node itself). However, heuristic computations are only
required for nodes that are actually removed from the open queue
rather than for all nodes on the fringe, and the latter are usually
significantly more numerous.

\subsection{Multi-Heuristic Best-First Search}
\label{section:multi-heuristic-best-first-search}

As an alternative to greedy best-first search, Fast Downward supports
an extended algorithm called \emph{multi-heuristic best-first search}.
This algorithm differs from greedy best-first search in its use of
multiple heuristic estimators, based on our observation that different
heuristic estimators have different weaknesses. It may be the case
that a given heuristic is sufficient for directing the search towards
the goal except for one part of the plan, where it gets stuck on a
plateau. Another heuristic might have similar characteristics, but get
stuck in another part of the search space.

Various ways of combining heuristics have been proposed in the
literature, typically adding together or taking the maximum of the
individual heuristic estimates. We believe that it is often beneficial
\emph{not} to combine the different heuristic estimates into a single
numerical value. Instead, we propose maintaining a \emph{separate} open list
for each heuristic estimator, which is sorted according to the
respective heuristic. The search algorithm alternates between
expanding a state from each open list. Whenever a state is expanded,
estimates are calculated according to \emph{each} heuristic, and the
successors are put into each open list.

When Fast Downward is configured to use multi-heuristic best-first
search, it computes estimates both for the causal graph heuristic and FF
heuristic, maintaining two open lists. Of course, the approach can be
combined with the use of preferred operators; in this case, the search
algorithm maintains four open lists, as each heuristic distinguishes
between normal and preferred successors.

\subsection{Focused Iterative-Broadening Search}
\label{section:focused-iterative-broadening-search}

The \emph{focused iterative-broadening search} algorithm is the most
experimental piece of Fast Downward's search arsenal. In its present
form, the algorithm is unsuitable for many planning domains,
especially those containing comparatively few different goals. Yet we
think that it might contain the nucleus for a successful approach to
domain-independent planning which is very different to most current
methods, so we include it for completeness and as a source of
inspiration.

The algorithm is intended as a first step towards developing search
techniques that emphasize the idea of using heuristic criteria
locally, for limiting the set of operators to apply, rather than
globally, for choosing which states to expand from a global set of
open states. We made first experiments in this direction after
observing the large boost in performance that can be obtained by using
preferred operators in heuristic search. The algorithm performed
surprisingly well in some of the standard benchmark domains, while
performing badly in most others.

As the name suggests, the algorithm \emph{focuses} the search by
concentrating on one goal at a time, and by restricting its attention
to operators which are supposedly important for reaching that goal:

\begin{definition}{distance}{Modification distances}
Let $\Pi$ be an MPT, let $o$ be an operator of $\Pi$, and let $v$ be a
variable of $\Pi$.

The \definedTerm{modification distance} of $o$ with respect to $v$ is
defined as the minimum, over all variables $v'$ that occur as affected
variables in the effect list of $o$, of the distance from $v'$ to $v$ in
$\textit{CG}(\Pi)$.
\end{definition}

For example, operators that modify $v$ directly have a modification
distance of 0 with respect to $v$, operators that modify variables
which occur in preconditions of operators modifying $v$ have a
modification distance of 1, and so on. We assume that in order to
change the value of a variable, operators with a low modification
distance with respect to this variable are most useful.

\includefigure{reach-one-goal}{The \emph{reach-one-goal}
  procedure for reaching a state with $v=d$. The value
  \emph{max-threshold} is equal to the maximal modification distance
  of any operator with respect to $v$.}

Fig.~\ref{figure:reach-one-goal} shows the \emph{reach-one-goal}
procedure for achieving a single goal of an MPT. For the time being,
assume that the $\cond$ parameter is always $\emptyset$. The procedure
makes use of the assumption that high modification distance implies
low usefulness in two ways. First, operators with high modification
distance with respect to the goal variable are considered to have a
higher associated cost, and are hence applied less frequently. Second,
operators whose modification distance is beyond a certain threshold
are forbidden completely. Instead of choosing a threshold a priori,
the algorithm first tries to find a solution with the lowest possible
threshold of 0, increasing the threshold by 1 whenever the previous
search has failed. The \emph{uniform-cost-search} algorithm mentioned
in Fig.~\ref{figure:reach-one-goal} is the standard textbook method
\cite{russell-norvig}.

Although we were ignorant of this fact at the time our algorithm was
conceived, the core idea of \emph{reach-one-goal} is not new: Ginsberg
and Harvey \citeyear{ginsberg-harvey:aij92} present a search technique
called \emph{iterative broadening}, which is also based on the idea of
repeatedly doing a sequence of uninformed searches with an
ever-growing set of operators. Their work demonstrates the superiority
of iterative broadening over standard depth-bounded search both
empirically and analytically under the reasonable assumption that the
choices made at each branching point are equally
important.\footnote{See the original analysis for a precise definition
  of ``equally important'' \cite{ginsberg-harvey:aij92}. While
  Ginsberg and Harvey's assumption is certainly not valid in practice,
  we find it much more convincing than the competing model where goal
  states are uniformly distributed across the search fringe.} The
original iterative broadening algorithm applies to scenarios without
any knowledge of the problem domain, so it chooses the set of
operators which may be applied at every search node randomly, rather
than using heuristic information from the causal graph as in our case.
However, Ginsberg and Harvey already discuss the potential
incorporation of heuristics into the operator selection. The
introduction of operator costs (in the form of modification distances)
is new, but it is a fairly straightforward extension where heuristic
information is available.

The focused iterative-broadening search algorithm is based on the
\emph{reach-one-goal} method; the idea is to achieve the goals of the
planning task one after the other, by using the \emph{reach-one-goal}
algorithm as the core subroutine for satisfying individual goals.
Since it is not obvious what a good order of achieving the goals would
be, one invocation of \emph{reach-one-goal} is started for each goal
in parallel. As each one-goal solver focuses on the (supposedly)
relevant operators for reaching its particular goal, there is hope
that the number of states considered before a goal is reached is
small. Once one of the one-goal solvers reaches its goal, the
resulting plan is reported and all sub-searches are stopped. The
overall search algorithm commits to this part of the plan; the
situation in which the first goal has been reached is considered a new
initial state.

From this situation, we try to satisfy the second goal, by once more
starting parallel invocations of \emph{reach-one-goal} for
each possible second goal. Of course, this can lead to a situation
where the search algorithm oscillates between goals, first achieving 
goal $a$, then abandoning it in favour of goal $b$, without any sign of
making real progress. Therefore, we demand that \emph{reach-one-goal}
achieves the second goal \emph{in addition} to the one we reached
first, by setting the $\cond$ argument accordingly. Once two goals
have been reached, the sub-searches are again stopped,
sub-searches for the third goal are started, and so on, until all
goals have been reached.

In some sense, our focusing technique is similar to the beam search
algorithm \cite{beam-search}, which also performs a fixed number of
concurrent searches to avoid committing to a particular path in the
search space too early. Beam search uses a heuristic function to
evaluate which branches of search should be abandoned and where new
branches should be spawned. While focused iterative-broadening search
does not appear to use heuristic evaluations at first glance, the
number of satisfied goals of a state is used as an evaluation
criterion in essentially the same way. One important difference to
beam search is our use of modification distances relative to a
particular goal, which means that the different ``beams'' explore the
state space in qualitatively different ways.

There is one final twist: To motivate \emph{reach-one-goal} not to
needlessly wander away from satisfied goals, we forbid applying
operators that undo any of the previously achieved goals in $\cond$.
This is an old idea called \emph{goal protection}
\cite{joslin-roach:aij89}. It is well-known that protecting goals
renders a search algorithm incomplete, even in state spaces where all
operators are reversible and local search approaches like focused
iterative-broadening search would be otherwise complete. In
particular, search must fail in planning tasks which are not
\emph{serializable} \cite{korf:aij-1987}. Therefore, if the first
solution attempt fails, the algorithm is restarted without
goal protection. The complete procedure is shown in
Fig.~\ref{figure:reach-one-goal-complete}, which concludes our
discussion of Fast Downward's search component.

\includefigure{reach-one-goal-complete}{The \emph{reach-one-goal}
  procedure for reaching a state with $v=d$ (corrected).}


==> hoffmann05a/Airport.tex <==






\subsection{Airport}
\label{results:airport}



In the Airport domain, the planner has to control the ground traffic
on an airport. The task is to find a plan that solves a specific
traffic situation, specifying inbound and outbound planes along with
their current and goal positions on the airport. The planes must not
endanger each other, i.e. they must not both occupy the same airport
``segment'' (a smallest road unit), and if plane $x$ drives behind
plane $y$ then between $x$ and $y$ there must be a safety distance
(depending on the size of $y$). These safety constraints are modelled
in terms of ``blocked'' and ``occupied'' predicates, whose value is
updated and controlled via complex ADL preconditions and conditional
effects.


There were four different versions of the domain in IPC-4: a
non-temporal version, a temporal version, a temporal version with time
windows, and a temporal version with compiled time windows. The time
windows in the latter two versions concern airplanes that are known to
land in the future, and that will thus block certain airport segments
(runways) during certain time windows. The time windows are modelled
using timed initial literals, respectively their compilation. In every
domain version, there is an ADL formulation, as well as a STRIPS
formulation obtained by compiling the ADL constructs away (resulting
in a partially grounded encoding).


Instances scale in terms of the size of the underlying airport, as
well as the number of airplanes that must be moved. One remarkable
thing about the Airport domain is that the instances were generated
based on a professional airport simulation tool. The largest instances
used in IPC-4 (number 36 to 50) correspond to a real airport, namely
Munich airport (MUC). Instance number 50 encodes a traffic situation
with 15 moving airplanes, which is typical of the situations
encountered at MUC in reality. Instances number 1 to 20 come from
smaller toy airports, instances number 21 to 35 are based on one half
of MUC airport.



\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/AIRPORT/NONTEMPORAL/GNUPLOT/Time-suboptimal-1.eps} &
\includegraphics[width=7.3cm]{RESULTS/AIRPORT/NONTEMPORAL/GNUPLOT/Time-suboptimal-2.eps}\\
(a) & (b)
\end{tabular}
\includegraphics[width=7.3cm]{RESULTS/AIRPORT/NONTEMPORAL/GNUPLOT/Time-optimal.eps}\\
(c)
\vspace{-0.0cm}
\caption{Performance in non-temporal Airport, satisficing (a) and (b), optimal (c).}
\label{airport:nontemporal}
\vspace{-0.0cm}
\end{center}
\end{figure}




Figure~\ref{airport:nontemporal} shows the runtime performance in the
non-temporal version of the domain. For readability, the set of satisficing
planners is split over two graphs. As will be the case in all graphs
displayed in the subsequent discussions, the $x$-axis denotes the
instance number (obviously, the higher the number the larger the
instance), and the $y$-axis gives CPU runtime in seconds on a
logarithmic scale. CPU time is total, including parsing and any form
of static pre-processing.



It can be observed in Figure~\ref{airport:nontemporal} that FDD is the
only planner solving all problem instances. LPG-TD and SGPlan both
scale relatively well, but fail on the largest instances. The other
planners all behave much more unreliably. Observe also that the IPC-3
version of LPG lags far behind FDD, LPG-TD, and SGPlan. For the
optimal planners, which unsurprisingly behave clearly worse than the
satisficing planners, the only clear-cut observation is a performance
advantage for SATPLAN. The other optimal planners all behave
relatively similarly; Semsyn and BFHSP are the only ones out of that
group solving a few of the larger instances.


For plan quality, there are two groups of planners, one trying to
minimize the number of actions, and one trying to minimize makespan,
i.e. the number of parallel action {\em steps}. In the former group,
the plan quality performance differences are moderate. CRIKEY, LPG-TD,
SGPlan, and YAHSP sometimes find sub-optimal plans. FDD's plans are
optimal in all cases where an optimal planner found a solution. As a
measure of comparative plan quality, from now on we provide, given
planners A and B, the min, mean, and maximum of the ratio quality(A)
divided by quality(B), for all instances that are solved by both A and
B. We call this data the ``ratio A vs B''. For CRIKEY (A) vs FDD (B),
the ratio is $0.91$ (min), $1.04$ (mean), and $1.45$ (max), $[0.91
(1.04) 1.45]$ for short. For LPG-TD.speed vs FDD the ratio is $[0.91
(1.08) 1.80]$; for LPG-TD.quality vs FDD it is $[0.91 (1.06) 1.80]$.
For SGPlan vs FDD it is $[0.91 (1.07) 2.08]$; for YAHSP vs FDD it is
$[0.91 (1.07) 1.43]$.


In the group of planners minimizing makespan, (only) Marvin has a
tendency to find very long plans. The comparison Marvin vs the optimal
SATPLAN is $[1.00 (2.46) 4.64]$. In the maximum case, SATPLAN finds a
plan with 53 steps, and Marvin's plan is 246 steps long.




An interesting observation concerns the two scaling parameters of that
domain: the number of airplanes, and the size of the airport. In all
the plots in Figure~\ref{airport:nontemporal}, and also in most plots
in Figure~\ref{airport:temporal} below, one can observe that the
instances number 26 to 35 become increasingly hard for the planners --
but in the step to instance number 36, the performance suddenly
becomes better again. As said above, the instances 21 to 35 are based
on one half of MUC airport, while the instances 36 to 50 are based on
the full MUC airport. But between instances 26 and 35, the number of
airplanes rises from 6 to 12; instance 36 contains only 2 airplanes,
instances 37 and 38 contain 3.  That is, it is easier for the planners
to address a larger airport with fewer planes. Note here the domain
combinatorics: the number of reachable states is in the order of
$S^n$, where $S$ is the number of different airport segments, and $n$
is the number of airplanes.





\begin{figure}[htb]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/AIRPORT/TEMPORAL/GNUPLOT/Time-suboptimal.eps} &
\includegraphics[width=7.3cm]{RESULTS/AIRPORT/TEMPORAL/GNUPLOT/Time-optimal.eps}\\
(a) & (b)\\
\includegraphics[width=7.3cm]{RESULTS/AIRPORT/TEMPORAL_TIMEWINDOWS/GNUPLOT/Time-suboptimal.eps} &
\includegraphics[width=7.3cm]{RESULTS/AIRPORT/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT/Time-suboptimal.eps}\\
(c) & (d)
\end{tabular}
\vspace{-0.0cm}
\caption{Performance in temporal Airport, satisficing (a) and optimal (b). In temporal Airport
  with time windows, satisficing, explicit encoding (c) and compiled
  encoding (d).}
\label{airport:temporal}
\vspace{0.0cm}
\end{center}
\end{figure}


Figure~\ref{airport:temporal} shows the runtime performance in the
temporal versions of the domain. We first consider the domain versions
without time windows: parts (a) and (b) of the figure. Of the
satisficing planners, LPG-TD and SGPlan both scale just as well as
they do in the non-temporal case; all other satisficing planners scale
orders of magnitude worse. Of the optimal planners, CPT scales best,
followed by TP4. The two planners minimizing the number of actions are
SGPlan and CRIKEY; SGPlan behaves somewhat worse, the ratio is $[0.95
(1.03) 1.54]$. Of the planners that minimize makespan, only LPG-TD
scales beyond the smallest instances. The ratio LPG-TD.speed vs the
optimal CPT is $[1.00 (1.15) 1.70]$, P-MEP vs CPT is $[1.00 (1.11)
1.42]$. The ratio LPG-TD.quality vs CPT is $[1.00 (1.03) 1.44]$.



No optimal planner in the competition could handle timed initial
literals, so with explicit time windows no such planner participated.
With compiled time windows, only CPT participated, scaling a little
worse than in the temporal domain version without time windows. For
the satisficing planners, the results are more interesting. With
explicit time windows, again LPG-TD and SGPlan maintain their good
scaling behavior from the simpler domain versions. To the other
planners, there is a huge runtime performance gap. SGPlan is the only
planner here that minimizes the number of actions. The makespan ratio
LPG-TD.speed vs LPG-TD.quality is $[1.00 (1.15) 2.01]$. With compiled time
windows, only SGPlan and CRIKEY participated. The former consistently
solves the smaller instances up to a certain size, the latter fails on
many of the small instances but can solve a few of the larger ones.
Neither of the planners shows reasonable runtime performance compared
to the explicit encoding of the domain. The number of actions ratio
CRIKEY vs SGPlan is $[1.00 (1.14) 1.36]$.



Our main motivation for including the Airport domain in IPC-4 was that
we were able to model it quite realistically, and to generate quite
realistic test instances -- the only thing we could not model was the
real optimization criterion (which asks to minimize the summed up
travel time of all airplanes). So the good scaling results of, at
least, the satisficing planners, are encouraging. Note, however, that
in reality the optimization criterion is of crucial importance, and
really the only reason for using a computer to control the traffic.

We remark that the domain is not overly difficult from the perspective
of relaxed-plan based heuristic planners (using the wide-spread
``ignore deletes'' relaxation). \citeA{hoffmann:jair-05} shows that
Airport instances can contain unrecognized dead ends (states from
which the goal can't be reached, but from which there is a relaxed
plan); but such states are not likely to occur very often. A dead end
in Airport can only occur when two planes block each other, trying to
get across the same segment in different directions. Due to the
topology of the airports (with one-way roads), this can happen only in
densely populated parking regions.  In case for any two airplanes the
respective paths to the goal position are disjoint, the length of a
relaxed plan provides the {\em exact} distance to the nearest goal
state. In that sense, the good runtime performance of the satisficing
planners didn't come entirely unexpected to us, though we did not
expect them to behave {\em that} well. Note that most of these
planners, particularly FDD, SGPlan, and LPG-TD, do much more than/do
things different from a standard heuristic search with goal distances
estimated by relaxed plan length.  Note also that
\citeA{hoffmann:jair-05}'s results are specific to {\em non-temporal}
domains.





In the non-temporal domain version, we awarded 1st places to FDD (and
FD) and SATPLAN; we awarded 2nd places to LPG-TD, SGPlan, Semsyn,
and BFHSP. In the temporal version, we awarded 1st places to LPG-TD,
SGPlan, and CPT; a 2nd place was awarded to TP4. In the domain version
with explicit time windows, 1st places were awarded to LPG-TD and
SGPlan.




==> hoffmann05a/PSR.tex <==







\subsection{PSR}
\label{results:psr}







PSR is short for {\em Power Supply Restoration}. The domain is a PDDL
adaptation of an application domain investigated by Sylvie Thi\'ebaux
and other researchers
\cite{thiebaux:etal:uai-96,thiebaux:cordier:ecp-01}, which deals with
reconfiguring a faulty power distribution system to resupply customers
affected by the faults. In the original PSR problem, various numerical
parameters such as breakdown costs and power margins need to be
optimized, subject to power capacity constraints.  Furthermore, the
location of the faults and the current network configuration are only
partially observable, which leads to a tradeoff between acting to
resupply lines and acting to reduce uncertainty.  In contrast, the
version used for IPC-4 is set up as a pure goal-achievement problem,
numerical aspects are ignored, and total observability is assumed.
Temporality is not a significant aspect even in the original
application, and the IPC-4 domain is non-temporal.



We used four domain versions of PSR in IPC-4. Primarily, these
versions differ by the size of the problem instances encoded. The
instance size determined in what languages we were able to formulate
the domain version. The domain versions are named 1. {\em large}, 2.
{\em middle}, 3. {\em middle-compiled}, and 4. {\em small}. Version 1
has the single formulation {\em adl-derivedpredicates}: in the most
natural formulation, the domain comes with derived predicates to model
the flow of electricity through the network, and with ADL formulas to
express the necessary conditions on the status of the network
connectors. Version 2 has the formulations {\em
  adl-derivedpredicates}, {\em simpleadl-derivedpredicates}, and {\em
  strips-derivedpredicates}.  Version 3 has the single formulation
{\em adl}, and version 4 has the single formulation {\em strips}. As
indicated, the formulation names simply give the language used. In
version 2, ADL constructs were compiled away to obtain the simpler
formulations. In version 3, derived predicates were compiled away by
introducing additional artificial actions; due to the increase in plan
length (which we discuss in some detail further below), we turned this
into a separate domain version, rather than a formulation. As for the
{\em strips}\ domain version, to enable encoding of reasonably-sized
instances for this we adopted a different fully-grounded encoding
inspired by the work of \citeA{bertoli:etal:ecai-02}. The encoding is
generated from a description of the problem instance by a tool
performing some of the reasoning devoted to the planner under the
other domain versions.  Still we were only able to formulate
comparatively small instances in pure STRIPS.






\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/PSR/SMALL/GNUPLOT/Time-suboptimal-1.eps} &
\includegraphics[width=7.3cm]{RESULTS/PSR/SMALL/GNUPLOT/Time-suboptimal-2.eps} \\
(a) & (b) \\
\includegraphics[width=7.3cm]{RESULTS/PSR/SMALL/GNUPLOT/Time-optimal-1.eps} &
\includegraphics[width=7.3cm]{RESULTS/PSR/SMALL/GNUPLOT/Time-optimal-2.eps} \\
(c) & (d)
\end{tabular}
\caption{PSR \emph{small}, satisficing (a) and (b), optimal (c) and (d).}
\label{psr:small}
\end{center}
\vspace{-0.0cm}
\end{figure}



Starting with the performance in the smallest instances, we depict the
performance of satisficing and optimal planners in the PSR STRIPS
domain in Figure~\ref{psr:small}. Both result graphs are divided into
two because they are completely unreadable otherwise. Most planners
show a lot of variance in this domain, blurring the performance
differences (observable) between the individual systems. Still it is
possible to identify systems that behave better than others. Of the
satisficing systems, only FDD can solve all the 50 instances; it does
so consistently fast (the results for FD are almost identical). Of the
other planners, LPG-TD, SGPlan, and YAHSP have the best success ratio:
they solve 49, 47, and 48 instances, respectively; CRIKEY solves 29
instances, Marvin 41. As for the optimal systems, here the only system
solving the entire test suite is SATPLAN. BFHSP solved 48 instances,
CPT 44, HSP$_a^*$ 44, Optiplan 29, Semsyn 40, TP4 38.



For plan quality, once again there are groups of planners trying to
minimize plan length (number of actions), and makespan. In the former
group, we take as a performance measure the plans found by BFHSP,
which are optimal in that sense, and which, as said above, we have for
all but 2 of the 50 instances. The ratio CRIKEY vs BFHSP is $[1.00
(1.72) 3.44]$; the ratio FDD vs BFHSP is $[1.00 (1.02) 1.52]$; the
ratio LPG-TD.speed vs BFHSP is $[1.00 (5.52) 12.70]$; the ratio
LPG-TD.quality vs BFHSP is $[1.00 (1.82) 8.32]$; the ratio SGPlan vs
BFHSP is $[1.00 (1.01) 1.24]$; the ratio YAHSP vs BFHSP is $[1.00
(1.00) 1.05]$. In the planner group minimizing makespan, all planners
except Marvin are optimal. The ratio Marvin vs SATPLAN is $[1.00
(1.28) 2.07]$.


Apart from the observations to be made within the groups of
satisficing respectively optimal planners, there is something to be
said here on the relationship between these two groups. Like in
Dining-Philosophers, we have the rather unusual situation that the
optimal planners are just as efficient as the satisficing ones.
Indeed, by solving all instances, SATPLAN is superior to most of the
satisficing planners. We remark at this point that
\citeA{hoffmann:jair-05} shows the existence of arbitrarily deep local
minima in PSR, i.e., regions where it takes arbitrarily many step to
escape a local minimum under relaxed plan distances. For example,
local minima arise naturally because a relaxed plan is able to supply
{\em and} not supply a line at the same time, and thereby does not
have to make the crucial distinction between faulty and non-faulty
lines.  Now, these observations hold for the {\em original} domain
formulation, with derived predicates and ADL constructs. As said, the
IPC-4 STRIPS formulation of PSR is obtained from that by a combination
of complicated pre-processing machines. These are not likely to make
the real structure of the domain more amenable to relaxed plan
distances. While the satisficing planners participating in PSR {\em
  small} are by no means exclusively dependent on relaxed plan
distances, for most of them these distances do form an important part
of the search heuristics.





\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/PSR/MIDDLE/GNUPLOT/Time-suboptimal-all.eps} & 
\includegraphics[width=7.3cm]{RESULTS/PSR/LARGE/GNUPLOT/Time-suboptimal-all.eps} \\
(a) & (b)
\end{tabular}
\caption{PSR, \emph{middle} (a) and \emph{large} (b), satisficing planners.}
\label{psr:middle-large}
\end{center}
\vspace{-0.0cm}
\end{figure}




Figure~\ref{psr:middle-large} gives the results for the PSR domain
versions, {\em middle} and {\em large}, with larger instances, encoded
with ADL constructs and/or derived predicates. No optimal planner
could handle these language constructs, so unfortunately the above
comparison between the two groups can not be continued. In the middle
sized instances, FDD, SGPlan, and LPG-TD all scale through the entire
test suite. FDD indicates better scaling behavior in the largest
instances. In the domain version with large instances (available only
in a formulation using ADL), FDD indeed shows that it outperforms the
other planners (at least, SGPlan, that also participates here) by far.
The data for FD is almost identical to that for FDD.


Regarding plan quality, the only participating planner in each of {\em
  middle} and {\em large} that tries to minimize makespan is Marvin,
so we have no basis for a comparison.  Of the other planners, SGPlan
generally finds the plans with the smallest number of actions.
Precisely, in the {\em middle} version the plan quality ratios are as
follows. The ratio FDD vs SGPlan is $[0.67 (1.23) 2.33]$ (FD: $[0.67 (1.25)
2.85]$). The ratio LPG-TD.speed vs SGPlan is $[0.67 (1.82) 7.27]$; the
maximum case is instance number 49, where LPG-TD.speed takes 80 steps
and SGPlan 11. The ratio LPG-TD.quality vs SGPlan is $[0.60 (1.08) 7.27]$,
with the same maximum case. In the {\em large} version, only FD and
FDD solve a considerable number of instances; the ratio FD vs FDD is
$[0.60 (1.01) 1.30]$.


In the PSR domain version with middle-size instances and derived
predicates compiled into ADL, i.e., in domain version {\em
  middle-compiled}, only Macro-FF and SGPlan participated.  Macro-FF
scaled relatively well, solving 32 instances up to instance number 48.
SGPlan solved only 14 instances up to instance number 19. Both
planners try to minimize the number of actions, and the ratio SGPlan
vs Macro-FF is $[0.51 (1.28) 1.91]$.


It is interesting to observe that, in PSR, when compiling derived
predicates away, the plan length increases much more than what we have
seen in Section~\ref{results:promela} for Dining-Philosophers and
Optical-Telegraph. In the latter, the derived predicates just replace
two action applications per process, detecting that the respective
process is blocked. In PSR, however, as said the derived predicates
model the flow of electricity through the network, i.e., they encode
the transitive closure of the underlying graph. The number of
additional actions needed to simulate the latter grows, of course,
with the size of the graph. This phenomenon can be observed in the
IPC-4 plan length data. The PSR {\em middle-compiled} instances are
identical to the {\em middle} instances, except for the compilation of
derived predicates. Comparing the plan quality of Macro-FF in {\em
  middle-compiled} with that of SGPlan in {\em middle}, we obtain the
remarkably high ratio values $[7.17 (12.53) 25.71]$. The maximum case
is in instance number 48 -- the largest instance solved by Macro-FF --
where Macro-FF takes 180 steps to solve the compiled instance, while
SGPlan takes only 7 steps to solve the original
instance.\footnote{While Macro-FF is not an optimal planner, and the
  optimal plan lengths for the {\em middle-compiled} instances are not
  known, it seems highly unlikely that these observations are only due
  to overlong plans found by Macro-FF.}




In domain version {\em small}, we awarded 1st places to FDD (and FD),
and SATPLAN; we awarded 2nd places to LPG-TD, SGPlan, YAHSP, and
BFHSP. In domain version {\em middle}, we awarded a 1st place to FDD
(and FD); we awarded 2nd places to LPG-TD and SGPlan. In domain
version {\em middle-compiled}, we awarded a 1st place to Macro-FF. In
domain version {\em large}, we awarded a 1st place to FDD (and FD).



==> hoffmann05a/Pipesworld.tex <==




\subsection{Pipesworld}
\label{results:pipesworld}








The Pipesworld domain is a PDDL adaptation of an application domain
dealing with complex problems that arise when transporting oil
derivative products through a pipeline system. Note that, while there
are many planning benchmarks dealing with variants of transportation
problems, transporting oil derivatives through a pipeline system has a
very different and characteristic kind of structure. The pipelines
must be filled with liquid at all times, and if you push something
into the pipe at one end, something possibly completely different
comes out of it at the other end. As a result, the domain exhibits
some interesting planning space characteristics and good plans
sometimes require very tricky maneuvers. Additional difficulties that
have to be dealt with are, for example, interface restrictions
(different types of products interfere with each other in a pipe),
tankage restrictions in areas (i.e., limited storage capacity defined
for each product in the places that the pipe segments connect), and
deadlines on the arrival time of products.


In the form of the domain used in IPC-4, the product amounts dealt
with are discrete in the sense that we assume a smallest product unit,
called ``batch''. There were six different domain versions in IPC-4:
notankage-nontemporal, notankage-temporal, tankage-nontemporal,
tankage-temporal, notankage-temporal-deadlines, and
notankage-temporal-deadlines-compiled. All versions include interface
restrictions. The versions with ``tankage'' in their name include
tankage restrictions, modelled by a number of ``tank slots'' in each
place in the network, where each slot can hold one batch (note that
the slots introduce some additional symmetry into the problem; we get
back to this below). In the versions with ``temporal'' in their name,
actions take (different amounts of) time.  The versions with
``deadlines'' in their name include deadlines on the arrival of the
goal batches, modelled by timed initial literals respectively their
compilation to standard PDDL2.1. None of the encodings uses any ADL
constructs, so of each domain version there is just one (STRIPS)
formulation. 


The IPC-4 example instances were generated based on five scaling
network topologies. The smallest network topology has 3 areas
connected by 2 pipes; the largest network topology has 5 places
connected by 5 pipes. For each network we generated 10 instances, with
growing numbers of batches, and of batches with a goal location. So
altogether we had 50 instances per domain version, numbered
consecutively. Between domain versions, the instances were, as much as
possible, transferred by adding/removing constructs. E.g., the
instances in tankage-nontemporal (tankage-temporal) are exactly the
same as those in notankage-nontemporal (notankage-temporal) except
that tankage restrictions were added.




We do not include graphs for the domain versions featuring deadlines.
In the version with explicit deadlines (modelled by timed initial
literals), only LPG-TD and Tilsapa participated, of which LPG-TD
scaled up to middle-size instances; Tilsapa solved only a few of the
smallest instances. In the domain version with compiled deadlines,
only CPT participated, solving a few small instances.



\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT/Time-suboptimal-1.eps} &
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT/Time-suboptimal-2.eps}\\
(a) & (b)
\end{tabular}
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT/Time-optimal.eps}\\
(c)
\vspace{0.0cm}
\caption{Non-temporal Pipesworld, no tankage constraints, satisficing (a) and (b), 
  optimal (c).}
\label{pipesworld:nontankagenontemp}
\vspace{0.0cm}
\end{center}
\end{figure}



Figure~\ref{pipesworld:nontankagenontemp} shows the results for the
non-temporal domain version without tankage restrictions. Parts (a)
and (b) contain the results for satisficing planners in the respective
non-temporal domain version. We observe that YAHSP and SGPlan are the
only planners that can solve all instances. YAHSP is a lot faster in
most instances; but it finds excessively long plans: the ratio YAHSP
vs SGPlan is $[0.38 (1.77) 14.04]$, where in the maximum case SGPlan needs
72 actions, YAHSP 1,011. For the other planners, plan quality does not
vary much, with the exception of Marvin, whose makespan ratio vs the
optimal CPT is $[0.88 (1.60) 2.19]$.  LPG-TD and FDD both solve all but a
few of the largest instances. Note that, as in Airport, the IPC-3
version of LPG is outperformed dramatically by the best IPC-4
planners.



Part (c) of Figure~\ref{pipesworld:nontankagenontemp} shows the
results for the optimal planners.  The runtime curves are extremely
similar, nearing indistinguishable.  Note that Optiplan is the only
optimal planner that solves an instance with a very large size
parameter. However, in Pipesworld, like in Airport, due to the domain
combinatorics, planners are likely to find it easier to solve a large
network with little traffic, than a small network with a lot of
traffic.\footnote{On the other hand, note at this point that the
  networks in Pipesworld do by far not grow as much as in Airport,
  where they grow from microscopic toy airports for the smallest
  instances to a real-world airport for the largest instances. As
  said, the smallest network in Pipesworld has 3 areas connected by 2
  pipes, and the largest network has 5 places connected by 5 pipes.}
The other optimal planners here may just not have tried to run their
planner on larger instances when it already failed on the smaller ones
-- we explicitly advised people to save machine workload by not
insisting on spending half an hour runtime on instances that were
probably infeasible for their planners anyway. In cases like this one
here, this admittedly is a potentially misleading guideline.





\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT/Time-suboptimal.eps} &
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT/Time-optimal.eps}\\
(a) & (b)
\end{tabular}
\vspace{0.0cm}
\caption{Temporal Pipesworld without tankage constraints, satisficing (a), optimal (b).}
\label{pipesworld:nontankagetemp}
\vspace{0.0cm}
\end{center}
\end{figure}


In parts (a) and (b) of Figure~\ref{pipesworld:nontankagetemp}, we
display the results in the temporal domain version without tankage
restrictions. Part (a) shows a clear win of SGPlan over the other
planners. We find it particularly remarkable that, as before in
Airport, SGPlan is just as good in the temporal domain version as in
the nontemporal one.  Again, LPG-3 is outperformed by far. As for the
optimal planners in part (b) of the figure, CPT scales best; TP4 and
HSP$_a^*$ scale similarly. The only planners minimizing the number of
actions here are CRIKEY and SGPlan; the ratio is $[0.35 (1.24) 5.67]$,
showing quite some variance with a slight mean advantage for SGPlan.
Of the planners minimizing makespan, LPG-TD and P-MEP sometimes return
long plans; in one instance (number 2), LPG-TD's plan is extremely
long (makespan 432). More precisely, the ratio LPG-TD.speed vs the
optimal CPT is $[1.00 (4.55) 36.00]$; the ratio P-MEP vs CPT is $[1.19
(2.25) 4.59]$; the ratio LPG-TD.quality vs CPT is $[0.73 (1.05) 1.62]$
(i.e., in particular the peak at instance 2 disappears for
LPG-TD.quality). Note that, strangely at first sight, sometimes LPG-TD
finds better plans here than the optimal CPT. This is due to the
somewhat simpler model of durative actions that CPT uses
\cite{vidal:geffner:aaai-04}, making no distinction between the start
and end time points of actions.


\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT/Time-suboptimal-1.eps} &
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT/Time-suboptimal-2.eps}\\
(a) & (b)
\end{tabular}
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT/Time-optimal.eps}\\
(c)\\
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT/Time-suboptimal.eps} &
\includegraphics[width=7.3cm]{RESULTS/PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT/Time-optimal.eps}\\
(d) & (e)
\end{tabular}
\vspace{0.0cm}
\caption{Pipesworld with tankage constraints: non-temporal satisficing (a) and (b), 
  optimal (c), temporal satisficing (d), optimal (e).}
\label{pipesworld:tankage}
\vspace{0.0cm}
\end{center}
\end{figure}



In Figure~\ref{pipesworld:tankage}, results are displayed for the two
domain versions that do feature tankage restrictions. Very generally,
we see that the planners have much more trouble with these domain
versions than with their less constrained counterparts.


In the non-temporal domain version with tankage constraints, for the
satisficing planners in parts (a) and (b) we observe that, as before,
YAHSP is most efficient, solving more instances than any of the other
planners.  Again, this efficiency is bought at the cost of overlong
plans: the ratio YAHSP vs. SGPlan is $[0.66 (1.89) 6.14]$, where in
the maximum case SGPlan needs 64 actions, YAHSP 393. For the other
planners, plan quality does not vary as much (e.g. the ratio FDD vs
SGPlan is $[0.56 (0.96) 1.38]$. Of the optimal planners displayed in
part (c), same non-temporal domain version, SATPLAN and Optiplan scale
a little better than the other planners, solving two and three more
instances, respectively.  SATPLAN tends to be faster than Optiplan in
the solved cases. Part (d) displays the results for the satisficing
planners in the respective temporal domain version. SGPlan clearly
scales best, once again keeping its performance from the corresponding
non-temporal domain version. LPG-TD is followed relatively closely by
CRIKEY but can solve some more instances. Regarding plan quality,
CRIKEY and SGPlan minimize plan length, and the ratio CRIKEY vs SGPlan
is $[0.62 (1.37) 2.54]$. For makespan, LPG-TD again has a peak in
instance 2; the ratio LPG-TD.speed vs CPT is $[1.00 (2.55) 7.27]$,
maximum 160 vs 22 units; the ratio LPG-TD.quality vs CPT is $[0.86
(0.95) 1.18]$ (LPG-TD.quality's makespan in instance 2 is $26$). Note
that, as above, LPG-TD.quality can find better plans than CPT due to
the somewhat simpler model of durative actions used in CPT. In the
optimal track, TP4 performs a little better, in terms of runtime, than
the similar-performing CPT and HSP$_a^*$; all the planners solve only
a few of the smallest instances.




We remark that we were rather surprised by the relatively good scaling
behavior of some planners, particularly of the fastest satisficing
planners in the domain versions without tankage restrictions.
\citeA{hoffmann:jair-05} shows that, in Pipesworld, there can be
arbitrarily deep local minima under relaxed plan distances (i.e., the
distance from a local minimum to a better region of the state space
may be arbitrarily large). No particularly unusual constructs are
needed to provoke local minima -- for example, a cycle of pipe
segments, as also occurs in the network topologies underlying the
IPC-4 instances, suffices. Not less importantly, in the limited
experiments we did during testing, FF \cite{hoffmann:nebel:jair-01}
and Mips \cite{edelkamp:jair-03} generally scaled much worse than,
e.g., YAHSP and SGPlan do as shown above.
% So the lookahead and
% problem decomposition techniques employed by these planners,
% respectively, seem to be quite effective in this domain.


As for the domain versions that do feature tankage restrictions, these
are harder than their counterparts. There are two important
differences between the domain versions with/without tankage
restrictions. First, the problem is more constrained (remember that,
modulo the tankage constraints, the IPC-4 instances are identical in
both respective versions). Second, the tank slots, that model the
restrictions, introduce additional symmetry into the problem: a
planner can now choose into which (free) slot to insert a batch. This
choice does not make a difference, but enlarges the state space
exponentially in the number of such choices (to the basis of the
number of tank slots). We considered the option to use a ``counter''
encoding instead, to avoid the symmetry: one could count the product
amounts in the areas, and impose the tankage restrictions based on the
counter values. We decided against this because symmetry is a
challenging aspect of a benchmark.







In domain version notankage-nontemporal, we awarded 1st places to
YAHSP and SGPlan; we awarded 2nd places to LPG-TD and FDD. In version
notankage-temporal, we awarded 1st places to SGPlan and CPT; we
awarded 2nd places to LPG-TD, TP4, and HSP$_a^*$. In version
tankage-nontemporal, we awarded 1st places to YAHSP and FDD; we
awarded 2nd places to SGPlan, SATPLAN, and Optiplan. In version
tankage-temporal, we awarded a 1st place to SGPlan; we awarded 2nd
places to LPG-TD and TP4. In version notankage-temporal-deadlines, we
awarded a 1st place to LPG-TD.







==> hoffmann05a/Promela.tex <==







\subsection{Promela}
\label{results:promela}





Promela is the input language of the model checker
SPIN~\cite{Holzmann04}, used for specifying communication protocols.
Communication protocols are distributed software systems, and many
implementation bugs can arise, like deadlocks, failed assertions, and
global invariance violations. The model checking
problem~\cite{ModelChecking} is to find those errors by returning a
counter-example, or to verify correctness by a complete exploration of
the underlying state-space. \citeA{edelkamp:spin-03} developed an
automatic translation of this problem, i.e., of the Promela language,
into (non-temporal) PDDL, making it possible to apply state-of-the-art
planners without any modification.


For IPC-4, two relatively simple communication protocols were selected
as benchmarks -- toy problems from the Model-Checking area. One is the
well-known Dining-Philosophers protocol, the other is a larger
protocol called Optical-Telegraph. The main point of using the domain,
and these protocols, in IPC-4 was to promote the connection between
Planning and Model-Checking, and to test how state-of-the-art planners
scale to the basic problems in the other area. 



The IPC-4 instances exclusively require to find deadlocks in the
specified protocols -- states in which no more transitions are
possible. The rules that detect whether or not a given state is a
deadlock are most naturally modelled by derived predicates, with
complex ADL formulas in the rule bodies. To enable broad
participation, we provided compilations of derived predicates into
additional actions, and of ADL into STRIPS. Edelkamp's original
translation of Promela into PDDL also makes use of numeric variables.
For the non-numeric planners, the translation was adapted to use
propositional variables only -- for the relatively simple
Dining-Philosophers and Optical-Telegraph protocols, this was
possible.



Precisely, the domain versions and formulations were the following.
First, the versions were split over the modelled protocol,
Dining-Philosophers or Optical-Telegraph. Second, the versions were
split over the used language: with/without numeric variables, and
with/without derived predicates.\footnote{We split with/without
  numeric variables into different domain versions, rather than
  formulations, to encourage the use of numeric planning techniques.
  We split with/without derived predicates into different versions
  since, through the modelling of derived predicates as new actions,
  the plans become longer.} So, all in all, we had 8 domain versions.
Each of them used ADL constructs. In those 4 versions without numeric
variables, we also provided STRIPS formulations, obtained from the ADL
formulations with automatic compilation software based on FF's
pre-processor \cite{hoffmann:nebel:jair-01}, producing fully grounded
encodings. All Promela domain versions are non-temporal.



















Here, we show plots only for the results obtained in the non-numeric
domain versions. In the domain versions using both numeric variables
and derived predicates, {\em no} planner participated. In the numeric
version of Dining-Philosophers (without derived predicates), only
SGPlan and P-MEP participated. SGPlan solved all instances while P-MEP
solved only a few of the smallest ones. In the numeric version of
Optical-Telegraph (without derived predicates), only SGPlan
participated, solving some relatively small instances.







\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/PROMELA/PHILOSOPHERS/GNUPLOT/Time-suboptimal-all.eps} & 
\includegraphics[width=7.3cm]{RESULTS/PROMELA/PHILOSOPHERS/GNUPLOT/Time-optimal.eps}\\
(a) & (b)
\end{tabular}
\includegraphics[width=7.3cm]{RESULTS/PROMELA/PHILOSOPHERS_DERIVEDPREDICATES/GNUPLOT/Time-suboptimal-all.eps}\\
(c)
\caption{Performance in Promela/Dining Philosophers. Encoding without derived predicates, satisficing (a), 
  optimal (b). Encoding with derived predicates, satisficing (c).}
\label{fig:phil}
\vspace{0.0cm}
\end{center}
\end{figure}





Parts (a) and (b) of Figure~\ref{fig:phil} show the results for
Dining-Philosophers, without derived predicates, i.e. with additional
actions to derive the deadlocks. In the the satisficing track, YAHSP
and SGPlan clearly show the best performance. The other planners all
lag several orders of magnitude behind. In the optimal track, SATPLAN
clearly scales best, followed by Optiplan. Observe that, in difference
to what we have seen in Airport and Pipesworld, {\em the optimal
  planners are just as efficient as the satisficing ones.} This is
evident from the plots. Most particularly, SATPLAN and Optiplan solve
just as many instances, up to $30$ philosophers (instance number $x$
features $x+1$ philosophers), like YAHSP and
SGPlan.\footnote{Importantly, these planners handle only STRIPS, and
  for compilation reasons there were STRIPS instances up to $n=30$
  only. So these planners solve {\em all} their respective test
  instances. We discuss this in a little more detail further below.}
SATPLAN even does so in comparable time. Such a competitivity of
optimal planners with satisficing ones has not been seen in any test
suite used in any of the last three competitions.\footnote{In the first
  IPC, in 1998, apart from the fact that the ``heuristic search''
  satisficing planners were still in their infancy, Mystery and Mprime
  were used as benchmarks. These can't be solved particularly
  efficiently by any planner up to today, except, maybe, FD and FDD
  \cite{helmert:icaps-04}.} The efficiency of SATPLAN and Optiplan in
Dining-Philosophers is probably due the fact that the needed number of
parallel time steps is {\em constantly} $11$ across all instances (see
below).  In a (standard) planning graph
\cite{blum:furst:ijcai-95,blum:furst:ai-97}, the goals are first
reached after $7$ steps; so only 4 unsuccessful iterations are made
before a plan is found.



Regarding plan quality, there is one group of planners trying to
minimize the number of actions, and one group trying to minimize the
makespan (the number of parallel action steps). The results clearly
point to an important difference between this domain and the other
IPC-4 domains. Namely, there is only a single scaling parameter $n$ --
the number of philosophers -- and only a single instance per value of
$n$.  The optimal number of actions is a linear function of $n$,
precisely $11n$: basically, one blocks all philosophers in sequence,
taking $11$ steps for each. The optimal makespan is, as mentioned
above, constantly $11$: one can block all philosophers in parallel.
The only sub-optimal plan found by any planner minimizing the number
of actions is that of CRIKEY for $n=8$, containing 104 instead of 88
actions. Of the planners minimizing makespan, only P-MEP finds
sub-optimal plans: it solves only the smallest four instances,
$n=2,3,4,5$, with a makespan of 19, 25, 30, and 36, respectively.





Figure~\ref{fig:phil} (c) shows the results in the domain version that
uses derived predicates to detect the deadlock situations. No optimal
planner could handle derived predicates which is why there are no
results for this. Of the satisficing planners, SGPlan clearly shows
the best performance. FDD and LPG-TD are roughly similar -- note that,
while LPG-TD is faster than FDD in most examples, the behavior of FDD
in the largest instances indicates an advantage in scaling. There is a
sudden large increase in LPG-TD's runtime, from the second largest
instance (that is solved in 52 seconds) to the largest instance (that
is solved in 1045 seconds). In difference to that, FDD solves the
largest instance in almost the same time as the second largest one,
taking 111 seconds instead of 110 seconds (in fact, FDD's runtime
performance shows little variance and is pretty much a linear function
in the instance size). We remark that the plans for the largest of
these instances are huge: more than 400 steps long, see below. SGPlan
generates these plans in little more than a single second CPU time.


Regarding plan quality, in this domain version the optimal number of
actions is $9n$, and the optimal makespan is constantly $9$. All
planners except Marvin tried to minimize the number of actions. FD and
SGPlan always find optimal plans. FDD, LPG-TD.speed, and
LPG-TD.quality sometimes find slightly sub-optimal plans. Precisely,
the ratio FDD vs FD is $[1.00 (1.08) 1.44]$; LPG-TD.speed vs FD is $[1.00
(1.10) 2.19]$; LPG-TD.quality vs FD is $[1.00 (1.03) 1.24]$. As for Marvin,
the makespan of its plans is, roughly, linear in $n$; it always lies
between $7n$ and $9n$.



At this point, there is an important remark to be made about a detail
regarding our compilation techniques in these domain versions. Observe
the huge gap in planner performance between Figure~\ref{fig:phil} (a)
and (b), and Figure~\ref{fig:phil} (c). As we have seen, the
difference in plan length (makespan) is not very large -- $11n$ ($11$)
compared to $9n$ ($9$). Indeed, the apparent performance difference is
due to a {\em compilation} detail, inherent in the IPC-4 instances,
rather than to planner performance. In the version without derived
predicates, we were able to compile only the instances with up to
$n=30$ philosophers from ADL into STRIPS. For larger values of $n$,
the (fully-grounded) STRIPS representations became prohibitively
large. In the version {\em with} derived predicates, the blow-up was a
lot smaller, and we could compile {\em all} instances, with up to
$n=49$ philosophers. SGPlan, YAHSP, SATPLAN, and Optiplan can all
handle only STRIPS. So, as mentioned above, in Figure~\ref{fig:phil}
(a) and (b) these planners actually solve all instances in their
respective test suite; they would probably scale up further when
provided with STRIPS representations of instances with larger $n$
values.







\begin{figure}[htb]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/PROMELA/OPTICAL_TELEGRAPH/GNUPLOT/Time-suboptimal-all.eps} & 
\includegraphics[width=7.3cm]{RESULTS/PROMELA/OPTICAL_TELEGRAPH/GNUPLOT/Time-optimal.eps}\\
(a) & (b)
\end{tabular}
\includegraphics[width=7.3cm]{RESULTS/PROMELA/OPTICAL_TELEGRAPH_DERIVEDPREDIC/GNUPLOT/Time-suboptimal-all.eps}\\
(c)
\caption{Performance in Promela/Optical Telegraph. Encoding without derived predicates, satisficing (a), 
  optimal (b). Encoding with derived predicates, satisficing (c).}
\label{fig:opt}
\vspace{0.0cm}
\end{center}
\end{figure}





The Optical-Telegraph protocol is slightly more complex than the
Dining-Philosopher example, i.e. it involves more complicated and
indirect interactions between the communicating processes, leading to
longer solutions. There is still just one scaling parameter, the
number $n$ of ``telegraph station pairs'', and a single instance per
value of $n$. Each telegraph station pair is a pair of processes that
goes through a rather complicated internal communication structure,
enabling the exchange of data. The telegraph station pair shares with
the outside world -- i.e., with the other telegraph station pairs --
two ``control channels'' that must be occupied as a prerequisite to
the internal exchange of data. Thus, the role of the control channels
is pretty similar to the role of the (shared) forks in the
Dining-Philosopher example. Instance number $x$ in IPC-4 features
$x+1$ telegraph station pairs.



Figure~\ref{fig:opt} shows in parts (a) and (b) the performance of the
satisficing and optimal planners, respectively, in the domain version
using additional actions to derive deadlocks. In the group of
satisficing planners, Macro-FF clearly performs best. Of the other
satisficing planners, SGPlan is the most efficient. It is important to
note that, here, we were able to compile only the instances up to
$n=15$ from ADL into STRIPS. So SGPlan and LPG-TD solve all their
respective test instances. Of the optimal planners, SATPLAN and
Optiplan solve the instances up to $n=14$, i.e., they failed to solve
the largest instance in the STRIPS test suite they attacked. SATPLAN
is much faster than Optiplan. Each of the other optimal planners could
solve only the smallest instance, $n=2$. Figure~\ref{fig:opt} (c)
shows that FDD, which handles the ADL formulation, is by far the most
successful satisficing planner in the domain version encoding
Optical-Telegraph with derived predicates for deadlock detection; of
the other planners, SGPlan scales best, solving all instances in the
STRIPS set, up to $n=20$.




Regarding plan quality, in Optical-Telegraph without derived
predicates the optimal number of actions is $18n$, and the optimal
makespan is constantly $13$: optimal sequential plans block all
telegraph station pairs in sequence, taking $18$ steps for each; in
parallel plans, some simultaneous actions are possible {\em within}
each telegraph station pair. In Optical-Telegraph {\em with} derived
predicates, the optimal number of actions is $14n$, and the optimal
makespan is constantly $11$. In the competition results, all planners
returned the optimal plans in these test suites, in all cases -- with
a single exception. The plans found by Marvin in the version with
derived predicates have makespan $14n$ in all solved cases.








As we have seen, the results in Promela are, over all, quite different
from, e.g., those we have seen in Airport and Pipesworld. There is
only a single scaling parameter and a single instance per size, and
optimal makespan is constant. This leads to rather smooth runtime and
plan quality curves, as well as to an unusual competitivity of optimal
planners with satisficing planners. The scalability of the planners
both shows that current planners {\em are} able to efficiently solve
the most basic Model-Checking benchmarks (Dining-Philosophers), and
that they are not very efficient in solving more complex
Model-Checking benchmarks (Optical-Telegraph). We remark that
\citeA{hoffmann:jair-05} shows that there exist arbitrarily deep local
minima under relaxed plan distances in Optical-Telegraph, but not in
Dining-Philosophers, where there exists a large upper bound (31) on
the number of actions needed to escape a local minimum. It is not
clear, however, how much these theoretical results have to do with the
planner performance observed above. The worst-cases observed by
Hoffmann all occur in regions of the state space {\em not} entered by
plans with optimal number of actions -- as found by the IPC-4
participants, in most cases.






In Dining-Philosophers without derived predicates, we awarded 1st
places to YAHSP, SGPlan, and SATPLAN; we awarded a 2nd place to
Optiplan. In Dining-Philosophers with derived predicates, we awarded a
1st place to SGPlan, and 2nd places to FDD and LPG-TD. In
Optical-Telegraph without derived predicates, we awarded 1st places to
Macro-FF and SATPLAN; we awarded 2nd places to SGPlan and Optiplan.
In Optical-Telegraph with derived predicates, we awarded a 1st place
to FDD, and a 2nd place to SGPlan. In the numeric version of
Dining-Philosophers, we awarded a 1st place to SGPlan.



==> hoffmann05a/RESULTS/gnus <==
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL_DEADLINES/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL_DEADLINES/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL_DEADLINES_CO/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL_DEADLINES_CO/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_DERIVEDPREDIC/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_DERIVEDPREDIC/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_DERIVEDPREDIC/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_FLUENTS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_FLUENTS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_DERIVEDPREDICATES/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_DERIVEDPREDICATES/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_DERIVEDPREDICATES/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_FLUENTS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_FLUENTS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_FLUENTS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/LARGE/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/LARGE/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/LARGE/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE_COMPILED/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_OPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_OPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS/GNUPLOT ; gnuplot <  METRICVALUE.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/NUMERIC/GNUPLOT ; gnuplot <  METRICVALUE.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/NUMERIC/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/NUMERIC/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/STRIPS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/STRIPS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/STRIPS/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/STRIPS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SETTLERS/IPC_3/GNUPLOT ; gnuplot <  METRICVALUE.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SETTLERS/IPC_3/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SETTLERS/IPC_3/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS_COMPI/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS_COMPI/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS


==> hoffmann05a/Satellite.tex <==




\subsection{Satellite}
\label{results:satellite}









The {\em Satellite} domain was introduced in IPC-3 by
\citeA{long:fox:jair-03}. It is motivated by a NASA space application:
a number of satellites has to take images of a number of spatial
phenomena, obeying constraints such as data storage space and fuel
usage. In IPC-3, there were the domain versions {\em Strips}, {\em
  Numeric}, {\em Time} (action durations are expressions in static
variables), and {\em Complex} (durations {\em and} numerics, i.e. the
``union'' of Numeric and Time). The numeric variables transport the
more complex problem constraints, regarding data capacity and fuel
usage. 


For IPC-4, the domain was made a little more realistic by additionally
introducing time windows for the sending of the image data to earth,
i.e. to antennas that are visible for satellites only during certain
periods of time. We added the new domain versions {\em
  Time-timewindows}, {\em Time-timewindows-compiled}, {\em
  Complex-timewindows}, and {\em Complex-timewindows-compiled}, by
introducing time windows, explicit and compiled, into the IPC-3 {\em
  Time} and {\em Complex} versions, respectively.\footnote{In the new
  domain versions derived from Complex, we also introduced utilities
  for the time window inside which an image is sent to earth. For each
  image, the utility is either the same for all windows, or it
  decreases monotonically with the start time of the window, or it is
  random within a certain interval. Each image was put randomly into
  one of these classes, and the optimization requirement is to
  minimize a linear combination of makespan, fuel usage, and summed up
  negated image utility.} None of the domain versions uses ADL
constructs, so of all versions there was only a single (STRIPS)
formulation. The instances were, as much as possible, taken from the
original IPC-3 instance suites. Precisely, the Strips, Numeric, Time,
and Complex versions each contained the 20 instances posed in IPC-3 to
the fully-automatic planners, plus the 16 instances posed in IPC-3 to
the hand-tailored planners. For Time-timewindows and
Time-timewindows-compiled, we extended the 36 instances from Time with
the time windows. Similarly, for Complex-timewindows and
Complex-timewindows-compiled, we extended the 36 instances from
Complex with the time windows.  That is, in the newly added domain
versions the sole difference to the previous instances lies in the
time windows.






\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]
{RESULTS/SATELLITE/STRIPS/GNUPLOT/Time-suboptimal-all.eps} & 
\includegraphics[width=7.3cm]
{RESULTS/SATELLITE/STRIPS/GNUPLOT/Time-optimal.eps} \\
(a) & (b) \\
\includegraphics[width=7.3cm]
{RESULTS/SATELLITE/TIME/GNUPLOT/Time-suboptimal.eps} &
\includegraphics[width=7.3cm]
{RESULTS/SATELLITE/TIME/GNUPLOT/Time-optimal.eps} \\
(c) & (d) 
\end{tabular}
\caption{Satellite; Strips satisficing (a), optimal (b), and Time satisficing (c), optimal (d).}
\label{sat:nontandt}
\end{center}
\vspace{-0.0cm}
\end{figure}



Let us first consider the results in the simpler versions of the
Satellite domain. Figure~\ref{sat:nontandt} shows the results for the
Strips and Time versions. To many of the satisficing planners, the
Strips version does not pose a serious problem, see
Figure~\ref{sat:nontandt} (a). Macro-FF and YAHSP show the best
runtime behavior, followed closely by LPG-TD and FDD (as well as FD).
As for the optimal planners in Figure~\ref{sat:nontandt} (b), none of
them scales up very far. SATPLAN is most efficient, solving 11
instances; CPT and Semsyn each solve 9 instances, Optiplan solves 8,
BFHSP solves only 6. In the Time version, LPG-TD and SGPlan behave
similarly up to instance number 30, but LPG-TD solves two more,
larger, instances. The Time optimal planners, see
Figure~\ref{sat:nontandt} (d), are clearly headed by CPT.



Regarding the efficiency of the satisficing planners in the Strips
test suite, we remark that these instances were solved quite
efficiently at IPC-3 already, e.g. by FF and LPG-3. Further,
\citeA{hoffmann:jair-05} shows that, in this domain, under relaxed
plan distance, from any non-goal state, one can reach a state with
strictly smaller heuristic value within at most 5 steps. In that
sense, the results depicted in Figure~\ref{sat:nontandt} (a) didn't
come as a surprise to us.


\begin{sloppypar}
Let us consider plan quality in Strips and Time. In both domain
versions, as before the addressed optimization criteria are plan
length, and makespan. In Strips, the plan quality behavior of all the
planners trying to minimize plan length is rather similar. The overall
shortest plans are found by LPG-TD.quality. Precisely, the ratio FDD
vs LPG-TD.quality is $[0.96 (1.19) 1.48]$; the ratio FD vs
LPG-TD.quality is $[0.96 (1.20) 1.53]$; the ratio LPG-TD.speed vs
LPG-TD.quality is $[1.00 (1.12) 1.31]$; the ratio Macro-FF vs
LPG-TD.quality is $[0.95 (1.03) 1.17]$; the ratio Roadmapper vs
LPG-TD.quality is $[1.00 (1.35) 1.71]$; the ratio SGPlan vs
LPG-TD.quality is $[0.99 (1.07) 1.70]$; the ratio YAHSP vs
LPG-TD.quality is $[0.97 (1.22) 1.93]$. Of the planners trying to
optimize makespan in the Strips version, only Marvin and P-MEP are
satisficing; Marvin is the only planner that scales to the larger
instances. The ratio P-MEP vs SATPLAN (which solves a superset of the
instances solved by P-MEP) is $[1.01 (2.22) 3.03]$. The ratio Marvin
vs SATPLAN is $[1.08 (2.38) 4.00]$.
\end{sloppypar}


In the Time version, the only planner minimizing plan length (i.e.,
the number of actions) is SGPlan, so there is no basis for comparison.
The only satisficing planners trying to minimize makespan are P-MEP
and LPG-TD. In the small instances solved by CPT (actually, a superset
of those solved by P-MEP), the ratio P-MEP vs CPT is $[1.10 (3.71)
6.49]$.  The ratio LPG-TD.speed vs CPT is $[1.33 (3.37) 5.90]$; the
ratio LPG-TD.quality vs CPT is $[0.85 (1.24) 1.86]$. Note that, like
we have seen in Pipesworld before, sometimes LPG-TD finds better plans
here than the optimal CPT. As said, this is due to the somewhat
simpler model of durative actions that CPT uses
\cite{vidal:geffner:aaai-04}, making no distinction between the start
and end time points of actions.









\begin{figure}[t]
\vspace{-0.0cm}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=7.3cm] {RESULTS/SATELLITE/NUMERIC/GNUPLOT/Time-all.eps} &
\includegraphics[width=7.3cm]{RESULTS/SATELLITE/TIME_TIMEWINDOWS/GNUPLOT/Time-suboptimal.eps} \\
(a) & (b) \\
\includegraphics[width=7.3cm]{RESULTS/SATELLITE/COMPLEX/GNUPLOT/Time-suboptimal.eps} &
\includegraphics[width=7.3cm]{RESULTS/SATELLITE/COMPLEX_TIMEWINDOWS/GNUPLOT/Time-all.eps} \\
(c) & (d)
\end{tabular}
\caption{Satellite; Numeric (a), Time-timewindows (b), satisficing Complex (c), Complex-timewindows (d).}
\label{sat:ntwc}
\end{center}
\vspace{-0.0cm}
\end{figure}




Figure~\ref{sat:ntwc} (a) shows the results in Satellite Numeric,
together for all participating planners -- the only optimal planner
that participated here was Semsyn. SGPlan and LPG-TD scale best; they
solve the same number of instances, but SGPlan solves some larger ones
and is at least an order of magnitude faster in those instances solved
by both. Regarding plan quality, SGPlan was the only planner here
trying to minimize plan length. The other planners tried to minimize
the metric value of the plan, i.e., the quality metric specified in
the instance files, which is fuel usage. The best plans in this
respect are found by LPG-TD.quality; it is unclear to us why Semsyn
was marked to optimize the metric value here, and why it does not find
the optimal plans. The ratio LPG-TD.speed vs LPG-TD.quality is $[1.00
(2.26) 4.69]$; the ratio P-MEP vs LPG-TD.quality is $[1.01 (2.16)
3.03]$; the ratio Semsyn vs LPG-TD.quality is $[1.00 (1.28) 1.58]$.



In Time-timewindows, no optimal planner could participate due to the
timed initial literals. Of the satisficing planners, see
Figure~\ref{sat:ntwc} (b), only SGPlan and LPG-TD participated, which
both scaled relatively well, with a clear advantage for SGPlan.
Regarding plan length, SGPlan minimizes the number of actions, and
LPG-TD the makespan. The ratio LPG-TD.speed vs LPG-TD.quality is
$[1.00 (1.22) 1.51]$. In Time-timewindows-compiled, only SGPlan and
CPT participated. SGPlan largely maintained its performance from the
Time-timewindows version, CPT could solve only 3 of the smallest
instances. Plan quality can't be compared due to the different
criteria (plan length and makespan) that are minimized.





Figure~\ref{sat:ntwc} (c) shows the performance of the satisficing
planners in Satellite Complex. SGPlan and LPG-TD scale well, in
particular much better than the only other competitor, P-MEP. In the
largest three instances, SGPlan shows a clear runtime advantage over
LPG-TD. In the optimal track, only TP4 and HSP$_a^*$ competed here.
Both solved the same four very small instances, numbers 1, 2, 3, and
5, in almost the same runtime. SGPlan is the only planner minimizing
the number of actions. Of the other planners, which all try to
minimize makespan, only LPG-TD scales up to large instances. The ratio
LPG-TD.speed vs LPG-TD.quality is $[1.01 (2.76) 4.71]$. The ratio
LPG-TD.speed vs TP4 is $[1.81 (2.09) 2.49]$; the ratio LPG-TD.quality
vs TP4 is $[0.93 (1.07) 1.19]$; the ratio P-MEP vs TP4 is $[1.27
(2.25) 3.32]$.  As above for CPT, the better plan (in one case) found
by LPG-TD.quality is due to the somewhat simpler action model used in
TP4 \cite{haslum:geffner:ecp-01}.




Figure~\ref{sat:ntwc} (d) shows the performance of all planners in
Complex-timewindows -- as above, due to the timed initial literals no
optimal planner could compete here. SGPlan scales clearly best,
followed by LPG-TD; Tilsapa solves only the 3 smallest instances. Of
these 3 participating planners, each one minimizes a different quality
criterion: number of actions for SGPlan, makespan for Tilsapa, and
metric value -- the aforementioned linear combination of makespan,
fuel usage, and summed up negated image utility -- for LPG-TD. So the
only useful comparison is that between LPG-TD.speed and
LPG-TD.quality, where the ratio is $[1.00 (2.33) 7.05]$.\footnote{Due
  to the negated image utility, the quality values here can be
  negative.  For LPG-TD.speed and LPG-TD.quality here, this happened
  in 5 instances. We skipped these when computing the given ratio
  values, since putting positive and negative values together doesn't
  make much sense -- with negative quality, the number with larger
  absolute value represents the better plan. It would probably have
  been better to define, in this domain version, an image penalty
  instead of an image utility, and thus obtain strictly positive
  action ``costs''.}  In Complex-timewindows-compiled, the only
participating planner was SGPlan. It maintained its good scalability
from the Complex domain version with explicit time windows.





In domain version Strips, we awarded 1st places to Macro-FF, YAHSP,
and SATPLAN; we awarded 2nd places to FDD (and FD), LPG-TD, CPT,
Optiplan, and Semsyn. In domain version Time, we awarded 1st places to
LPG-TD and CPT; we awarded a 2nd place to SGPlan. In each of the
domain versions Numeric, Time-timewindows, Complex, and
Complex-timewindows, we awarded a 1st place to SGPlan and a 2nd place
to LPG-TD.



==> hoffmann05a/Settlers.tex <==









\subsection{Settlers}
\label{results:settlers}











The {\em Settlers} domain was also introduced in IPC-3
\cite{long:fox:jair-03}. It features just a single domain version,
which makes extensive use of numeric variables. These variables carry
most of the domain semantics, which is about building up an
infrastructure in an unsettled area, involving the building of houses,
railway tracks, sawmills, etc.  In IPC-3, no planner was able to deal
with the domain in an efficient way -- the best IPC-3 planner in
Settlers, Metric-FF \cite{hoffmann:jair-03}, solved only the smallest
six instances of the test suite. For these reasons, we included the
domain into IPC-4 as a challenge for the numeric planners. We used the
exact same domain file and example instances as in IPC-3, except that
we compiled away some universally quantified preconditions to improve
accessibility for planners. The quantifiers were not nested, and
ranged over a fixed set of domain constants, so they could easily be
replaced by conjunctions of atoms.





\begin{figure}[t]
\begin{center}
\includegraphics[width=7.3cm]{RESULTS/SETTLERS/IPC_3/GNUPLOT/Time-all.eps}
\end{center}
\caption{Performance of all planners in Settlers.}
\label{settlers:all}
\end{figure}





Figure~\ref{settlers:all} shows the runtime results obtained in IPC-4.
The efficiency increase compared to IPC-3 is, obviously, dramatic:
SGPlan solves every instance within less than 15 seconds (instance
number 8 is unsolvable).\footnote{We remark that instance $8$ is
  trivially unsolvable. One of the goals can only be achieved by
  actions having a static precondition that is false in the initial
  state.  This can be detected by simple reachability analyses like,
  e.g., planning graphs, even without taking account of delete lists.}
LPG-TD solves 13 instances out of the set, Semsyn solves 3 (numbers
1,2, and 5). We remark that the solutions for these tasks, as returned
by SGPlan, are huge, up to more than 800 actions in the largest tasks.
On the one hand, this once again demonstrates SGPlan's capability to
find extremely long plans extremely quickly. On the other hand,
SGPlan's plans in Settlers might be unnecessarily long, to some
extent. In the largest instance solved by Semsyn, number 5, Semsyn
finds a plan with 94 actions, while the plan found by SGPlan has 264
actions. In the largest instance solved by LPG-TD, number 17,
LPG-TD.quality takes 473 actions while SGPlan takes 552. LPG-TD
minimizes the metric value of the plans, a linear combination of the
invested labor, the resource use, and the caused pollution. The ratio
LPG-TD.speed vs LPG-TD.quality is $[1.00 (1.21) 3.50]$.


We awarded a 1st place to SGPlan and a 2nd place to LPG-TD.



% Figure~\ref{settlers:all} shows the runtime results obtained in IPC-4.
% The efficiency increase compared to IPC-3 is, obviously, dramatic:
% SGPlan solves every instance within less than 15 seconds (instance
% number 8 is unsolvable). We awarded a 1st place to SGPlan and a 2nd
% place to LPG-TD. We remark that the solutions for these tasks, as
% returned by SGPlan, are huge, up to more than 800 actions in the
% largest tasks. On the one hand, this once again demonstrates SGPlan's
% capability to find extremely long plans extremely quickly. On the
% other hand, SGPlan's plans in Settlers are probably overly long. In
% those instances solved by both LPG-TD and SGPlan, SGPlan's plans are
% around 20\% longer.



==> hoffmann05a/UMTS.tex <==






\subsection{UMTS}
\label{results:umts}








UMTS applications require comparatively much time to be started on a
hand-held device, since they have to communicate with the network
several times. If there is more than one application that has been
called, this yields a true bottleneck for the user.  Therefore, the
applications set-up is divided into several parts to allow different
set-up modules to work concurrently.  The task in the domain is to
provide a good schedule -- minimizing the used time -- for setting up
timed applications, respecting the dependencies among them.




In IPC-4, there were the six domain versions {\em UMTS}, {\em
  UMTS-timewindows}, {\em UMTS-timewindows-compiled}, {\em UMTS-flaw},
{\em UMTS-flaw-timewindows}, and {\em UMTS-flaw-timewindows-compiled}.
All of these domain versions are temporal, and make use of numeric
variables to model the properties of the applications to be set up.
ADL constructs are not used. UMTS is our standard model of the domain.
In UMTS-timewindows there are additional time windows regarding the
executability of set up actions, encoded with timed initial literals.
In UMTS-timewindows-compiled the same time windows are compiled into
artificial constructs. The remaining three domain versions result, as
their names suggest, from adding a {\em flaw} construction to their
respective counterparts. The flaw construction is practically
motivated. It consists of an extra action that has an important
sub-goal as its add effect, but that deletes another fact that can't
be re-achieved. So the flaw action can't be used in a plan, but it can
be used in relaxed plans, i.e. when ignoring the delete effects.  In
particular, adding an important sub-goal, the flawed action provides a
kind of ``short-cut'' for relaxed plans, where the short-cut does not
work in reality. This can lead to overly optimistic heuristic values.
Thus the flaw may confuse the heuristic functions of relaxed-plan
based heuristic planners. We used the flawed domain versions in IPC-4
to see whether the latter would be the case.




In the IPC-4 test suites, all instances, irrespective of their
number/size, contain 10 applications. The main scaling parameter is
the number of applications that must actually be set up. For IPC-4
instances number 1 \dots 5, a single application must be set up; for
instances number 6 \dots 10, two applications must be set up, and so
on, i.e., the number of needed applications is $\lfloor x/5 \rfloor$
where $x$ is the index of the instance.





\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/UMTS/TEMPORAL/GNUPLOT/Time-suboptimal.eps} &
\includegraphics[width=7.3cm]{RESULTS/UMTS/TEMPORAL/GNUPLOT/Time-optimal.eps} \\
(a) & (b) \\
\includegraphics[width=7.3cm]{RESULTS/UMTS/FLAW_TEMPORAL/GNUPLOT/Time-suboptimal.eps} &
\includegraphics[width=7.3cm]{RESULTS/UMTS/FLAW_TEMPORAL/GNUPLOT/Time-optimal.eps}\\
(c) & (d)
\end{tabular}
\vspace{-0.0cm}
\end{center}
\caption{UMTS, satisficing (a) optimal (b); UMTS-flaw, satisficing (c) optimal (d).}
\label{umts:notw}
\end{figure}



Figure~\ref{umts:notw} (a) and (b) shows the IPC-4 performance in the
basic domain version. Obviously, SGPlan and LPG-TD have no difficulty
at all with the domain -- they solve every instance within split
seconds. CRIKEY takes more time, but also scales up nicely. As for the
optimal planners, only TP4 and HSP$_a^*$ were able to handle the
domain syntax, due to the combination of numeric variables and action
durations. As Figure~\ref{umts:notw} (b) shows they scaled relatively
similarly, with a slight advantage for HSP$_a^*$. Note that the two
planners {\em scaled better than P-MEP and LPG-3 in the satisficing
  track.}


We remark at this point that UMTS is mainly intended as a benchmark
for {\em optimal} planners minimizing makespan. The domain is a pure
scheduling problem by nature. As in most scheduling problems, it is
trivial to find {\em some} plan -- for example, one can simply
schedule all applications in sequence.\footnote{Note that this is not
  possible in the Airport domain -- that can also be viewed as a type
  of scheduling problem \cite{hatzack:nebel:ecp-01} -- due to the
  restricted space on the airport. In that sense, the Airport domain
  incorporates more planning aspects than UMTS.} The only point of the
domain, and, indeed, of using a computer to solve it, is to provide
{\em good} schedules, that is, schedules with the smallest possible
execution time, corresponding to the makespan of the plan.


That said, we observe that the satisficing planners in IPC-4 were
quite good at finding near-optimal plans in UMTS. In fact, as we will
see in detail in the following, the only planner finding highly
non-optimal plans was LPG-3.  Let's consider the basic domain version
treated in Figure~\ref{umts:notw} (a) and (b). Two of the
participating planners, CRIKEY and SGPlan, try to minimize the number
of actions (i.e., the wrong optimization criterion). Their data is
identical, i.e. the plan ``lengths'' are the same for all instances.
Precisely, both planners find, for each instance number $x$, a plan
with $\lfloor x/5 \rfloor*8$ actions in it. This is, in fact, the
optimal (smallest possible) number of actions -- remember what we said
above about the scaling in the IPC-4 test suites. The participating
planners trying to minimize makespan are LPG-3, LPG-TD, P-MEP,
HSP$_a^*$, and TP4. P-MEP solves only the smallest 5 instances,
finding the optimal plans. The ratio LPG-TD.speed vs HSP$_a^*$ is
$[1.00 (1.02) 1.11]$. The ratio LPG-TD.quality vs HSP$_a^*$ is $[1.00 (1.00)
1.03]$. The ratio LPG-3 vs HSP$_a^*$ is $[1.00 (1.53) 2.27]$; we remark that
the plan quality data used here is for ``LPG-3.bestquality'', which
takes the entire available half hour time trying to optimize the found
plan. Looking at the plots, one sees that the LPG-3 makespan curve is
much steeper than those of the other planners.







In Figure~\ref{umts:notw} (c) and (d), we see the performance of the
IPC-4 planners in the same basic domain version, but with the flaw
construct. LPG-TD remains unaffected, but SGPlan and CRIKEY become a
lot worse. Particularly, CRIKEY now takes several minutes to solve
even the smallest instances. We take this to confirm our intuition
that the flaw can (but does not necessarily) confuse the heuristic
functions of relaxed-plan based heuristic planners. Whether or not the
heuristic function becomes confused probably depends on details in the
particular way the relaxed plans are constructed (such a construction
may, e.g., choose between different actions based on an estimate of
how harmful they are to already selected actions). In the optimal
track, when introducing the flaw construct into the domain, the
performance of TP4 and HSP$_a^*$ becomes slightly worse, and nearly
indistinguishable.  Regarding plan quality, there now is a quality
difference in terms of the number of actions needed by CRIKEY and
SGPlan. SGPlan's plans still all have the smallest possible
``length'', $\lfloor x/5 \rfloor*8$. Those of CRIKEY have a lot of
variance, and are longer; the ratio CRIKEY vs SGPlan is $[1.07 (1.72)
3.88]$.  In the group minimizing makespan, the observations are very
similar to the unflawed domain version above.  The ratio LPG-TD.speed
vs HSP$_a^*$ is $[1.00 (1.01) 1.04]$, and the ratio LPG-TD.quality vs
HSP$_a^*$ is $[1.00 (1.00) 1.01]$. Although it solves only the smaller
half of the instances, the ratio LPG-3.bestquality vs HSP$_a^*$ is
$[1.00 (1.48) 2.27]$.







\begin{figure}[t]
\begin{center}
\vspace{-0.0cm}
\begin{tabular}{cc}
\includegraphics[width=7.3cm]{RESULTS/UMTS/TEMPORAL_TIMEWINDOWS/GNUPLOT/Time-suboptimal.eps} &
\includegraphics[width=7.3cm]{RESULTS/UMTS/FLAW_TEMPORAL_TIMEWINDOWS/GNUPLOT/Time-suboptimal.eps} \\
(a) & (b)
\end{tabular}
\vspace{-0.0cm}
\end{center}
\caption{UMTS-timewindows (a); UMTS-flaw-timewindows (b).}
\label{umts:tw}
\end{figure}




Figure~\ref{umts:tw} shows the results in the two domain versions with
explicitly encoded time windows. No optimal planners could participate
since none of them could handle timed initial literals. In the version
without the flaw, again LPG-TD and SGPlan need only split seconds. The
only other competitor, Tilsapa, needs more runtime but also scales up
well. When introducing the flaw, the only competitors are SGPlan and
LPG-TD.  SGPlan's runtime performance becomes a lot worse, while
LPG-TD remains completely unaffected. Regarding plan quality, the
number of actions in SGPlan's plans is still $\lfloor x/5 \rfloor*8$
in all cases.  LPG-TD.speed and LPG-TD.quality return plans with
identical makespan in all cases. In the non-flawed version,
UMTS-timewindows, the makespan ratio Tilsapa vs LPG-TD is $[1.00 (1.20)
1.37]$.




We do not show runtime graphs for the domain versions with compiled
time windows. In UMTS-timewindows-compiled, SGPlan and CRIKEY
participated. Both scale up well and solve all instances, but SGPlan
needs only split seconds, while CRIKEY needs up to more than 100
seconds per instance in the larger cases. Both planners try to
minimize the number of actions, and both need exactly $\lfloor x/5
\rfloor*8+5$ actions for each instance number $x$ -- namely, the
optimal number $\lfloor x/5 \rfloor*8$ of actions as before, plus $5$
artificial actions encoding the time windows. In
UMTS-flaw-timewindows-compiled, the sole participating planner was
SGPlan. It solved only the smaller half of the instances, finding
plans of length $\lfloor x/5 \rfloor*8+6$ -- i.e., using one
unnecessary action in each instance (the action concerns an
application that does not need to be set up).





In domain version UMTS, we awarded 1st places to SGPlan, LPG-TD, and
HSP$_a^*$; we awarded 2nd places to CRIKEY and TP4. In domain version
UMTS-flaw, we awarded a 1st place to LPG-TD, and 2nd places to SGPlan,
HSP$_a^*$, and TP4. In version UMTS-timewindows, we awarded 1st places
to SGPlan and LPG-TD, and a 2nd place to Tilsapa. In
UMTS-flaw-timewindows, we awarded a 1st place to LPG-TD. In
UMTS-timewindows-compiled, we awarded a 1st place to SGPlan.




==> hoffmann05a/awards.tex <==







\section{IPC-4 Awards}
\label{awards}



The numbers of 1st and 2nd places achieved by the planners are shown
in Tables~\ref{awards-satisficing} and~\ref{awards-optimal}; planners
that never came in 1st or 2nd place are left out of the tables. 
Since many of the planners (6 of the satisficing planners, and 4 of
the optimal planners) only dealt with the purely propositional domain
versions (i.e., STRIPS or ADL), we counted the performance in these
domains separately.


\begin{table}[htb]
\begin{tabular}{lrrrrrrrr}
&
SGPlan &
LPG-TD &
FD &
FDD &
Macro-FF & 
YAHSP & 
CRIKEY &
Tilsapa \\
Propositional 
& 3 / 6
&1 / 6
&5 / 2
&6 / 3
&3 / 0
&4 / 1
&0 / 0 
&0 / 0\\
Temp/Metric
&13 / 2
&7 / 7
&
&
&
&
& 0 / 1
& 0 / 1\\ \hline

Total Count
&16 / 8
&8 / 13
&5 / 2
&6 / 3
&3 / 0
&4 / 1
&0 / 1
&0 / 1
\end{tabular}
\caption{\label{awards-satisficing}Summary of results: satisficing planners, number 
of 1st places / number of 2nd places.}
\end{table}


\begin{table}[htb]
\begin{tabular}{lrrrrrrrr}
&CPT 
&TP-4
&HSP$_a^*$
&SATPLAN
&Optiplan
&Semsyn
&BFHSP \\
Propositional 
&0 / 1
&0 / 0
&0 / 0
&5 / 1
&0 / 4
&0 / 2
&0 / 2 \\

Temp/Metric 
&3 / 0
&0 / 5
&1 / 2
&&&& \\ \hline

Total Count 
&3 / 1
&0 / 5
&1 / 2
&5 / 1
&0 / 4
&0 / 2
&0 / 2
\end{tabular}
\caption{\label{awards-optimal}Summary of results: optimal planners, number 
of 1st places / number of 2nd places.}
\end{table}



For the satisficing planners, based on our observations we decided to
award separate prizes for performance in the pure STRIPS and ADL
domains. For the optimal planners this seemed not appropriate due to,
first, the small number of planners competing in the temporal/metric
domains, and, second, the smaller overall number of competing systems
-- giving 4 prizes to 7 systems seemed too much.  Overall, the awards
made in the deterministic part of IPC-4 are the following:



\begin{itemize}
\item 1st Prize, Satisficing Propositional Track -- Fast (Diagonally) Downward, by Malte Helmert and Silvia Richter
\item 2nd Prize, Satisficing Propositional Track -- YAHSP, by Vincent Vidal
\item 2nd Prize, Satisficing Propositional Track -- SGPlan, by Yixin Chen, Chih-Wei Hsu and Benjamin W. Wah
\item 1st Prize, Satisficing Metric Temporal Track -- SGPlan, by Yixin Chen, Chih-Wei Hsu and Benjamin W. Wah
\item 2nd Prize, Satisficing Metric Temporal Track -- LPG-TD, by
  Alfonso Gerevini, Alessandro Saetti, Ivan Serina, and Paolo
  Toninelli
\item 1st Prize, Optimal Track -- SATPLAN, by Henry Kautz, David
  Roznyai, Farhad Teydaye-Saheli, Shane Neth, and Michael Lindmark
\item 2nd Prize, Optimal Track -- CPT, by Vincent Vidal and Hector Geffner 
\end{itemize}

We would like to re-iterate that the awarding of prizes is, and has to
be, a very sketchy ``summary'' of the results of a complex event such
as IPC-4. A few bits of information are just not sufficient to
summarize thousands of data points. Many of the decisions we took in
the awarding of the prizes, i.e. in the judgement of scaling behavior,
were very close. This holds especially true for most of the runtime
graphs concerning optimal planners, and for some of the runtime graphs
concerning satisficing propositional planners. What we think is best,
and what we encourage everybody to do, is to have a closer look at the
results plots for themselves. As said before, the full plots are
available in an online appendix.




%The above left aside, our congratulations to the awardees! And many
%thanks again to all the competitors, to the people who helped us
%creating the domains, and last but not least to the organizing
%committee who helped us set up the language PDDL2.2. All these people
%contributed to make IPC-4 such an exciting and fruitful event!!

==> hoffmann05a/bnf.tex <==








\section{BNF Description of PDDL2.2}
\label{bnf}



\setcounter{tocdepth}{2}



This appendix contains a complete BNF specification of the PDDL2.2
language. For readability, we mark with $(***)$ the points in the BNF
where, in comparison to PDDL2.1, the new language constructs of
PDDL2.2 are inserted.






\subsection{Domains}


Domains are defined exactly as in PDDL2.2, except that we now also
allow to define rules for derived predicates at the points where
operators (actions) are allowed.

\begin{nopagebreak}\begin{tabtt}
\bump \= $\langle$domain$\rangle$ \bump\bump\=::= (def\=ine (domain $\langle$name$\rangle$)\+\+\+\\
                        {[}$\langle$require-def$\rangle$]  \\
                        {[}$\langle$types-def$\rangle$]\req{:typing} \\
                        {[}$\langle$constants-def$\rangle$] \\
                       {[}$\langle$predicates-def$\rangle$] \\
                        {[}$\langle$functions-def$\rangle$]\req{:fluents} \\
                        $\langle$structure-def$\rangle$\zom) \-\-\\
  $\langle$require-def$\rangle$  \> ::= (:requirements $\langle$require-key$\rangle$\oom) \\
  $\langle$require-key$\rangle$  \> ::= {\em See Section~\ref{sec-requirements}} \\
  $\langle$types-def$\rangle$    \> ::= (:types $\langle$typed list (name)$\rangle$) \\
  $\langle$constants-def$\rangle$ \>::= (:constants $\langle$typed list (name)$\rangle$) \\
  $\langle$predicates-def$\rangle$ \> ::= (:predicates $\langle$atomic formula skeleton$\rangle$\oom) \\
  $\langle$atomic formula skeleton$\rangle$ \\
                \> ::= ($\langle$predicate$\rangle$ $\langle$typed list (variable)$\rangle$) \\
  $\langle$predicate$\rangle$ \> ::= $\langle$name$\rangle$ \\
  $\langle$variable$\rangle$ \> ::= ?$\langle$name$\rangle$ \\
  $\langle$atomic function skeleton$\rangle$ \\
                \> ::= ($\langle$function-symbol$\rangle$ $\langle$typed list (variable)$\rangle$) \\
  $\langle$function-symbol$\rangle$ \> ::= $\langle$name$\rangle$ \\
  $\langle$functions-def$\rangle$ \> ::=\req{:fluents} (:fun\=ctions $\langle$function typed list \\
  \> \>                                 (atomic function skeleton)$\rangle$) \\
  $\langle$structure-def$\rangle$ \>::= $\langle$action-def$\rangle$\\
  $\langle$structure-def$\rangle$ \>::=\req{:durative-actions} $\langle$durative-action-def$\rangle$\\
\hspace{-1.2cm} $(***)$  $\langle$structure-def$\rangle$ \>::=\req{:derived-predicates} $\langle$derived-def$\rangle$\\
\= $\langle$typed list ($x$)$\rangle$ \=::= $x$\zom\+\\
  $\langle$typed list ($x$)$\rangle$ \>::=\req{:typing} $x$\oom - $\langle$type$\rangle$ $\langle$typed list($x$)$\rangle$\\
  $\langle$primitive-type$\rangle$\> ::= $\langle$name$\rangle$ \\
  $\langle$type$\rangle$ \> ::= (either $\langle$primitive-type$\rangle$\oom) \\
  $\langle$type$\rangle$ \> ::= $\langle$primitive-type$\rangle$ \\
\=  $\langle$function typed list ($x$)$\rangle$ \=::= $x$\zom\+\\
  $\langle$function typed list ($x$)$\rangle$ \>::=\req{:typing} $x$\oom - $\langle$\=function type$\rangle$ \\
  \> \> $\langle$function typed list($x$)$\rangle$\\
  $\langle$function type$\rangle$ \> ::= number \\
\end{tabtt}\end{nopagebreak}





\subsection{Actions}


The BNF for an action definition is the same as in PDDL2.2.

\begin{nopagebreak}\begin{tabtt}
\bump\=  $\langle$action-def$\rangle$ \bump \= ::= (:act\=ion $\langle$action-symbol$\rangle$\+\+\+\\
                        :parameters  ( $\langle$typed list (variable)$\rangle$ ) \\
                        $\langle$action-def body$\rangle$) \-\-\\
   $\langle$action-symbol$\rangle$ \> ::= $\langle$name$\rangle$ \\
   $\langle$action-def body$\rangle$ \>::= 
\=
                        {[}:precondition $\langle$GD$\rangle$] \+\+\\
                       {[}:effect       $\langle$effect$\rangle$]  \-\-\\
\= $\langle$GD$\rangle$ \hspace{3cm} \= ::= () \+\\
  $\langle$GD$\rangle$ \>::= $\langle$atomic formula(term)$\rangle$ \\
  $\langle$GD$\rangle$ \>::=\req{:negative-preconditions} $\langle$literal(term)$\rangle$\\
  $\langle$GD$\rangle$ \>::= (and $\langle$GD$\rangle$\zom) \\
  $\langle$GD$\rangle$ \> ::=\req{:disjunctive-preconditions} (or  $\langle$GD$\rangle$\zom) \\
  $\langle$GD$\rangle$\> ::=\req{:disjunctive-preconditions} (not $\langle$GD$\rangle$) \\
  $\langle$GD$\rangle$\> ::=\req{:disjunctive-preconditions} (imply $\langle$GD$\rangle$ $\langle$GD$\rangle$) \\
\smallskip
  $\langle$GD$\rangle$\> ::=\=\req{:existential-preconditions}  \+\+\\
             (exists ($\langle$typed list(variable)$\rangle$\zom) $\langle$GD$\rangle$ )\-\-\\ 
\smallskip
  $\langle$GD$\rangle$\> ::=\=\req{:universal-preconditions} \+\+\\
            (forall ($\langle$typed list(variable)$\rangle$\zom) $\langle$GD$\rangle$ ) \-\-\\ 
  $\langle$GD$\rangle$\> ::=\=\req{:fluents} $\langle$f-comp$\rangle$ \\
  $\langle$f-comp$\rangle$\> ::= ($\langle$binary-comp$\rangle$ $\langle$f-exp$\rangle$ $\langle$f-exp$\rangle$) \\
  $\langle$literal($t$)$\rangle$ \>::= $\langle$atomic formula($t$)$\rangle$ \\
  $\langle$literal($t$)$\rangle$ \>::= (not $\langle$atomic formula($t$)$\rangle$) \\
  $\langle$atomic formula($t$)$\rangle$ \>::= ($\langle$predicate$\rangle$ $t$\zom) \\
  $\langle$term$\rangle$ \> ::= $\langle$name$\rangle$ \\
  $\langle$term$\rangle$ \> ::= $\langle$variable$\rangle$ \\
  $\langle$f-exp$\rangle$ \> ::= $\langle$number$\rangle$ \\
  $\langle$f-exp$\rangle$ \> ::= ($\langle$binary-op$\rangle$ $\langle$f-exp$\rangle$ $\langle$f-exp$\rangle$) \\
  $\langle$f-exp$\rangle$ \> ::= (- $\langle$f-exp$\rangle$)\\
  $\langle$f-exp$\rangle$ \> ::= $\langle$f-head$\rangle$ \\
  $\langle$f-head$\rangle$ \> ::= ($\langle$function-symbol$\rangle$ $\langle$term$\rangle$\zom) \\
  $\langle$f-head$\rangle$ \> ::= $\langle$function-symbol$\rangle$ \\
  $\langle$binary-op$\rangle$ \> ::= $+$ \\
  $\langle$binary-op$\rangle$ \> ::= $-$ \\
  $\langle$binary-op$\rangle$ \> ::= $*$ \\
  $\langle$binary-op$\rangle$ \> ::= $/$ \\
  $\langle$binary-comp$\rangle$ \> ::= $>$ \\
  $\langle$binary-comp$\rangle$ \> ::= $<$ \\
  $\langle$binary-comp$\rangle$ \> ::= $=$ \\
  $\langle$binary-comp$\rangle$ \> ::= $>=$ \\
  $\langle$binary-comp$\rangle$ \> ::= $<=$ \\
  $\langle$number$\rangle$ \> ::= {\em Any numeric literal} \\
 \> $\quad$ {\em (integers and floats of form $n.n$).}\\
\=   $\langle$effect$\rangle$ \bump\= ::= () \+\\
  $\langle$effect$\rangle$ \> ::= (and $\langle$c-effect$\rangle$\zom)\\
  $\langle$effect$\rangle$ \> ::= $\langle$c-effect$\rangle$ \\
  $\langle$c-effect$\rangle$ \> ::=\req{:conditional-effects} (forall ($\langle$variable$\rangle$\zom) $\langle$effect$\rangle$) \\
  $\langle$c-effect$\rangle$ \>::=\req{:conditional-effects} (when $\langle$GD$\rangle$ $\langle$cond-effect$\rangle$) \\
  $\langle$c-effect$\rangle$ \>::= $\langle$p-effect$\rangle$ \\
  $\langle$p-effect$\rangle$ \> ::= ($\langle$assign-op$\rangle$ $\langle$f-head$\rangle$ $\langle$f-exp$\rangle$) \\
  $\langle$p-effect$\rangle$ \> ::= (not $\langle$atomic formula(term)$\rangle$) \\
  $\langle$p-effect$\rangle$ \>::= $\langle$atomic formula(term)$\rangle$  \\
  $\langle$p-effect$\rangle$ \>::=\req{:fluents}($\langle$assign-op$\rangle$ $\langle$f-head$\rangle$ $\langle$f-exp$\rangle$) \\  
  $\langle$cond-effect$\rangle$ \>::= (and $\langle$p-effect$\rangle$\zom)\\
  $\langle$cond-effect$\rangle$ \>::= $\langle$p-effect$\rangle$\\
  $\langle$assign-op$\rangle$ \>::= assign \\
  $\langle$assign-op$\rangle$ \>::= scale-up \\
  $\langle$assign-op$\rangle$ \>::= scale-down \\
  $\langle$assign-op$\rangle$ \>::= increase \\
  $\langle$assign-op$\rangle$ \>::= decrease \\
\end{tabtt}\end{nopagebreak}







\subsection{Durative Actions}



Durative actions are the same as in PDDL2.2, except that we restrict
ourselves to level 3 actions, where the duration is given as the fixed
value of a numeric expression (rather than as the possible values
defined by a set of constraints). This slightly simplifies the BNF.


\begin{nopagebreak}\begin{tabtt}
\bump\=  $\langle$durative-action-def$\rangle$ \= ::= (:dur\=ative-action $\langle$da-symbol$\rangle$\+\+\+\\
                        :parameters  ( $\langle$typed list (variable)$\rangle$ ) \\
                        $\langle$da-def body$\rangle$) \-\-\\
   $\langle$da-symbol$\rangle$ \> ::= $\langle$name$\rangle$ \\
   $\langle$da-def body$\rangle$ \>::= 
\=
                                :duration (= ?duration $\langle$f-exp$\rangle$) \+\+\\
                        :condition $\langle$da-GD$\rangle$\\
                        :effect $\langle$da-effect$\rangle$\-\-\\
\= $\langle$da-GD$\rangle$ \hspace{3cm} \= ::= () \+\\
  $\langle$da-GD$\rangle$ \>::= $\langle$timed-GD$\rangle$ \\
  $\langle$da-GD$\rangle$ \>::= (and $\langle$timed-GD$\rangle$\oom) \\
  $\langle$timed-GD$\rangle$ \>::= (at $\langle$time-specifier$\rangle$ $\langle$GD$\rangle$)\\
  $\langle$timed-GD$\rangle$ \>::= (over $\langle$interval$\rangle$ $\langle$GD$\rangle$)\\
  $\langle$time-specifier$\rangle$ \>::= start\\
  $\langle$time-specifier$\rangle$ \>::= end\\
  $\langle$interval$\rangle$ \>::= all\\
\end{tabtt}\end{nopagebreak}











\subsection{Derived predicates}




As said, rules for derived predicates can be given in the domain
description at the points where actions are allowed. The BNF is:



\begin{nopagebreak}\begin{tabtt}
\bump\= \hspace{-1.0cm} $(***)$  $\langle$derived-def$\rangle$ \bump \= ::= (:der\=ived $\langle$typed list (variable)$\rangle$
$\langle$GD$\rangle$)\\ 
\end{tabtt}\end{nopagebreak}


Note that we allow the specification of types with the derived
predicate arguments. This might seem redundant as the predicate types
are already declared in the {\tt :predicates} field. Allowing to
specify types with the predicate (rule) ``parameters'' serves to give
the language a more unified look-and-feel, and one might use the
option to make the parameter ranges more restrictive. (Remember that
the specification of types is optional, not mandatory.)



Repeating what has been said in Section~\ref{pddl:derived:syntax},
this BNF is more generous than what is considered a well-formed domain
description in PDDL2.2. We call a predicate $P$ {\em derived} if there
is a rule that has a predicate $P$ in its head; otherwise we call $P$
{\em basic}. The restrictions we apply are:


\begin{enumerate}
\item The actions available to the planner do not affect the derived
  predicates: no derived predicate occurs on any of the effect lists
  of the domain actions.
\item If a rule defines that $P(\overline{x})$ can be derived from
  $\phi(\overline{x})$, then the variables in $\overline{x}$ are
  pairwise different (and, as the notation suggests, the free
  variables of $\phi(\overline{x})$ are exactly the variables in
  $\overline{x}$).
\item If a rule defines that $P(\overline{x})$ can be derived from
  $\phi$, then the Negation Normal Form (NNF) of $\phi(\overline{x})$
  does not contain any derived predicates in negated form.
\end{enumerate}







\subsection{Problems}





The only change made to PDDL2.1 in the problem description is that we
allow the specification of timed initial literals.



\begin{nopagebreak}\begin{tabtt}
\bump\=$\langle$problem$\rangle$ \bump\bump \=::= (def\=ine (problem $\langle$name$\rangle$) \+\+\+\\
                                      (:domain $\langle$name$\rangle$) \\
                                     {[}$\langle$require-def$\rangle$] \\
                                      {[}$\langle$object declaration$\rangle$ ] \\
                                                          $\langle$init$\rangle$ \\
                                      $\langle$goal$\rangle$ \\
                                      {[}$\langle$metric-spec$\rangle$]\\
 % I think that length is a mistake, but it is used, so maybe we should include it?
                                      {[}$\langle$length-spec$\rangle$ ])\-\-\\
   $\langle$object declaration$\rangle$ ::= (:objects $\langle$typed list (name)$\rangle$) \\
   $\langle$init$\rangle$ \> ::= (:init $\langle$init-el$\rangle$\zom) \\
   $\langle$init-el$\rangle$ \> ::= $\langle$literal(name)$\rangle$\\
   $\langle$init-el$\rangle$ \> ::=\req{:fluents} (= $\langle$f-head$\rangle$ $\langle$number$\rangle$)\\
 \hspace{-1.2cm} $(***)$   $\langle$init-el$\rangle$ \> ::=\req{:timed-initial-literals} (at $\langle$number$\rangle$ $\langle$literal(name)$\rangle$)\\
   $\langle$goal$\rangle$ \> ::= (:goal $\langle$GD$\rangle$) \\
   $\langle$metric-spec$\rangle$ \> ::= (:metric $\langle$optimization$\rangle$ $\langle$ground-f-exp$\rangle$)\\
   $\langle$optimization$\rangle$ \> ::= minimize\\
   $\langle$optimization$\rangle$ \> ::= maximize\\
   $\langle$ground-f-exp$\rangle$ \> ::= ($\langle$binary-op$\rangle$ $\langle$ground-f-exp$\rangle$ $\langle$ground-f-exp$\rangle$)\\
   $\langle$ground-f-exp$\rangle$ \> ::= (- $\langle$ground-f-exp$\rangle$)\\
   $\langle$ground-f-exp$\rangle$ \> ::= $\langle$number$\rangle$\\
   $\langle$ground-f-exp$\rangle$ \> ::= ($\langle$function-symbol$\rangle$ $\langle$name$\rangle$\zom)\\
   $\langle$ground-f-exp$\rangle$ \> ::= total-time\\
   $\langle$ground-f-exp$\rangle$ \> ::= $\langle$function-symbol$\rangle$\\
\end{tabtt}
\end{nopagebreak}


Repeating what has been said in Section~\ref{pddl:derived:syntax}, the
requirement flag for timed initial literals implies the requirement
flag for durational actions (see also Section~\ref{sec-requirements}),
i.e. the language construct is only available in PDDL2.2 level 3.
Also, the above BNF is more generous than what is considered a
well-formed problem description in PDDL2.2. The times {\tt
  $\langle$number$\rangle$} at which the timed literals occur are
restricted to be greater than $0$. If there are also derived
predicates in the domain, then the timed literals are restricted to
not influence any of these, i.e., like action effects they are only
allowed to affect the truth values of the basic (non-derived)
predicates (IPC-4 will not use both derived predicates and timed
initial literals within the same domain).





\subsection{Requirements}
\label{sec-requirements}

\begin{sloppypar}
  Here is a table of all requirements in PDDL2.2. Some requirements
  imply others; some are abbreviations for common sets of
  requirements.  If a domain stipulates no requirements, it is assumed
  to declare a requirement for {\tt :strips}.
\begin{center}
{\small \begin{tabular}{ll}
\it Requirement & \it Description \\
\tt :strips & Basic STRIPS-style adds and deletes \\
\tt :typing & Allow type names in declarations of variables \\
\tt :negative-preconditions & Allow {\tt not} in goal descriptions\\
\tt :disjunctive-preconditions & Allow {\tt or} in goal descriptions \\
\tt :equality & Support {\tt =} as built-in predicate \\
\tt :existential-preconditions & Allow  {\tt exists} in
goal descriptions \\
\tt :universal-preconditions & Allow {\tt forall}  in
goal descriptions \\
\tt :quantified-preconditions & = {\tt :existential-preconditions}  \\
  & + {\tt :universal-preconditions} \\
\tt :conditional-effects & Allow {\tt when} in action effects \\
\tt :fluents & Allow function definitions and use of effects using\\
 & assignment operators and arithmetic preconditions.\\
\tt :adl & = {\tt :strips} + {\tt :typing}\\
   &      + {\tt :negative-preconditions}\\
   &      + {\tt :disjunctive-preconditions} \\
   &      + {\tt :equality}  \\
   &      + {\tt :quantified-preconditions}  \\
&+ {\tt :conditional-effects} \\
\tt :durative-actions & Allows durative actions. \\
& Note that this does not imply {\tt :fluents}.\\
\tt :derived-predicates & Allows predicates whose truth value is\\
& defined by a formula\\
\tt :timed-initial-literals & Allows the initial state to specify
literals\\
& that will become true at a specified time point\\
& implies {\tt durative actions} (i.e. applicable only\\
& in PDDL2.2 level 3)
\end{tabular}}
\end{center}
\end{sloppypar}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 












%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> hoffmann05a/conclusion.tex <==














\section{Conclusion}
\label{conclusion}










All in all, our feeling as the organizers is that the deterministic
part of IPC-4 was a great success, and made several valuable
contributions to the field. To mention the, from our perspective, two
most prominent points: the event provided the community with a set of
interesting new benchmarks, and made visible yet another major step
forward in the scalability of satisficing planning systems. The latter
was made possible by novel heuristics and domain analysis techniques.




There is a wide variety of questions to be addressed in the context of
the future of the (deterministic part of) the IPC. Let us discuss just
a few that we feel are important. Regarding benchmark domains, as said
we invested significant effort into the IPC-4 benchmarks, and we would
definitely recommend to re-use some of them in future IPC editions.
While some domain versions were solved relatively easily by certain
groups of planners, many of them still constitute major challenges.
Examples are Pipesworld with tankage restrictions, Optical-Telegraph,
large PSR instances, and UMTS for optimal planners.  That said, most
of the IPC-3 domains are also still challenging and should be re-used.
It is probably more useful for the community to consolidate
performance on the existing set of benchmarks, rather than to increase
the benchmark database at large pace. For one thing, to measure
progress between IPC editions, re-used benchmark domains (and
instances), like Satellite and Settlers in the case of IPC-4, are more
useful.\footnote{In the field addressing the SAT problem, particularly
  in the respective competition events, progress is also often
  measured simply in terms of the size (number of variables and
  clauses) of the formulas that could be tackled successfully, making
  just a few distinctions about the origin of the formulas (like,
  randomly generated or from an application). In the context of the
  IPC, one can do similar things by measuring parameters such as,
  e.g., the number of ground actions tackled successfully. However,
  given the large differences between the individual domains used in
  the IPC, more distinctions must be made. A detailed investigation of
  the effect of several parameters, in the IPC-4 domains, is given by
  \citeA{Benchmarks}.} More generally, the benchmark set is already
large; if there is a too large set, then a situation may arise where
authors select rather disjoint subsets in their individual
experiments.


Regarding PDDL extensions, the formalisms for derived predicates and
timed initial literals that we introduced are only first steps into
the respective directions. The PDDL2.2 derived predicates formalism is
restrictive in that it allows no negative interactions between derived
predicates; one could easily allow negative interactions that do not
lead to cycles and thus to ambiguous semantics
\cite{thiebaux:etal:ijcai-03,thiebaux:etal:ai-05}.  One could also
imagine derivation rules for values of more general data types than
predicates/Booleans, particularly for numeric variables. As for timed
initial literals, obviously they encode only a very restrictive subset
of the wide variety of forms that exogenous events can take. Apart
from exogenous events on numeric values, such events may in reality be
continuous processes conditioned on the world state, rather than
finitely many discrete time instants known beforehand. The PDDL2.2
action model itself is, of course, still restrictive in its
postulation of discrete variable value updates.  Still we believe that
the IPC should not let go off the very simple PDDL subsets such as
STRIPS, to support accessibility of the competition. As noted in
Section~\ref{systems:overview}, most systems are still not able to
handle all the language features introduced with IPC-3 and IPC-4.
Also, we believe that a STRIPS track, and more generally domain
versions formulated in simple language subsets, is important to
encourage basic algorithms research. A new idea is easier to try in a
simple language. To avoid misunderstandings: the language features
introduced with PDDL2.1 and PDDL2.2 already have a significant basis
of acceptance in implemented systems, and should definitely be kept
for future editions of the IPC.




In the context of basic research, it should be noted that the
satisficing track of IPC-4 was almost entirely populated by planners
of the relaxed-plan based heuristic search type. This demonstrates the
danger of the competition to concentrate research too much around a
few successful methods. Still, two of the most remarkable planners in
that track, Fast-Downward and SGPlan, use a significantly different
heuristic and new domain analysis techniques as the basis of their
success, respectively.


Putting the optimal planners in a separate track serves to maintain
this, very different, type of planning algorithms. We recommend to
keep this distinction in the future IPC events.




About the hand-tailored track, we have to say that it seems unclear if
and how that could be brought back into the focus. Maybe a more
suitable form of such an event would be an online (at the hosting
conference) programming (i.e., planner tailoring) competition. This
would, of course, imply a much smaller format for the event than the
format the IPC for automated planners has grown to already. But an
online hand-tailored competition would have the advantage of better
visibility of programming efforts, and of not taking up prohibitively
much time of the system developers.





In the context of competition size, last not least there are a few
words to be said about the role and responsibilities of the
organizers.  The IPC has grown too large to be handled, in all its
aspects, by just two persons. It may be worth thinking about
distributing the organization workload among a larger group of people.
One approach that might make sense would be to let different people
organize the tracks concerning the different PDDL subsets. Another
approach would be to let different people handle the language
definition, the benchmark preparation, and the results collection,
respectively. It would probably be a good idea to establish an IPC
council that, unlike the organizing committees in the past, would
persist across individual competitions, and whose role would be to
actively set up and support the organizing teams.





==> hoffmann05a/introduction.tex <==











\section{Introduction}
\label{introduction}






In the application of Artificial Intelligence technology to the
real-world, time and space resources are usually limited. This has led
to a performance-oriented interpretation of AI in many of its research
branches. Competition events have been established in automated
theorem proving, in satisfiability testing, and, in particular, in AI
Planning. A competition provides a large-scale evaluation platform.
Due to the broadness and neutrality of that platform, a competition is
far better at assessing the state-of-the-art in a research branch than
the experiments ran by individual authors: more systems are compared,
and the benchmarks are chosen by the competition organizers, rather
than by the system authors themselves. Moreover, a competition can
serve to establish a common representation formalism, and a common
core set of benchmarks, marking the edge of current system
capabilities.


The International Planning Competition ({IPC}) is a biennial
event, hosted at the international conferences on AI Planning and
Scheduling. The IPC began in 1998 when Drew McDermott and a committee
created a common specification language (PDDL) and a collection of
problems forming a first benchmark~\cite{pddl-handbook}.  PDDL is a
Lisp-like input language description format that includes planning
formalisms like STRIPS~\cite{fikes:nilsson:ai-71}.  Five systems
participated in the first international planning competition, IPC-1
for short, hosted at AIPS~1998 in Pittsburgh,
Pennsylvania~\cite{mcdermott:aim-00}.

In the year 2000, Fahiem Bacchus continued this work, and the IPC-2
event attracted 16 competitors~\cite{bacchus:aim-01}. The event --
hosted at AIPS~2000 in Breckenridge, Colorado -- was extended to
include both fully automatic and hand-tailored planning systems. As
hand-tailored planners were allowed to use some additional
domain-dependent information to the PDDL input in order to improve
their performance, they participated in an additional, separate,
track. Both STRIPS and ADL~\cite{pednault:kr-89} domains were used but
no further extensions were made to the
language~\cite{pddl-2000-subset}.



The 3rd International Planning Competition, IPC-3, was run by Derek
Long and Maria Fox and was hosted at AIPS~2002, Toulouse, France.  The
competition attracted 14 competitors \cite{long:fox:jair-03}, and
focussed on planning in temporal and metric domains. For that purpose,
Fox and Long developed the PDDL2.1 language~\cite{fox:long:jair-03},
of which the first three {\em levels} were used in IPC-3. Level 1 was
STRIPS and ADL planning as before, Level 2 added numeric variables,
Level 3 added durational constructs.

\begin{sloppypar}
  The 4th International Planning Competition, IPC-4, was hosted at
  ICAPS-2004, Whistler, Canada. IPC-4 built on the previous efforts,
  in particular the language PDDL2.1. The competition event was
  extended and revised in several respects. In particular, IPC-4
  featured, for the first time, a competition for probabilistic
  planners, so that the overall competition was split into a {\em
    deterministic} part -- a continuation of the previous events -- as
  well as a {\em probabilistic} part.\footnote{While IPC-4 was
    running, the deterministic part was named ``classical'' part. We
    re-named it into ``deterministic'' part since that wording is less
    ambiguous.} In the latter part, co-organized by Michael Littman
  and H{\aa}kan Younes, the main objective of the event was to
  introduce a common representation language for probabilistic
  planners, and to establish some first benchmarks and results. For
  more information on the probabilistic part of IPC-4 see the work of
  \citeA{ProbabilisticPart}.
\end{sloppypar}



Herein, we provide an overview of the organization and results of the
deterministic part of IPC-4. With 19 competing systems (21 when
counting different system versions), the event was even a little
larger than its already large predecessors.  Several important
revisions were made to the event. We briefly explain the main
differences in Section~\ref{revisions}.  Afterwards,
Section~\ref{pddl} describes the input language used, named {\em
  PDDL2.2}: the first three levels of PDDL2.1, extended with
\emph{derived predicates} and \emph{timed initial literals}.
Section~\ref{systems} lists and briefly explains the competing
systems. Section~\ref{results} then presents, for each benchmark
domain, a selection of results plots, highlighting the most important
points. The entire set of data points is far too large to be presented
in detail. The full data, including plots for all results, is
available in an online appendix.  Section~\ref{awards} explains how we
awarded the competition prizes, Section~\ref{conclusion} closes the
paper with some concluding remarks. Appendix~\ref{bnf} gives a BNF
description of PDDL2.2.










%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> hoffmann05a/pddl.tex <==










\section{PDDL 2.2}
\label{pddl}









As said, the IPC-4 competition language PDDL2.2 is an extension of the
first three levels of PDDL2.1 \cite{fox:long:jair-03}. PDDL2.2
inherits the separation into the levels. The language features added
on top of PDDL2.1 are {\em derived predicates} (into levels 1,2, and
3) and {\em timed initial literals} (into level 3 only). We now
discuss these two features in that order, describing their syntax and
semantics. A full BNF description of PDDL2.2 is in Appendix~\ref{bnf}.


















\subsection{Derived Predicates}
\label{pddl:derived}





Derived predicates have been implemented in several planning systems
in the past, for example in UCPOP \cite{penberthy:weld:kr-92}. They
are predicates that are not affected by any of the actions available
to the planner. Instead, the predicate's truth values are derived by a
set of rules of the form {\bf if} $\phi(\overline{x})$ {\bf then}
$P(\overline{x})$.  The semantics, roughly, are that an instance of a
derived predicate (a derived predicate whose arguments are
instantiated with constants; a {\em fact}, for short) is TRUE if and
only if it can be derived using the available rules (more details
below). Under the name ``axioms'', derived predicates were a part of
the original PDDL language defined by McDermott \cite{pddl-handbook}
for the first planning competition, but they have never been put to
use in a competition benchmark (we use the name ``derived predicates''
instead of ``axioms'' in order to avoid confusion with safety
conditions).


Derived predicates combine several key aspects that made them a useful
language extension for IPC-4:

\begin{itemize}
\item They are practically motivated: in particular, they provide a
  concise and convenient means to express updates on the transitive
  closure of a relation. Such updates occur in domains that include
  structures such as paths or flows (electricity flows, chemical
  flows, etc.); in particular, the {\em PSR} domain includes this kind
  of structure.
\item They are also theoretically justified in that compiling them
  away can be infeasible. It was recently proved that, in the worst
  case, compiling derived predicates away results in an exponential
  blow up of either the problem description or the plan length
  \cite{thiebaux:etal:ijcai-03,thiebaux:etal:ai-05}.
\item Derived predicates do not cause a significant implementation
  overhead in, at least, the state transition routines used by forward
  search planners. When the world state -- the truth values of all
  non-derived, {\em basic}, predicates -- is known, computing the
  truth values of the derived predicates is trivial.\footnote{Note,
    though, that it may be much less trivial to adapt a heuristic
    function to handle derived predicates; this is, for example,
    discussed by \citeA{thiebaux:etal:ijcai-03,thiebaux:etal:ai-05}.}
\end{itemize}


In the IPC-4 benchmarks, derived predicates were used only in the
non-durational context, PDDL2.2 level 1.






\subsubsection{Syntax}
\label{pddl:derived:syntax}



The BNF definition of derived predicates involves just two small
modifications to the BNF definition of PDDL2.1:


\begin{center}
  {\tt {\small $\langle$structure-def$\rangle$ ::=\req{:derived-predicates}
      $\langle$derived-def$\rangle$}}
\end{center}

  
The domain file specifies a list of ``structures''. In PDDL2.1 these
were either actions or durational actions. Now we also allow
``derived'' definitions at these points.

\begin{center}
  {\tt {\small $\langle$derived-def$\rangle$ ::= (:derived
      $\langle$atomic formula(term)$\rangle$ $\langle$GD$\rangle$)}}
\end{center}

The ``derived'' definitions are the ``rules'' mentioned above. They
simply specify the predicate $P$ to be derived (with variable vector
$\overline{x}$), and the formula $\phi(\overline{x})$ from which
instances of $P$ can be concluded to be true. Syntactically, the
predicate and variables are given by the {\tt $\langle$atomic
  formula(term)$\rangle$} expression, and the formula is given by {\tt
  $\langle$GD$\rangle$} (a ``goal description'', i.e. a formula).


The BNF is more generous than what we actually allow in PDDL2.2,
respectively in IPC-4. We make a number of restrictions to ensure that
the definitions make sense and are easy to treat algorithmically. We
call a predicate $P$ {\em derived} if there is a rule that has a
predicate $P$ in its head; otherwise we call $P$ {\em basic}. The
restrictions we make are the following.

\begin{enumerate}
\item The actions available to the planner do not affect the derived
  predicates: no derived predicate occurs on any of the effect lists
  of the domain actions.
\item If a rule defines that $P(\overline{x})$ can be derived from
  $\phi(\overline{x})$, then the variables in $\overline{x}$ are
  pairwise different (and, as the notation suggests, the free
  variables of $\phi(\overline{x})$ are exactly the variables in
  $\overline{x}$).
\item If a rule defines that $P(\overline{x})$ can be derived from
  $\phi$, then the Negation Normal Form (NNF) of $\phi(\overline{x})$
  does not contain any derived predicates in negated form.
\end{enumerate}

The first restriction ensures that there is a separation between the
predicates that the planner can affect (the basic predicates) and
those (the derived predicates) whose truth values follow from the
basic predicates. The second restriction ensures that the rule right
hand sides match the rule left hand sides. Let us explain the third
restriction. The NNF of a formula is obtained by ``pushing the
negations downwards'', i.e. transforming $\neg \forall x: \phi$ into
$\exists x: (\neg \phi)$, $\neg \exists x: \phi$ into $\forall x:
(\neg \phi)$, $\neg \bigvee \phi_i$ into $\bigwedge (\neg \phi_i)$,
and $\neg \bigwedge \phi_i$ into $\bigvee (\neg \phi_i)$. Iterating
these transformation steps, one ends up with a formula where negations
occur only in front of atomic formulas -- predicates with variable
vectors, in our case. The formula contains a predicate $P$ {\em in
  negated form} if and only if there is an occurrence of $P$ that is negated. By
requiring that the formulas in the rules (that derive predicate
values) do not contain any derived predicates in negated form, we
ensure that there can not be any negative interactions between
applications of the rules (see the semantics below).



An example of a derived predicate is the ``above'' predicate in the
{\sl Blocksworld}, which is true between blocks $x$ and $y$ whenever
$x$ is transitively (possibly with some blocks in between) on $y$.
Using the derived predicates syntax, this predicate can be defined as
follows.

{\small
\begin{verbatim}
(:derived (above ?x ?y)
  (or (on ?x ?y) 
      (exists (?z) (and (on ?x ?z) 
                        (above ?z ?y)))))
\end{verbatim}}
  
  Note that formulating the truth value of ``above'' in terms of the
  effects of the normal {Blocksworld} actions is very awkward.
  Since the set of atoms affected by an action depends on the
  situation, one either needs artificial actions or complex
  conditional effects.





















\subsubsection{Semantics}
\label{pddl:derived:semantics}






We now describe the updates that need to be made to the PDDL2.1
semantics definitions given by \citeA{fox:long:jair-03}. We introduce
formal notations to capture the semantics of derived predicates. We
then ``hook'' these semantics into the PDDL2.1 language by modifying
two of \citeA{fox:long:jair-03}'s definitions.


Say we are given the truth values of all (instances of the) basic
predicates, and want to compute the truth values of the (instances of
the) derived predicates from that. We are in this situation every time
we have applied an action, or parallel action set. In the durational
context, we are in this situation at the ``happenings'' in our current
plan, that is every time a durative action starts or finishes.
Formally, what we want to have is a function ${\mathcal D}$ that maps
a set of basic facts (instances of basic predicates) to the same set
but enriched with derived facts (the derivable instances of the
derived predicates). Assume we are given the set $R$ of rules for the
derived predicates, where the elements of $R$ have the form
$(P(\overline{x}), \phi(\overline{x}))$ -- {\bf if}
$\phi(\overline{x})$ {\bf then} $P(\overline{x})$. Then ${\mathcal
  D}(s)$, for a set of basic facts $s$, is defined as follows.
\begin{equation}\label{eq-derived}
  {\mathcal D}(s) := \bigcap \{ s' \mid s \subseteq s', \forall
  (P(\overline{x}), \phi(\overline{x})) \in R: \forall \overline{c},
  |\overline{c}| = |\overline{x}|: (s' \models \phi(\overline{c}) \Rightarrow P(\overline{c}) \in s') \}
\end{equation}
This definition uses the standard notations of the modelling relation
$\models$ between states (represented as sets of facts in our case)
and formulas, and of the substitution $\phi(\overline{c})$ of the free
variables in formula $\phi(\overline{x})$ with a constant vector
$\overline{c}$. In words, ${\mathcal D}(s)$ is the intersection of all
supersets of $s$ that are closed under application of the rules $R$.


Remember that we restrict the rules to not contain any derived
predicates in negated form. This implies that the order in which the
rules are applied to a state does not matter (we can not ``lose'' any
derived facts by deriving other facts first). This, in turn, implies
that ${\mathcal D}(s)$ is itself closed under application of the rules
$R$. In other words, ${\mathcal D}(s)$ is the least fixed point over
the possible applications of the rules $R$ to the state where all
derived facts are assumed to be FALSE (represented by their not being
contained in $s$). 

More constructively, ${\mathcal D}(s)$ can be computed by the
following simple process.

\begin{tabbing}
$s' := s$\\
{\bf do} \=\\
\> {\bf select} \= a rule $(P(\overline{x}), \phi(\overline{x}))$ and a
vector $\overline{c}$ of constants,\\
\> \> with $|\overline{c}| = |\overline{x}|$, such that $s' \models \phi(\overline{c})$ and $P(\overline{c}) \not \in s'$\\
\> let $s' := s' \cup \{ P(\overline{c}) \}$\\
{\bf until} no such rule and constant vector exist\\
let ${\mathcal D}(s) := s'$
\end{tabbing}

In words, apply the applicable rules in an arbitrary order until no
new facts can be derived anymore.

We can now specify what an executable plan is in PDDL2.1 with derived
predicates. All we need to do is to hook the function ${\mathcal D}$
into Definition 13, ``Happening Execution'', given by
\citeA{fox:long:jair-03}. By this definition, \citeA{fox:long:jair-03}
define the state transitions in a plan. The happenings in a (temporal
or non-temporal) plan are all time points at which at least one action
effect occurs. \citeA{fox:long:jair-03}'s definition is this:

\bigskip

\noindent
{\bf Definition 13 Happening Execution} \cite{fox:long:jair-03}
\\ {\em Given a state, $(t,s,{\bf x})$ and a
  happening, $H$, the {\em activity} for $H$ is the set of grounded
  actions 
\begin{tabbing}
$A_{H} = \{a |$ \= $\mbox{the name for $a$ is in $H$, $a$ is
    valid and}$\\
\> $Pre_{a} \,\, \mbox{is satisfied in}\,\, (t,s,{\bf
    x})\}$
\end{tabbing}
The {\em result of executing a happening}, $H$, associated with time
$t_{H}$, in a state $(t,s,{\bf x})$ is undefined if $|A_{H}| \not=
|H|$ or if any pair of actions in $A_{H}$ is mutex. Otherwise, it is
the state $(t_{H},s',{\bf x'})$ where 
\begin{equation}\label{eq-foxlong-result}
s' = (s \setminus \bigcup_{a \in A_{H}} Del_{a}) \cup \bigcup_{a \in
  A_{H}} Add_{a} \hspace{0.5cm}
\end{equation}
and ${\bf x'}$ is the result of applying the composition of the
functions $\{${\em NPF}$_{a} \, | \, a \in A_{H}\}$ to {\bf x}.}


\medskip


Note that the happenings consist of grounded actions, i.e., all
operator parameters are instantiated with constants. To introduce the
semantics of derived predicates, we now modify the result of executing
the happening. (We will also adapt the definition of mutex actions,
see below.) The result of executing the happening is now obtained by
applying the actions to $s$, then subtracting all derived facts from
this, then applying the function ${\mathcal D}$.  That is, in the
above definition we replace Equation~\ref{eq-foxlong-result} with the
following:
\begin{equation}\label{eq-result-derived}
s' = {\mathcal D}(((s \setminus \bigcup_{a \in A_{H}} Del_{a}) \cup
\bigcup_{a \in A_{H}} Add_{a}) \setminus D)
\end{equation}
where $D$ denotes the set of all derived facts. If there are no
derived predicates, $D$ is the empty set and ${\mathcal D}$ is the
identity function.


As an example, say we have a {\sl Blocksworld} instance where A is on
B is on C, $s = \{ clear(A)$, $on(A,B)$, $on(B,C)$, $ontable(C)$,
$above(A,B)$, $above(B,C)$, $above(A,C) \}$, and our happening applies
an action that moves A to the table. Then the happening execution
result will be computed by removing $on(A,B)$ from $s$, adding
$clear(B)$ and $ontable(A)$ into $s$, removing all of $above(A,B)$,
$above(B,C)$, and $above(A,C)$ from $s$, and applying ${\mathcal D}$
to this, which will re-introduce (only) $above(B,C)$.  So $s'$ will be
$s' = \{ clear(A),$ $ontable(A),$ $clear(B),$ $on(B,C),$ $ontable(C),$
$above(B,C)$ $\}$.



By the definition of happening execution, \citeA{fox:long:jair-03}
define the state transitions in a plan. The definitions of what an
executable plan is, and when a plan achieves the goal, are then
standard. The plan is {\em executable} if the result of all happenings
in the plan is defined. This means that all action preconditions have
to be fulfilled in the state of execution, and that no two pairs of
actions in a happening are {\em mutex}. The plan {\em achieves the
  goal} if the goal holds true in the state that results after the
execution of all actions in the plan.



With our above extension of the definition of happening executions,
the definitions of plan executability and goal achievement need not be
changed. We do, however, need to adapt the definition of when a pair
of actions is mutex. This is important if the happenings can contain
more than one action, i.e., if we consider parallel (Graphplan-style)
or concurrent (durational) planning. \citeA{fox:long:jair-03} give a
conservative definition that forbids the actions to interact in any
possible way.  The definition is the following.


\bigskip

\noindent
{\bf Definition 12 Mutex Actions} \cite{fox:long:jair-03}
\\ 
{\em Two grounded actions,
$a$ and $b$ are {\em non-interfering} if 
{\small
\begin{equation}\label{eq-foxlong-mutex}
  \begin{array}{c}
  GPre_{a} \cap (Add_{b} \cup Del_{b}) = GPre_{b} \cap (Add_{a} \cup Del_{a}) = \emptyset,\\
  Add_{a} \cap Del_{b} = Add_{b} \cap Del_{a} = \emptyset,\\
  L_{a} \cap R_{b} = R_{a} \cap L_{b} = \emptyset,\\
  L_{a} \cap L_{b} \subseteq L^{*}_{a} \cup L^{*}_{b}
\end{array}
\end{equation}
}
If two actions are not non-interfering they are {\em mutex}.}

\medskip

Note that the definition talks about grounded actions where all
operator parameters are instantiated with constants. $L_{a}$, $L_b$,
$R_a$, and $R_b$ refer to the left and right hand side of $a$'s and
$b$'s numeric effects. $Add_a$/$Add_b$ and $Del_a$/$Del_b$ are $a$'s
and $b$'s positive (add) respectively negative (delete) effects.
$GPre_a$/$Gpre_b$ denotes all (ground) facts that occur in $a$'s/$b$'s
precondition. If a precondition contains quantifiers then these are
grounded out ($\forall x$ transforms to $\bigwedge c_i$, $\exists x$
transforms to $\bigvee c_i$ where the $c_i$ are all objects in the
given instance), and $GPre$ is defined over the resulting
quantifier-free (and thus variable-free) formula. Note that this
definition of mutex actions is very conservative -- if, for example,
fact $F$ occurs only positively in $a$'s precondition, then it does
not matter if $F$ is among the add effects of $b$. The conservative
definition has the advantage that it makes it algorithmically very
easy to figure out if or if not $a$ and $b$ are mutex.



In the presence of derived predicates, the above definition needs to
be extended to exclude possible interactions that can arise indirectly
due to derived facts, in the precondition of the one action, whose
truth value depends on the truth value of (basic) facts affected by
the effects of the other action. In the same spirit in that
\citeA{fox:long:jair-03} forbid any possibility of direct interaction,
we now forbid any possibility of indirect interaction. Assume we
ground out all rules $(P(\overline{x}), \phi(\overline{x}))$ for the
derived predicates, i.e., we insert all possible vectors
$\overline{c}$ of constants; we also ground out the quantifiers in the
formulas $\phi(\overline{c})$, ending up with variable free rules. We
define a directed graph where the nodes are (ground) facts, and an
edge from fact $F$ to fact $F'$ is inserted iff there is a grounded
rule $(P(\overline{c}), \phi(\overline{c}))$ such that $F' =
P(\overline{c})$, and $F$ occurs in $\phi(\overline{c})$. Now say we
have an action $a$, where all ground facts occurring in $a$'s
precondition are, see above, denoted by $GPre_a$. By $DPre_a$ we
denote all ground facts that can possibly influence the truth values
of the derived facts in $GPre_a$:
\begin{equation}\label{eq-derivedP}
DPre_a := \{ F \mid \mbox{there is a path from $F$ to an $F' \in GPre_a$}
\}
\end{equation}
The definition of mutex actions is now updated simply by replacing
Equation~\ref{eq-foxlong-mutex} with: {\small
\begin{equation}\label{eq-derivedmutex}
\begin{array}{c}
  (DPre_a \cup GPre_{a}) \cap (Add_{b} \cup Del_{b}) =\\
 (DPre_b \cup GPre_b) \cap (Add_{a} \cup Del_{a}) = \emptyset,\\
  Add_{a} \cap Del_{b} = Add_{b} \cap Del_{a} = \emptyset,\\
  L_{a} \cap R_{b} = R_{a} \cap L_{b} = \emptyset,\\
  L_{a} \cap L_{b} \subseteq L^{*}_{a} \cup L^{*}_{b}
\end{array}
\end{equation}
}Note that the only thing that has changed is the first line,
regarding interference of propositional effects and preconditions. As
an example, reconsider the {\sl Blocksworld} and the ``above''
predicate.  Assume that the action that moves a block $A$ to the table
requires as an additional, derived, precondition, that $A$ is above
some third block. Then, in principle, two actions that move two
different blocks $A$ and $B$ to the table can be executed in parallel.
Which block $A$ ($B$) is on can influence the $above$ relations in
that $B$ ($A$) participates; however, this does not matter because if
$A$ and $B$ can be both moved then this implies that they are both
clear, which implies that they are on top of different stacks anyway.
We observe that the latter is a statement about the domain semantics
that either requires non-trivial reasoning, or access to the world
state in which the actions are executed. In order to avoid the need to
either do non-trivial reasoning about domain semantics, or resort to a
forward search, our definition is the conservative one given above.
The definition makes the actions moving $A$ and $B$ mutex on the
grounds that they can possibly influence each other's derived
preconditions.






The definition adaptations described above suffice to define the
semantics of derived predicates for the whole of PDDL2.2.
\citeA{fox:long:jair-03} reduce the temporal case to the case of
simple plans above, so by adapting the simple-plan definitions we have
automatically adapted the definitions of the more complex cases. In
the temporal setting, PDDL2.2 level 3, the derived predicates
semantics are that their values are computed anew at each happening in
the plan where an action effect occurs. As said, in IPC-4 we used
derived predicates only in the non-temporal setting. Some remarks on
limitations of the IPC-4 treatment of derived predicates, and on
future prospects, are in Section~\ref{conclusion}.






























\subsection{Timed Initial Literals}
\label{pddl:timed}





Timed initial literals are a syntactically very simple way of
expressing a certain restricted form of exogenous events: facts that
will become TRUE or FALSE at time points that are known to the planner
in advance, independently of the actions that the planner chooses to
execute. Timed initial literals are thus deterministic unconditional
exogenous events. Syntactically, we simply allow the initial state to
specify -- beside the usual facts that are true at time point $0$ --
literals that will become true at time points greater than $0$.


Timed initial literals are practically very relevant: in the real
world, deterministic unconditional exogenous events are very common,
typically in the form of time windows -- within which a shop has
opened, within which humans work, within which traffic is slow, within
which there is daylight, within which a seminar room is occupied,
within which nobody answers their mail because they are all at
conferences, etc. The timed initial literals syntax is just about the
simplest way one can think of to communicate such things to a planner.


Timed initial literals can easily be compiled into artificial
constructs \cite{expressivepddl}, involving an only linear blow-up in
the instance representation and in plan length (i.e., number of
actions in it). Still it seems highly likely that handing the timed
literals over to an automated planner explicitly results in far better
performance than when one hands over the artificial (compiled)
representation. The results obtained in IPC-4 confirm this, see also
Section~\ref{results}.










\subsubsection{Syntax}
\label{pddl:timed:syntax}




The BNF notation is:


\begin{center}
  {\tt {\small $\langle$init$\rangle$ ::= (:init $\langle$init-el$\rangle$\zom)}}
\end{center}


\begin{center}
  {\tt {\small $\langle$init-el$\rangle$ ::=\req{:timed-initial-literals} (at $\langle$number$\rangle$ $\langle$literal(name)$\rangle$) }}
\end{center}



The requirement flag for timed initial literals implies the
requirement flag for durational actions, i.e., as said the language
construct is only available in PDDL2.2 level 3. The times {\tt
  $\langle$number$\rangle$} at which the timed literals occur are
restricted to be greater than $0$.  If there are also derived
predicates in the domain, then the timed literals are restricted to
not influence any of these, i.e., like action effects they are only
allowed to affect the truth values of the basic (non-derived)
predicates (IPC-4 will not use both derived predicates and timed
initial literals within the same domain).



As an illustrative example, consider a planning task where the goal is
to have completed the shopping. There is a single action {\sl
  go-shopping} that achieves the goal, and requires the (single) shop
to be open as the precondition. The shop opens at time 9 relative to
the initial state, and closes at time 20. We can express the shop
opening times by two timed initial literals:

{\small
\begin{verbatim}
(:init
  (at 9 (shop-open))
  (at 20 (not (shop-open)))
)
\end{verbatim}}
























\subsubsection{Semantics}
\label{pddl:timed:semantics}







We now describe the updates that need to be made to the PDDL2.1
semantics definitions given by \citeA{fox:long:jair-03}. Adapting two
of the definitions suffices.


The first definition we need to adapt is the one that defines what a
``simple plan'', and its happening sequence, is. The original
definition by \citeA{fox:long:jair-03} is this.

\bigskip

\noindent
{\bf Definition 11 Simple Plan} \cite{fox:long:jair-03}\\
{\em A {\em simple plan}, $SP$, for a planning instance, $I$, consists
  of a finite collection of {\em timed simple actions} which are pairs
  $(t,a)$, where $t$ is a rational-valued time and $a$ is an action
  name.
  
  The {\em happening sequence}, $\{t_{i}\}_{i=0\ldots k}$ for $SP$ is
  the ordered sequence of times in the set of times appearing in the
  timed simple actions in $SP$. All $t_{i}$ must be greater than $0$.
  It is possible for the sequence to be empty (an empty plan).
  
  The {\em happening} at time $t$, $E_{t}$, where $t$ is in the
  happening sequence of $SP$, is the set of (simple) action names that
  appear in timed simple actions associated with the time $t$ in
  $SP$.}

\medskip

In the STRIPS case, the time stamps are the natural numbers $1, \dots,
n$ when there are $n$ actions/parallel action sets in the plan. The
happenings then are the actions/parallel action sets at the respective
time steps. \citeA{fox:long:jair-03} reduce the temporal planning case
to the simple plan case defined here by splitting each durational
action up into at least two simple actions -- the start action, the
end action, and possibly several actions in between that guard the
durational action's invariants at the points where other action
effects occur. So in the temporal case, the happening sequence is
comprised of all time points at which ``something happens'', i.e., at
which some action effect occurs.




To introduce our intended semantics of timed initial literals, all we
need to do to this definition is to introduce additional happenings
into the temporal plan, namely the time points at which some timed
initial literal occurs. The timed initial literals can be interpreted
as simple actions that are forced into the respective happenings
(rather than selected into them by the planner), whose precondition is
true, and whose only effect is the respective literal. The rest of
\citeA{fox:long:jair-03}'s definitions then carry over directly
(except goal achievement, which involves a little care, see below).
The PDDL2.2 definition of simple plans is this here.


\bigskip

\noindent
{\bf Definition 11 Simple Plan}\\ {\em A {\em simple plan}, $SP$, for
  a planning instance, $I$, consists of a finite collection of {\em
    timed simple actions} which are pairs $(t,a)$, where $t$ is a
  rational-valued time and $a$ is an action name. By $t_{end}$ we
  denote the largest time $t$ in $SP$, or $0$ if $SP$ is empty.
  
  Let $TL$ be the (finite) set of all timed initial literals, given as
  pairs $(t,l)$ where $t$ is the rational-valued time of occurrence of
  the literal $l$. We identify each timed initial literal $(t,l)$ in
  $TL$ with a uniquely named simple action that is associated with
  time $t$, whose precondition is TRUE, and whose only effect is $l$.

  The {\em happening sequence}, $\{t_{i}\}_{i=0\ldots k}$ for $SP$ is
  the ordered sequence of times in the set of times appearing in the
  timed simple actions in $SP$ and $TL$. All $t_{i}$ must be greater than $0$.
  It is possible for the sequence to be empty (an empty plan).
  
  The {\em happening} at time $t$, $E_{t}$, where $t$ is in the
  happening sequence of $SP$, is the set of (simple) action names that
  appear in timed simple actions associated with the time $t$ in
  $SP$ or $TL$.}


\medskip


Thus the happenings in a temporal plan are all points in time where
either an action effect, or a timed literal, occurs. The timed
literals are simple actions forced into the plan. With this
construction, \citeA{fox:long:jair-03}'s Definitions~12 (Mutex
Actions) and~13 (Happening Execution), as described (and adapted to
derived predicates) in Section~\ref{pddl:derived:semantics}, can be
kept unchanged.  They state that no action effect is allowed to
interfere with a timed initial literal, and that the timed initial
literals are true in the state that results from the execution of the
happening they are contained in. \citeA{fox:long:jair-03}'s
Definition~14 (Executability of a plan) can also be kept unchanged --
the timed initial literals change the happenings in the plan, but not
the conditions under which a happening can be executed.



The only definition we need to reformulate is that of what the {\em
  makespan} of a valid plan is. In \citeA{fox:long:jair-03}'s original
definition, this is implicit in the definition of valid plans. The
definition is this.

\bigskip

\noindent
{\bf Definition 15 Validity of a Simple Plan} \cite{fox:long:jair-03}\\
{\em A simple plan (for a planning instance, $I$) is {\em valid} if it
  is executable and produces a final state $S$, such that the goal
  specification for $I$ is satisfied in $S$.}


\medskip

The makespan of the valid plan is accessible in PDDL2.1 and PDDL2.2 by
the ``total-time'' variable that can be used in the optimization
expression. Naturally, \citeA{fox:long:jair-03} take the makespan to
be the end of the plan, the time point of the plan's final state.




In the presence of timed initial literals, the question of what the
plan's makespan is becomes a little more subtle. With
\citeA{fox:long:jair-03}'s above original definition, the makespan
would be the end of all happenings in the simple plan, which {\em
  include} all timed initial literals (see the revised Definition 11
above). So the plan would at least take as long as it takes until no
more timed literals occur. But a plan might be finished long before
that -- imagine something that needs to be done while there is
daylight; certainly the plan does not need to wait until sunset. We
therefore define the makespan to be the earliest point in time at
which the goal condition becomes (and remains) true. Formally this
reads as follows.

\bigskip

\noindent
{\bf Definition 15 Validity and Makespan of a Simple Plan}\\
{\em A simple plan (for a planning instance, $I$) is {\em valid} if it
  is executable and produces a final state $S$, such that the goal
  specification for $I$ is satisfied in $S$. The plan's {\em makespan}
  is the smallest $t \geq t_{end}$ such that, for all happenings at
  times $t' \geq t$ in the plan's happening sequence, the goal
  specification is satisfied after execution of the happening.}

\medskip

Remember that $t_{end}$ denotes the time of the last happening in the
plan that contains an effect caused by the plan's {\em actions} -- in
simpler terms, $t_{end}$ is the end point of the plan. What the
definition says is that the plan is valid if, at some time point $t$
after the plan's end, the goal condition is achieved and remains true
until after the last timed literal has occurred. The plan's makespan is
the first such time point $t$. Note that the planner can ``use'' the
events to achieve the goal, by doing nothing until a timed literal
occurs that makes the goal condition true -- but then the waiting time
until the nearest such timed literal is counted into the plan's
makespan.  (The latter is done to avoid situations where the planner
could prefer to wait millions of years rather than just applying a
single action itself.) Remember that the makespan of the plan, defined
as above, is what can be denoted by {\tt total-time} in the
optimization expression defined with the problem instance.




As with the derived predicates, the definition adaptations above
suffice to define the semantics of timed initial literals for PDDL2.2.
Some remarks on limitations of the language construct, and on future
prospects, are in Section~\ref{conclusion}.





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% TeX-master: t
%%% End: 



==> hoffmann05a/results.tex <==











\section{Results}
\label{results}











The CPU times for IPC-4 were measured on a machine located in
Freiburg, running 2 Pentium-4 CPUs at 3 GHz, with 6 GB main memory.
Competitors logged in remotely and ran their planners, producing one
separate ASCII result file for each solved instance, giving the
runtime taken, the quality of the found plan, as well as the plan
itself. Each planner run was allowed at most half an hour (CPU, not
real) runtime, and 1 GB memory, i.e., these were the cutoff values for
solving a single instance. As a kind of performance measure, the IPC-3
version of LPG \cite{gerevini:etal:jair-03} (called ``LPG-3''), i.e.
the most successful automatic planner from IPC-3, was also run (by its
developers, on top of the workload with their new planner version
LPG-TD). We remark that, for the sake of simplicity, to save CPU time,
and to ensure fairness, randomized planners were allowed only a single
run one ach instance, with a fixed random seed.





IPC-4 featured a lot of domain versions and instances, and a lot of
planners. The only way to fully understand the results of such a
complex event is to examine the results in detail, making sense of
them in combination with the descriptions/PDDL encodings of the
domains, and the techniques used in the respective planners. We
recommend doing so, at least to some extent, to everybody who is
interested in the results of (the deterministic part of) IPC-4. The
on-line appendix of this paper includes all the individual solution
files. The appendix also includes all \emph{gnuplot} graphics we
generated (more details below), as well as a GANNT chart for each of
the result files; the GANNT charts can be visualized using the Vega
visualization front-end~\cite{Hipke:Dissertation}.





In what follows, we provide an overview of the results, and we
highlight (what we think are) the most important points; we explain
how we decided about the IPC-4 competition awards.


More precisely, Section~\ref{results:overview} gives an overview over
the results, in terms of percentages of attacked and solved instances
per language subset and planner. Section~\ref{results:evaluation}
describes how we evaluated the results, particularly what procedure we
chose to decide about the awards. Thereafter,
Sections~\ref{results:airport} to~\ref{results:umts} in turn consider
in some more detail the results in the single domains.



























\subsection{Results Overview}
\label{results:overview}






One crude way to obtain an overview over such a large data set is to
simply count the number of instances each planner {\em attacked}, i.e.
tried to solve, and those that it succeeded to solve. In our case, it
also makes sense to distinguish between the different PDDL2.2 subsets
used by the IPC-4 benchmarks. The data is displayed in
Table~\ref{tab:results-overview}.

\setlength{\tabcolsep}{3.5pt}


\begin{table}[t]
\centering
\begin{small}
\centering
\begin{tabular}{|l||rr|rr|rr|rr|rr|rr|rr||rrr|}
\hline    
              &  \multicolumn{2}{|c|}{N}       & \multicolumn{2}{|c|}{N+DP}    & \multicolumn{2}{|c|}{N+NV}    & \multicolumn{2}{|c|}{D}       & \multicolumn{2}{|c|}{D+TL}     & \multicolumn{2}{|c|}{D+NV}     & \multicolumn{2}{|c||}{D+TL+NV} & \multicolumn{3}{|c|}{All} \\\hline\hline
Number        &  \multicolumn{2}{|c|}{382}     &  \multicolumn{2}{|c|}{196}     &  \multicolumn{2}{|c|}{152}      & \multicolumn{2}{|c|}{302}     &  \multicolumn{2}{|c|}{116}      & \multicolumn{2}{|c|}{272}       &  \multicolumn{2}{|c||}{136} &  \multicolumn{3}{|c|}{1,556}        \\\hline\hline                                                            
CRIKEY       &42  &    77&\multicolumn{2}{|c|}{---}&    &       &47 &    66&\multicolumn{2}{|c|}{---}&98  &    55&\multicolumn{2}{|c||}{---}&56  &61 & 42 \\\hline
FAP           &33  &    64&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&33  &74  &16 \\\hline
FD            &83  &    62&84  &   100&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&83  &75  &28 \\\hline
FDD           &92  &    62&84  &   100&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&88  &75  &28 \\\hline
LPG-3      &55  &    62&\multicolumn{2}{|c|}{---}&42  &     24&45 &    62&\multicolumn{2}{|c|}{---}&56  &     50&\multicolumn{2}{|c||}{---}&51  &54  &38 \\\hline
LPG-TD        &67  &    87&75  &    74&61  &     37&76 &    62&63  &    100&96  &     50&87  &   100 &76  &71  &71 \\\hline
Macro-FF      &57  &    87&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&57  &100  &21 \\\hline
Marvin        &67  &    62&34  &   100&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&52  &75 &28  \\\hline
Optop         &    &      &\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&   &      & 8  &     43&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}& 8  & 7  & 3 \\\hline
P-MEP         &15  &    61&\multicolumn{2}{|c|}{---}& 8  &     55&24 &    45&24  &     43&13  &     32&    &       &17  &43  &38 \\\hline
Roadmapper    &28  &    49&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&28  &56 &12  \\\hline
SGPlan        &68  &   100&65  &   100&64  &    100&75 &    90&78  &     74&85  &    100&74  &   100 &73  &96 &96  \\\hline
Tilsapa       &    &      &\multicolumn{2}{|c|}{---}&    &       &   &      &10  &     69&    &       &62  &    63 &38  &13  &11 \\\hline
YAHSP         &77  &    87&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&77  &100 &21 \\\hline\hline
BFHSP         &29  &    87&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&29  &100 &21 \\\hline
CPT           &33  &    87&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&22 &   100&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&28  &100& 41 \\\hline
HSP$_a^*$     &33  &    38&\multicolumn{2}{|c|}{---}&    &       &10 &    62&\multicolumn{2}{|c|}{---}&50   &    50&\multicolumn{2}{|c||}{---}&29    &44 & 30 \\\hline
Optiplan      &34  &    87&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}& \multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&34    &100 &21 \\\hline
SATPLAN       &46  &    87&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&46    &100&21  \\\hline
SemSyn        &49  &    48&\multicolumn{2}{|c|}{---}&11  &     37&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c|}{---}&\multicolumn{2}{|c||}{---}&40    &23  &15 \\\hline
TP4        &29  &    64&\multicolumn{2}{|c|}{---}&    &       &17 &    62&\multicolumn{2}{|c|}{---}&52  &     50&\multicolumn{2}{|c||}{---}&31    &54 & 37 \\\hline
\end{tabular}
\end{small}
\caption{\label{tab:results-overview}An overview of the IPC-4 results. Used abbreviations: ``N'' no durations, 
  ``DP'' derived predicates, ``NV'' numeric variables, ``D'' durations, ``TL'' timed initial literals. Line ``Number'' gives number of instances, all other lines give percentage values. In each entry, the right number is the percentage of instances that were attacked, and the left number is the percentage {\em of these} that were solved -- i.e. the left number is the success ratio. In the rightmost column, the middle number is the percentage of attacked instances relative to all instances that lie within the language range of the respective planner; the right number is the percentage of attacked instances over all. A dash indicates that a planner can not handle a language subset. See the detailed explanation in the text.}
  \vspace{-0.0cm}
\end{table}

% 332
% CRIKEY       &123 &243 296&    &      &    &       &94 &   200&    &       &147 &    150&    &       &364 &646 \\\hline
% 332
% FAP           &80  &193 246&    &      &    &       &   &      &    &       &    &       &    &       & 80 &246 \\\hline
% FD            &196 &   236&164 &   196&    &       &   &      &    &       &     &      &    &       &360 &432 \\\hline
% FDD           &216 &   236&164 &   196&    &       &   &      &    &       &    &       &    &       &380 &432 \\\hline
% LPG-3      &130 &   236&    &      &15  &     36&83 &   186&    &       &76  &    136&    &       &304 &594 \\\hline
% LPG-TD        &222 &298 332&110 &   146&34  &     56&142&   186&86  &    116&130 &    136&119 &   136 &843 &1108\\\hline\
% Macro-FF      &189 &298 332&    &      &    &       &   &      &    &       &    &       &    &       &189 &332 \\\hline
% Marvin        &159 &   236&67  &   196&    &       &   &      &    &       &    &       &    &       &226 &432 \\\hline
% Optop         &    &      &    &      &    &       &   &      & 4  &     50&    &       &    &       & 4  & 50 \\\hline
% P-MEP         &35  &   232&    &      & 7  &     84&33 &   136&12  &     50&11  &     86&    &       &98  &588 \\\hline
% 332
% Roadmapper    &52  &   186&     &     &    &       &   &      &    &       &    &       &    &       &52  &186 \\\hline
% SGPlan        &261 &327 382&128 &   196&97  &    152&205&   272&67  &     86&231 &    272&101 &   136 &1090&1496    \\\hline
% 332
% tilsapa       &    &      &    &      &    &       &   &      &10  &     80&    &       &53  &    86 &63  &166 \\\hline
%                    total: 332 (ohne ADL PSR)
% YAHSP         &255 &277 332&    &      &    &       &   &      &    &       &    &       &    &       &255 &332 \\\hline\hline
% BFHSP         &97  &277 332&    &      &    &       &   &      &    &       &    &       &    &       &97  &332 \\\hline
% CPT           &109 &277 332&    &      &    &       &72 &   302&    &       &    &       &    &       &181 &634 \\\hline
% Optiplan      &114 &277 332&    &      &    &       &   &      &    &       &    &       &    &       &114 &332 \\\hline
% SATPLAN    &152 &277 332&    &      &    &       &    &     &    &       &    &       &    &       &152 &332 \\\hline
% SemSyn        &91  &   184&    &      & 6  &     56&   &      &    &       &    &       &    &       &97  &240 \\\hline
% TP4        &72  &193 246&    &      &    &       &31 &   186&    &       &71  &    136&    &       &174 &568 \\\hline
% HSP$_a^*$     &48  &93 146&    &      &    &       &19 &   186&    &       &68   &   136&    &       &135 &468 \\\hline






Table~\ref{tab:results-overview} is complicated, and needs some
explanation. First, consider the columns in the table. The leftmost
column is, as usual, for table indexing. The rightmost column contains
data for the entire set of instances in IPC-4. The columns in between
all refer to a specific subset of the instances, in such a way that
these subsets are disjunct and exhaustive -- i.e., the instance sets
associated with columns are pairwise disjunct, and their union is the
entire set of instances. The subsets of instances are defined by the
PDDL2.2 subsets they use. The abbreviations in
Table~\ref{tab:results-overview} are explained in the caption. ``X+Y''
means that these instances use language features ``X'' and ``Y'', and
none of the other features. For example, ``N+DP'' are (only) those
instances with uniform durations (i.e., PDDL2.2 level 1) and derived
predicates.  Note that Table~\ref{tab:results-overview} does not have
a column for {\em all} possible combinations of language features --
we show only those that were used by (a non-empty subset of) the IPC-4
benchmarks.  Note also that we do not distinguish between different
domain {\em formulations}, i.e. between ADL and STRIPS. The instance
numbers in Table~\ref{tab:results-overview} are counted for domain
{\em versions}. That is, if there is an ADL and a STRIPS formulation
of a version, then each instance is counted only once.\footnote{As
  said, each domain featured several domain {\em versions}, differing
  in terms of the application constraints modelled. Within each domain
  version, there could be several different domain version {\em
    formulations}, differing in terms of the precise PDDL subset used
  to encode the {\em same} semantics. In most cases with more than one
  formulation, there were exactly two formulations, using/not using
  ADL constructs, respectively.  Competitors could choose the
  formulation they liked best and the results across different
  formulations were evaluated together.} 



The first line in Table~\ref{tab:results-overview}, indexed
``Number'', simply gives the size of the instance set associated with
the column. All other lines correspond, obviously, to planning
systems. The upper half of the table contains, in alphabetical order,
the satisficing planners; the lower half contains the optimal
planners.  Note that we list only one version of LPG-TD.  This is
because the ``speed'' and ``quality'' version of this planner differ
in terms of plan quality, but not in terms of the number of
attacked/solved instances.




Let us consider the table entries in between the leftmost and
rightmost columns, i.e., the entries concerning a planner ``X'' and a
language/instance subset ``Y''. The numbers in these entries are the
{\em success ratio} and the {\em attacked ratio}. Precisely, they were
obtained as follows. We first counted the number ``y'' of instances in
``Y'' that planner ``X'' tried to solve -- our definition was to take
all domain versions (inside ``Y'') for which ``X'' delivered results,
and set ``y'' to be the total number of instances in these domain
versions. We then counted the number ``x'' of instances in ``Y'' that
planner ``X'' succeeded to solve. We obtained the first number in the
table entry -- the success ratio -- as the ratio (in percent) of ``x''
divided by ``y''. We obtained the second number in the entry -- the
attacked ratio -- as the ratio (in percent) of ``y'' divided by the
size of ``Y''. For space reasons, we rounded the percentages to the
values shown in the table. A dash in the table entry means that the
planner ``X'' can not handle the language subset ``Y''. An empty table
entry means that the planner can handle ``Y'', but did not attack any
instance in ``Y''.


In a few cases, namely in the Promela domain, see the discussion in
Section~\ref{results:promela}, we could not formulate the largest
instances in STRIPS because these (fully-grounded) representations
became too large. So, there, the numbers of test instances are
different between the ADL and STRIPS formulations {\em of the same
  domain version}.\footnote{In PSR, it also was impossible to
  formulate the largest instances in STRIPS.  But, there, we split the
  domain into different {\em versions} regarding the size and
  formulation language of the instances. We did not want to introduce
  more distinction lines in Promela because there we already had 8
  different domain versions.}  Table~\ref{tab:results-overview} uses
the number of ADL instances, not taking account of this subtlety. This
implies a slight disadvantage in terms of success ratio in columns
``N'' and ``All'', for the planners that attacked the smaller STRIPS
test suites. These planners are the following, with correct column
``N'' success ratio in parentheses: CRIKEY (51), FAP (41), LPG-TD
(74), SGPlan (80), YAHSP (92), BFHSP (35), CPT (39), HSP$_a^*$ (52),
Optiplan (41), SATPLAN (55), and TP4 (37).



The table entries in the rightmost column are obtained similarly as
above. They summarize the situation regarding the respective planners
across {\em all} used language subsets. The left and right number in
each entry give the ratio of the number of solved instances to the
number of attacked instances, and the number of attacked instances to
the number of all instances, respectively. The number in the middle of
each entry gives the ratio of the number of attacked instances to the
number of all instances {\em that lie within the language range of the
  respective planner.} We included this number in order to provide a
measure of to what extent each planner/team attacked those instances
that they could attack.



Some remarks are in order regarding the latter ratio, and the ratio of
attacked instances in general. First, there was no rule telling the
competitors to ``attack everything they can'' -- competitors were free
to choose. In retrospect, we feel that there should have been such a
rule, since it would make data interpretation easier. The way things
are, it is not known for what reason a planner did not attack an
instance subset (domain version): Bad results? Not interested?
Overlooked? Second, many planners can handle only subsets of
certain language features, like, of numeric variables (``NV''). This
can lead to too low percentages in Table~\ref{tab:results-overview},
where for simplicity we do not take account of these details. Third, 
one detail we {\em did} take account of is
that 50 of the 382 instances in column ``N'' (namely, the
``middle-compiled'' version of the PSR domain, see
Section~\ref{results:psr}) are formulated in ADL only, and are thus
not accessible to many of the planners. For planners not able to
handle ADL, when computing the middle number in the rightmost table
entry, we subtracted these 50 instances from the ``instances within
the language range'' of the respective planner. In column ``N'',
however, we took the usual ratio to the set of {\em all} instances --
in particular, this is why Macro-FF, YAHSP, BFHSP, CPT, Optiplan, and
SATPLAN all have an 87\% attacked-ratio in the ``N'' column, but a
100\% attacked-ratio as the middle number of the rightmost column.




All in all, the planners all have a pretty good coverage of the
language subset they could attack; except Optop, Tilsapa, and maybe
Semsyn. These planners/teams were probably interested only in a small
subset of the instances.\footnote{Drew McDermott, the developer of
  Optop, told us in private conversation that he tried to solve only
  the most complicated domain versions.} In the other cases where
instances were left out, planners/teams typically did not attack the
domain versions where derived predicates or timed initial literals had
been compiled away. Note that a lack of coverage may also be due to
language details not accounted for by the rather crude distinctions
made for Table~\ref{tab:results-overview}.\footnote{In private
  conversation, the LPG-TD team told us that this is the case for
  LPG-TD, and that they in fact attacked all domain versions they
  could at the time IPC-4 was running.}


% \footnote{In private conversation, the LPG-TD team
%   told us that they were actually integrating the new language
%   capabilities into their system on-line, i.e., while IPC-4 was
%   running. For some domain versions, they did not manage to implement
%   the needed capabilities in time. They did attack every domain
%   version they could. So in that sense the middle number in the
%   rightmost column should be $100$, not $71$, for LPG-TD.}




What can we conclude from Table~\ref{tab:results-overview}, in terms
of planner performance? Some spotlights are these:
\begin{itemize}
\item The success ratios of optimal planners are generally lower than
  those of satisficing planners. The largest overall success ratio of
  an optimal planner, SATPLAN, is 46 (55 when taking account of the
  above mentioned subtlety regarding ADL/STRIPS formulations in
  Promela); compared to 88 for FDD.
\item However, there are also various cases where an optimal planner
  has a higher success ratio than a satisficing one.
\item FD, FDD, and YAHSP have the best success ratios (as mentioned,
  the success ratio of YAHSP in the ``N'' column is 92 when taking
  account of ADL/STRIPS in Promela). FD and FDD also have a pretty
  good coverage in the ``N'' and ``N+DP'' columns, i.e. within PDDL2.2
  level 1 (the left out instances are the domain versions with
  compiled derived predicates).
\item SGPlan has an extremely high coverage, attacking 96\% of {\em
    all} instances. Even so, it has a very competitive success ratio.
  (Concretely, SGPlan solved 1,090 of the 1,556 IPC-4 instances; it
  attacked 1,496. The second place in terms of the %sheer
  number of instances solved is held by LPG-TD, which solved 843 out
  of the 1108 instances it could attack.)
\item LPG-3, i.e. the IPC-3 version of LPG, ranges somewhere in the
  middle-ground of the planners, in terms of success ratio and
  coverage. This indicates that significant performance improvements
  were made in difference to IPC-3. (Note that this holds for the new
  LPG version just as for the other top performance planners.)
\end{itemize}




Naturally, in our evaluation of the results, particularly in the
evaluation that formed the basis of the award decisions, we undertook
a more detailed examination of the data set. We considered, as much as
possible, {\em scaling behavior}, rather than the simple instance
counts above. In what follows, we first explain our evaluation process
in detail, then we consider each of the domains in turn.












\subsection{Results Evaluation}
\label{results:evaluation}






As said, runtime data for satisficing and optimal planners was
considered separately. For plan quality, we distinguished between
three kinds of optimization criteria: number of actions, makespan
(equalling the number of time steps in the non-temporal domains), and
metric value.  The last of these three was only defined if there was a
{\tt :metric} specification in the respective task. We compared each
planner according to only a single plan quality criterion. That is,
for every domain version the competitors told us what criterion their
planner was trying to optimize in that domain version. We evaluated
all (and only) those planners together that tried to optimize the same
criterion. Our reason for doing so is that it does not make sense to
evaluate planners based on criteria they don't actually consider.



Altogether, for every domain version we created up to 5 \emph{gnuplot}
graphics: for satisficing runtime, for optimal runtime, for number of
actions, for makespan, and for metric value. The plan quality data of
optimal planners was put into the same plots as those for satisficing
planners, to enable some comparison. In a few cases, we had to split a
runtime figure (typically, for satisficing planners) into two separate
figures because with too many runtime curves in it the graphic became
unreadable.




Based on the \emph{gnuplot} graphics, we evaluated the data in terms
of asymptotic runtime and solution quality performance. The
comparisons between the planners were made by hand, i.e. by looking at
the graphs.  While this is simplistic, we believe that it is an
adequate way of evaluating the data, given the goals of the field, and
the demands of the event. It should be agreed that what we are
interested in is the (typical) scaling behavior of planners in the
specific domains.  This excludes ``more formal'' primitive comparative
performance measures such as counts of instances solved more
efficiently -- a planner may scale worse than another planner, yet be
faster in a lot of smaller instances just due to pre-processing
implementation details.  The ideal formal measure of performance would
be to approximate the actual scaling functions underlying the
planners' data points. But it is infeasible to generate enough data,
in an event like the IPC, to do such formal approximations. So we
tried to judge the scaling behaviors by hand, laying most emphasis on
how efficiently/if at all the largest instances in a test suite were
solved by a planner.\footnote{Note that the success ratios displayed
  in Table~\ref{tab:results-overview} are also a crude way to access
  scaling behavior.}



The rest of the section contains one sub-section for each domain in
turn. Each sub-section provides the following material. First, we give
a brief description of the domain and its most important features
(such as domain versions and formulations used in IPC-4). We then
include a set of gnuplot graphics containing (what we think are) the
most important observations regarding runtime (the total set of
gnuplot graphs is too space-consuming). We discuss plan quality, with
data comparing the relative performance of pairs of planners.  We also
add some intuitions regarding structural properties of the domains,
and their possible influence on the performance of the planners.
Finally, we provide the information -- 1st and 2nd places, see below
-- underlying the decisions about the awards. This information is
contained in a text paragraph at the end of the sub-section for each
domain. %, so the un-interested reader can skip it over.



As the basis for deciding about the awards, within every domain
version, we identified a group of planners that scaled best and
roughly similar. These planners were counted as having a 1st place in
that domain version. Similarly, we also identified groups of 2nd place
planners. The awarding of prizes was then simply based on the number
of 1st and 2nd places of a planner, see
Section~\ref{awards}.\footnote{Of course, many of the decisions about
  1st and 2nd places were very close; there were numerous special
  cases due to, e.g., what planners participated in what domain
  versions; summing up the places introduces a dependency of the
  results on the number of domain versions in the individual domains.
  To hand out awards one has to make decisions, and in these decisions
  a lot of detail is bound to disappear. One cannot summarize the
  results of such a huge event with just a few prizes.}




We consider the domains in alphabetical order. Before we start, there
are a few more remarks to be made.  First, some planners are left out
of the plots in order to make the plots readable.  Specifically, we
left out LPG-TD.quality as well as LPG-3.quality (the IPC-3 version of
LPG with a preference on quality); these planners are always slower
than their counterparts with a preference on speed. We also left out
FD, since in most cases it showed very similar behavior to FDD. We
chose FDD because in a few cases its performance is superior. Note
further that we do not distinguish the runtime performance of optimal
planners optimizing different criteria.  Finally, it can make
a significant difference whether a planner is run on an ADL encoding,
or on its compilation to STRIPS; this distinction also gets lost in
our evaluation. We emphasize that we applied the simplifications only
in order to improve readability and understandability of the results.
We do not wish to imply that the planners/distinctions that are
omitted aren't important.






\input{Airport}

\input{Pipesworld} 

\input{Promela} 

\input{PSR}

\input{Satellite}

\input{Settlers}

\input{UMTS}







==> hoffmann05a/revisions.tex <==












\section{Main Revisions made in IPC-4}
\label{revisions}





The main revisions we made to the deterministic part of IPC-4, in
difference to its predecessors, were the following.



{\bf Competition Workshop.} We ran an international workshop on the
competition one year before the event itself
\cite{Own:WS-Proceedings}, providing the involved groups of people
(system developers, organizing committee, AI Planning researchers in
general) with an opportunity to express their views on issues related
to the IPC. Discussions, technical talks, and panels covered all
relevant topics ranging from the event's organizational structure and
its input language to the selection of benchmarks and the evaluation
of results. The workshop was especially useful for us as the
organizers, giving us direct feedback on the event's organization.





{\bf PDDL Extensions.} There was large agreement in the community that
PDDL2.1 still posed a significant challenge, and so the IPC-4 language
featured only relatively minor extensions. We added language features
for \emph{derived predicates} and \emph{timed initial literals}. The
resulting language is called PDDL2.2, and keeps the 3-leveled
structure of PDDL2.1. Both new language features are practically
motivated and were put to use in some of the IPC-4 domains. Derived
predicates add a form of domain axioms to PDDL2.1. A typical use is to
formulate indirect consequences of a planner's actions.  Timed initial
literals add to the temporal part of PDDL2.1 (level 3) 
a way of defining literals that will become true at a certain time point,
independently of the actions taken by the planner. A typical use is to
formulate time windows and/or goal deadlines.






{\bf Application-Oriented Benchmarks.} Our main effort in the
organization of IPC-4 was to devise a range of interesting benchmark
domains, oriented at (and as close as possible to) real-world
application domains. We collaborated with a number of people to
achieve this goal. The description of the application domains, and of
our PDDL2.2 adaptations, is long (50+ pages). It is submitted to this
same JAIR special track \cite{Benchmarks}. The application domains we
modelled were:
\begin{itemize}
\item \emph{Airport}, modelling airport ground traffic control
  \cite{hatzack:nebel:ecp-01,trueg:etal:ki-04}.
\item \emph{Pipesworld}, modelling oil derivative transportation in
  pipeline networks
  \cite{milidiu:et:al:icaps-ws-03,milidiu:liporace-hms-04}.
\item \emph{Promela}, modelling deadlock detection in communication
  protocols formulated in the Pro\-me\-la language \cite{edelkamp:spin-03,edelkamp:icaps-ws-03}.
\item \emph{PSR}, a deterministic variant of the Power Supply
  Restoration benchmark
  \cite{bertoli:etal:ecai-02,bonet:thiebaux:icaps-03}.
\item {\em UMTS}, modelling the task of scheduling the concurrent
  application setup in UMTS mobile devices~\cite{Englert:TP4,Roman:Journal}.
\end{itemize}
In addition, we re-used the \emph{Satellite} and \emph{Settlers}
domains from IPC-3. In the case of \emph{Satellite}, we added some
additional domain versions to model more advanced aspects of the
application (namely, the sending of the data to earth). Each domain is
described in a little more detail in the part (sub-section) of
Section~\ref{results} that contains the respective competition
results.








{\bf Domain Compilations.} For the first time in the IPC, we provided
domain formulations where problem constraints were compiled from the
more complex PDDL subsets into the less complex subsets. In many of
our domains the most natural domain formulation comes with complex
precondition formulas and conditional effects, i.e., in ADL. We
compiled these domain formulations to STRIPS. In previous IPCs, for
example in the {\em Elevator} domain used in IPC-2, the more
interesting problem constraints were dropped in the STRIPS domain
versions. By using the compilation approach, we hope and believe to
have created a structurally much more interesting range of STRIPS
benchmarks. The ADL and STRIPS encodings of the same instances were
posed to the competitors in an optional way, i.e., of every domain
{\em version} there could be several domain version {\em
  formulations}. The competitors were allowed to choose the
formulation they liked best. The results within a domain version were
evaluated together, in order to keep the number of separation lines in
the data at an acceptable level.


We also employed compilations encoding the new PDDL2.2 language
features in terms of artificial constructs with the old PDDL2.1
features. By this we intended to enable as wide participation in the
domains as possible. The compiled domains were offered as separate
domain {\em versions} rather than alternative formulations because, in
difference to the ADL/STRIPS case, we figured that the compiled
domains were too different from the original ones to allow joint
evaluation. Most importantly, when compiling derived predicates or
timed initial literals away, the plan length increases. Details about
the compilation methods and about the arrangement of the individual
domains are in the paper describing these domains \cite{Benchmarks}.






{\bf Optimal vs. Satisficing Planning.} We define {\em optimal}
planners as planners that prove a guarantee on the quality of the
found solution.  Opposed to that, {\em satisficing} planners are
planners that do {\em not} prove any guarantee other than the
correctness of the solution.\footnote{Satisficing planners were
  referred to as ``sub-optimal'' when IPC-4 was running. We decided to
  replace the term since it is a bit misleading. While not
  guaranteeing optimal solutions, a satisficing planner may well
  produce such solutions in some cases.} Previous IPCs did not
distinguish between optimal planners and satisficing planners. But
that is not fair since optimal planners are essentially solving a
different problem. The theoretical hardness of a domain can differ for
the different kinds of planners. In fact, it was recently proved that,
in most benchmark domains, satisficing planning is easy (polynomial)
while optimal planning is hard (NP-complete)
\cite{helmert:ecp-01,helmert:ai-03}. In practice, i.e., in most of the
commonly used benchmark domains, nowadays there is indeed a huge
performance gap between optimal and satisficing planners. In IPC-4, we
separated them into different tracks. The optimal track attracted
seven systems; for example, the planning as satisfiability approach,
that had disappeared in IPC-3, resurfaced.





{\bf Competition Booklet and Results Posters.} At previous
competitions, at conference time one could neither access the results
obtained in the competition, nor descriptions of the competing
planners. This is clearly a drawback, especially given the growing
complexity of the event. For ICAPS 2004, we assembled a booklet
containing extended abstracts describing the core aspects of all
competing systems \cite{Own:Comp-Proceedings}; the booklet was
distributed to all conference participants. The competition results,
i.e., those of the deterministic part, were made available in the form
of posters showing runtime and plan quality plots.






\begin{sloppypar}
{\bf IPC Web-page.} An important repository for any large-scale
competition event is a web page containing all the relevant information --
benchmark problems, language descriptions, result files, etc. For
IPC-4, we have set this page up at the permanent Internet address
\texttt{http://ipc.icaps-conference.org}. In the long run, this
address is intended to provide an entry point to {\em the IPC event as
  a whole}, thereby avoiding the need to look up the pages for the
different IPC editions at completely separate points in the web.
\end{sloppypar}








As a less positive change from IPCs 2 and 3 to IPC-4, the track for
{\em hand-tailored} planners disappeared. The reason for this is
simply that no such systems registered as competitors. Of course, this
is not a coincidence. There is a large agreement in the community that
there are several problems with the hand-tailored track as ran in
IPC-2 and IPC-3. The most important criticism is that, for
hand-tailored planners, ``performance'' is not just runtime and plan
quality results on a set of benchmarks. What's also important -- maybe
the most important aspect of all -- is how much effort was spent in
achieving these results: {\em how hard is it to tailor the planner?}
While the latter obviously is an important question, likewise
obviously there isn't an easy answer. We discussed the matter with a
lot of people (e.g., in the ICAPS'03 workshop), but no-one could come
up with an idea that seemed adequate and feasible. So basically we
offered the hand-tailored planners the opportunity to participate in a
track similar to the previous ones, maybe with some additional ad-hoc
measurements such as how many person hours were spent in tailoring the
planner to a domain. Apart from the evaluation shortcomings of such an
approach, another important reason why no hand-tailored planners
registered is that participating in that track is a huge amount of
work -- maintaining/developing the planner {\em plus} understanding
the domains and tailoring the planner. Understanding the domains would
have been particularly hard with the more complex domains used in
IPC-4. It is thus, obviously, difficult to find enough time to
participate in a hand-tailored IPC. Some more on the future of the
hand-tailored track is said in Section~\ref{conclusion}.












%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> hoffmann05a/systems.tex <==










\section{The Competitors}
\label{systems}




We now provide an overview table listing the systems along with their
language capabilities (subset of PDDL2.2 covered), and we sketch the
competing systems.  The deterministic part of IPC-4 attracted 19
competitors (21 when counting different system versions), 12 (14) of
which were satisficing and 7 of which were optimal. Each competitor
wrote a 2-3 page extended abstract for inclusion in the IPC-4 booklet
at ICAPS 2004 \cite{Own:Comp-Proceedings}. The included sketches are
very brief outlines of these abstracts. The reader is encouraged to
read the original work by the system authors.





At this point it is appropriate to say a few words on system
development.  We allowed competitors to modify their systems during
the competition phase, i.e., while data collection was running. Our
reasons for doing so were twofold. First, some of our domains were
quite unusual -- most particularly, those containing ADL constructs
compiled to STRIPS -- so we (rightly) expected planner implementations
to have parsing etc. trouble with them. Second, from our own
experience with the competitions we knew that people will try to
enhance their planners anyway so we did not see much point in
forbidding this. We trusted the competitors to not do stupid things
like hard-coding domain names etc., and we trusted to have a diverse
enough range of domains to make tuning a ``domain-independent'' task.


An alternative would have been to collect executables before data
collection, and then have all the results collected by the organizers.
Anyone who has ever run experiments with someone else's planner knows
that such an approach is completely infeasible due to the
prototype-nature of the systems, and due to the many tiny details in
minor language changes, programming environments, etc. -- if one wants
to obtain meaningful results, at least. One could in principle apply a
strict ``any failure is counted as unsolved'' rule, but doing so would
likely lay way too much emphasis on little programming errors that
have nothing to do with the evaluated {\em algorithms}.



The competition phase was, roughly, from February 2004 until middle
May 2004. During that time, we released the domains one-by-one, and
the competitors worked on their systems, handing the results over to
us when they were ready. At the end of that phase, the competitors had
to submit an executable, and we ran some sampled tests to see that the
executable did really produce the reported results, across all the
domains. The abstracts describing the systems had to be delivered a
little earlier, by the end of April, due to timing constraints for
printing the booklet.







We start with the overview table, then sketch the satisficing and
optimal competitors.






\subsection{Planner Overview}
\label{systems:overview}


An overview of the participating satisficing planners, and their
language capabilities (defined as what language features they attacked
in IPC-4), is given in Table~\ref{tab:planners-overview}.



\begin{table}[htb]
\centering
\begin{small}
\centering
\begin{tabular}{|l||c|c|c|c|c|}
\hline    
              &  ADL     &  DP      &  Numbers    & Durations &  TL      \\
\hline
\hline
CRIKEY       &   -      &   -      &    +        &   +      &    -       \\\hline
FAP           &   -      &   -      &    -        &   -      &    -       \\\hline
FD, FDD       &   +      &   +      &    -        &   -      &    -       \\\hline
LPG-TD        &   +      &   +      &    +        &   +      &    +       \\\hline
Macro-FF      &   +      &   -      &    -        &   -      &    -       \\\hline
Marvin        &   +      &   +      &    -        &   -      &    -       \\\hline
Optop         &   +      &   +      &    +        &   +      &    +       \\\hline
P-MEP         &   +      &   -      &    +        &   +      &    +       \\\hline
Roadmapper    &   -      &   -      &    -        &   -      &    -       \\\hline
SGPlan        &   +      &   +      &    +        &   +      &    +       \\\hline
Tilsapa       &   -      &   -      &    +        &   +      &    +       \\\hline
YAHSP         &   -      &   -      &    -        &   -      &    -       \\\hline\hline
BFHSP         &   -      &   -      &    -        &   -      &    -       \\\hline
CPT           &   -      &   -      &    -        &   +      &    -       \\\hline
HSP$_a^*$     &   -      &   -      &    +        &   +      &    -       \\\hline
Optiplan      &   -      &   -      &    -        &   -      &    -       \\\hline
SATPLAN     &   -      &   -      &    -        &   -      &    -       \\\hline
SemSyn        &   +      &   -      &    +        &   -      &    -       \\\hline
TP4        &   -      &   -      &    +        &   +      &    -       \\\hline
\end{tabular}
\end{small}
\caption{\label{tab:planners-overview}An overview of the planners in IPC-4, and their language capabilities 
  (i.e., the language features they attacked in IPC-4). satisficing planners are in the top half of the table, optimal planners are in the bottom half.
  Each table entry specifies whether (``+'') or not (``-'') a planner 
  can handle a language feature. 
  ``DP'' is short for derived predicates, ``TL'' is short
  for timed initial literals. With ``Numbers'' and ``Durations'' 
  we mean numeric fluents and fixed action durations (no duration 
  inequalities), in the sense of PDDL2.1 level 2 and 3, respectively. The 
  planners 
  (and their name abbreviations) are explained below.}
\vspace{-0.0cm}
\end{table}



Observe that most of the planners treat only a small subset of
PDDL2.2: from a quick glance at the table, one sees that there are far
more (``-'') entries than (``+'') entries. Note here that, often, even
when a (``+'') sign is given, a planner may treat only a subset of the
specified language feature (as needed for the respective IPC-4
domain). For example, a planner might treat only a subset of ADL, or
only linear arithmetic for numeric variables. We leave out these
details for the sake of readability.



LPG-TD, Optop, and SGPlan are the only planners that treat the full
range of PDDL2.2, as used in IPC-4. Three satisficing planners (FAP,
Roadmapper, and YAHSP), and three optimal planners (BFHSP, Optiplan,
and SATPLAN), treat only pure STRIPS.  Derived predicates are treated
by 4 planners, timed initial literals by 5 planners, ADL by 7
planners, numeric variables by 8 planners, and action durations by 9
planners.




Table~\ref{tab:planners-overview} shows that there is a significant
amount of acceptance of the new (PDDL2.1 and PDDL2.2) language
features, in terms of implemented systems participating in the IPC.
Table~\ref{tab:planners-overview} also shows that the development on
the systems side has a tendency to be slower than the development on
the IPC language side: even the most wide-spread language feature
beyond STRIPS, action durations, is dealt with by less than half of
the 19 planners. In our opinion, this should be taken to indicate that
further language extensions should be made slowly. Some more on this
is said in Section~\ref{conclusion}.











\subsection{Satisficing Planners}
\label{systems:satisficing}





The satisficing planners -- the planners giving no guarantee on the
quality of the returned plan -- were the following. We proceed in
alphabetical order.



{\bf CRIKEY} by Keith Halsey, University of Strathclyde, Glasgow, UK.
CRIKEY is a heuristic search forward state space planner. It includes
a heuristic for relaxed plans for temporal and numeric problems and
applies a scheduler based on simple temporal networks to allow
posterior plan scheduling.





{\bf FAP} by Guy Camilleri and Joseph Zalaket, University Paul
Sabatier / IRIT CCI-CSC, France. FAP handles non-temporal non-numeric
domains. It is a heuristic planner using the relaxed planning
heuristic in an $N$-best forward search, with meta-actions (action
sequences) extracted from the relaxed planning graph to perform jumps
in the state space.






{\bf Fast Downward}, \emph{FD} for short, and {\bf Fast Diagonally
  Downward}, \emph{FDD} for short, by Malte Helmert and Silvia
Richter, University of Freiburg, Germany. FD and FDD can treat
non-temporal non-numeric domains. They apply a new heuristic estimate
based on a polynomial relaxation to the automatically inferred
multivariate or SAS$^+$ representation of the problem space.  FDD also
applies the traditional FF-style relaxed planning heuristic, i.e., it
applies both heuristics in a hybrid search algorithm.





{\bf LPG-TD} by Alfonso Gerevini, Alessandro Saetti, Ivan Serina, and
Paolo Toninelli, University of Brescia, Italy. The extensions to the
randomized local plan graph search that was already included in LPG at
IPC-3 includes functionality for PDDL2.2 derived predicates and timed
initial literals, as well as various implementation refinements. A
version tailored to computation speed, LPG-TD.speed, and a version
tailored for plan quality, LPG-TD.quality, participated.
LPG-TD.quality differs from LPG-TD.speed basically in that it does not
stop when the first plan is found but continues until a stopping
criterion is met. The LPG-TD team also ran a third version, called
``LPG-TD.bestquality'', which used, for every instance, the entire
half hour CPU time available to produce as good a plan as possible.
This third version is not included in the official data because every
team was allowed to enter at most two system versions.



 
{\bf Macro-FF} by Adi Botea, Markus Enzenberger, Martin M\"uller,
Jonathan Schaeffer, University of Alberta, Canada. As the name
suggests Macro-FF extends Hoffmann's FF planner with macro operators
(and other implementation refinements). Macros are learned prior to
the search and fed into the planner as new data, separated from the
operator file and the problem file.  At runtime, both regular actions
and macro-actions are used for state expansion.  Heuristic rules for
pruning instantiations of macros are added to FF's original strategy
for search control.



{\bf Marvin} by Andrew Coles and Amanda Smith, University of
Strathclyde, Glasgow, UK. Marvin extends FF by adding extra features
and preprocessing information, such as plateau-escaping macro actions,
to enhance the search algorithm.



{\bf Optop} by Drew McDermott, Yale University, USA. Optop is an
extension of the well-known UNPOP planner, with the ability to handle
a complex input language including, amongst other things, autonomous
processes running in parallel to the actions taken by the planner. The
underlying principle is a forward search with heuristic guidance
obtained from greedy-regression match graphs that are built backwards
from the goals.





{\bf P-MEP} by Javier Sanchez, Minh Tang, and Amol D. Mali, University
of Wisconsin, USA. P-MEP is short for Parallel More Expressive
Planner. Unlike most planners, P-MEP can treat numeric variables with
non-linear action effects. It employs a forward search with relaxed
plan heuristics, enhanced by relevance detection in a pre-process, and
by taking into account exclusion relations during relaxed planning.






{\bf Roadmapper} by Lin Zhu and Robert Givan, Purdue University, USA.
Roadmapper handles non-temporal non-numeric domains. It is a forward
heuristic search planner enhancing the FF heuristic with a reasoning
about landmarks. The latter are propositions that must be true at some
point in every legal plan.  Roadmapper finds landmarks in a
pre-process, arranges them in a directed road-map graph, and uses that
graph to assign weights to actions in the FF-style relaxed plans.





{\bf SGPlan} by Yixin Chen, Chih-Wei Hsu and Benjamin W. Wah,
University of Illinois, USA. The planner bootstraps heuristic search
planners by applying Lagrange optimization to combine the solution of
planning subproblems.  To split the problem, an ordering of the
planning goals is derived.  The incremental local search strategy that
is applied for Lagrange optimization on top of the individual planners
relies on the theory of extended saddle points for mixed integer
linear programming.





{\bf Tilsapa} by Bharat Ranjan Kavuluri and Senthil U., AIDB Lab, IIT
Madras, India. The planner extends the SAPA system that handles
temporal numeric domains, with the ability to handle timed initial
literals.






    
{\bf YAHSP} by Vincent Vidal, University of Artois, France.  YAHSP, an
acronym for \emph{yet another heuristic search planner}, searches
forward with a FF-style relaxed planning heuristic. The main
enhancement is a relaxed-plan-analysis phase that replaces actions in
the relaxed plan based on heuristic notions of better suitability in
reality, producing macro-actions in the process. The macro-actions
are, basically, as long as possible feasible sub-sequences of the
(modified) relaxed plan.






















\subsection{Optimal Planners}
\label{systems:optimal}







The participating optimal planners were the following, in alphabetical
order.





  
{\bf BFHSP} by Rong Zhou and Eric A. Hansen, Mississippi State
University, USA. BFHSP, for breadth-first heuristic search planner,
optimizes the number of actions in the plan. The planner implements
the standard max-atom and max-pair heuristics (as well as the
max-triple heuristic, which was however not used in IPC-4). The main
difference to other systems is its search algorithm called {\em
  breadth-first heuristic search}; this improves the memory
requirements of A* search by searching the set of nodes up to a
certain threshold value in breadth-first instead of best-first manner.





{\bf CPT} by Vincent Vidal, University of Artois, France, and Hector
Geffner, University of Pompeu Fabra, Barcelona, Spain. CPT optimizes
makespan. The planner is based on constraint satisfaction, and
transforms the planning problem to a CSP.  The branching scheme that
solves the CSP makes use of several constraint propagation techniques
related to POCL, and of the temporal max-atom heuristic.





{\bf HSP$_a^*$} by Patrik Haslum, Link\"oping University, Sweden.
HSP*$_a$ is a derivate of TP4, see below, with the same expressivity,
but with a weakened version of the \emph{MaxTriple} heuristic instead
of the \emph{MaxPair} heuristic.



{\bf Optiplan} by Menkes van der Briel and Subbarao Kambhampati,
Arizona State University, USA. Optiplan is a planner based on integer
programming (IP), which itself is a consequent extension to the
encoding of the planning graph used in the planning as satisfiability
approach (see below). The compiled planning problem is solved using
the CPLEX/ILOG system. An interesting property of Optiplan is that,
due to the power of the underlying IP solver, it can optimize a great
variety of different plan metrics, in fact every plan metric that can
be expressed with a linear function.  In that respect, the planner is
unique. In IPC-4, step-optimal plans were computed because that is
typically most efficient.





{\bf SATPLAN04}, \emph{SATPLAN} for short, 
by Henry Kautz, David Roznyai, Farhad Teydaye-Saheli,
Shane Neph, and Michael Lindmark, University of Washington, USA.
SATPLAN treats non-tem\-po\-ral non-nu\-meric domains and optimizes the
number of parallel time steps. The system did not participate in IPC-3
but in IPC-1 and IPC-2, so it was a real comeback. As the planner
compiles a planning problem to a series of satisfiability tests, the
performance of the system relies on the integrated back-end SAT
solver. The graph-plan encoding scheme underwent only minor changes,
but the underlying SAT solver is much more powerful than that of 4
years ago.




{\bf SemSyn} by Eric Parker, Semsyn Software, Tempe, Arizona. The
\emph{SemSyn} system optimizes the number of actions. Semsyn is linked
to a commercial product and applies a combination of forward and
backward chaining. Both searches are variants of the original
algorithms.  Forward chaining is \emph{goal-directed}, while backward
chaining is \emph{generalized}, comprising a partition of the
top-level goal.  As the product is proprietary, detailed information
on the system is limited.
    




{\bf TP4-04}, \emph{TP4} for short, by Patrik Haslum, Link\"oping University, Sweden.  The
planner is an extended makespan-optimal scheduling system that does an
IDA* search routine with the max-pair heuristic.  It can deal with a
restricted form of metric planning problems with numerical
preconditions and effects.



